A characterization of ramification groups via Taylor morphism

In this paper, we present a functorial method to define ramification groups, identifying them as inertia groups of an induced action on composite jet algebras. This framework lays the foundation for defining higher ramification groups for actions involving group schemes. To achieve this, we introduce Taylor maps within the category of commutative unitary rings at prime ideals of an R-algebra and compute their kernels for algebras of finite type over a field with separably generated residue fields.

==> chapters/preliminary.tex <==
In the following, $R$ denotes a commutative unitary ring and $S= \operatorname{Spec}(R)$. $\mathbb{N}$ denotes the natural number including the $0$. We denote $ \mathbf{Sets}$ the category of sets, $\mathbf{Alg}_R$ the category of $R$-algebra, $\mathbf{RedAlg}_R$ the category of reduced $R$-algebra and $\mathbf{Sch}_S$ the category of $S$-schemes. 

For any ring $R$ we denote $\operatorname{Nil}(R)=\{x \in R | x^n =0 \text{ for some } n \in \mathbb{N}\}$ the nilradical of $R$ and $R_{\operatorname{red}} = R / \operatorname{Nil}(R)$ the reduced part of $R$.

When $\Gamma$ is a group we denote $e_\Gamma$ the identity element of $\Gamma$. Given $C$ a $k$-algebra and $\mathfrak{p}$ is a prime ideal of $C$. We denote $k (\mathfrak{p})$ to be the residue field at $\mathfrak{p}$. That is, $k (\mathfrak{p})= \frac{C_\mathfrak{p}}{ \mathfrak{p}C_\mathfrak{p}}$. We also denote $\zeta_\mathfrak{p}$ to be the canonical morphism from $C$ to $k (\mathfrak{p})$. That is, $\zeta_\mathfrak{p}: C \rightarrow k (\mathfrak{p})$ sending $c$ to $[\frac{c}{1}]_\mathfrak{p}$ where $[\frac{c}{1}]_\mathfrak{p}$ is the class of $\frac{c}{1} \in C_\mathfrak{p}$ in the quotient $k (\mathfrak{p})$.

In the following, we denote $\iota^C_m: C \rightarrow C[t]/ (t^{m+1})$ to be the canonical embedding. %and $p^C_m : C[t]/ (t^{m+1}) \rightarrow C$ be the canonical projection. 

We denote $ [t]_{m}$ the class of $t$ in the quotient $C[t]/(t^{m+1})$. 

Given a $R$-algebra morphism $\varphi: C_1 \rightarrow C_2$, we denote by $\tilde{\varphi} :  C_1 [t]/ (t^{m+1}) \rightarrow C_2 [t]/ (t^{m+1})$ sending $\sum_{j=0}^m c_{j} [t]_n^j$ to $\sum_{j=0}^m \varphi (c_{j}) [t]_n^j$ and $\operatorname{Spec}(\varphi)$ the canonical $S$-scheme morphism from $\operatorname{Spec}(C_1)$ to $\operatorname{Spec}(C_2)$ induced by $\varphi$. 

Given $\phi: B \rightarrow C$ an $R$-algebra morphism and $D$ a $R$-algebra, we denote $\phi_*$ for the morphism  $\phi \circ -: \operatorname{Hom}_{ \mathbf{Alg}_R} ( D, B) \rightarrow \operatorname{Hom}_{ \mathbf{Alg}_R} ( D, C)$ sending the map $\psi$ to $\phi \circ \psi$ and $\phi^*$ for the morphism $- \circ \phi : \operatorname{Hom}_{ \mathbf{Alg}_R} ( C, D) \rightarrow \operatorname{Hom}_{ \mathbf{Alg}_R} ( B, D)$ sending the map $\psi$ to $\psi \circ \phi$. 

Given $B$ an $R$-algebra, %and $X$ an $ \operatorname{Spec}(R)$-scheme. We denote $X(C)$ to be the set \\
%$\operatorname{Hom}_{ \mathbf{Sch}_R} (  \operatorname{Spec}( C), X)$.
we denote $\underline{B}$ to be that functor: 
$$\begin{array}{llll} \underline{B} : & \mathbf{Alg}_R &  \rightarrow & \mathbf{Sets}\\
& C & \mapsto & \operatorname{Hom}_{ \mathbf{Alg}_R}( B ,C  )\\
& \varphi  & \mapsto & \varphi*.
\end{array}$$ 

We start by defining a jet $R$-algebra.

Let $B$ be a $R$-algebra. We denote $Aut_R(B)$ the group of automorphisms of $R$-algebra. Let $G$ be a subgroup of the $Aut_R(B)$. Let $\mathfrak{p}$ be a prime ideal of $B$ and $s \in \mathbb{N}^\ast$. Then we define 
the decomposition group  at $\mathfrak{p}$ to be the subgroup of $G$ denoted $G_{-1}( \mathfrak{p}) $ such that
$$G_{-1}( \mathfrak{p}) = \{ \sigma \in G | \sigma ( \mathfrak{p})= \mathfrak{p} \}$$ 
the inertia group at $\mathfrak{p}$ to be the subgroup of $G$ denoted $G_0( \mathfrak{p}) $ such that
$$G_0( \mathfrak{p}) = \{ \sigma \in G | \sigma ( \mathfrak{p})= \mathfrak{p} \text{ and } \sigma( x) - x \in \mathfrak{p}\}$$ 
and we define the $s$-ramification group at $\mathfrak{p}$ to be the subgroup of $G$ denoted $$G_s( \mathfrak{p}) = \{ \sigma \in G | \sigma ( \mathfrak{p})= \mathfrak{p} \text{ and } \sigma( x) - x \in \mathfrak{p}^{s+1} \}.$$
We denote $\pi_{\mathfrak{p}, s,t} :  B/\mathfrak{p}^s  \rightarrow  B/\mathfrak{p}^{t}$ where $s \geq t$ is the canonical quotient map and $\pi_{0,t} :  B  \rightarrow  B/\mathfrak{p}^{t}$ the canonical quotient map. We denote $\pi_{\mathfrak{p}}:= \pi_{\mathfrak{p}, 0,1}$.
In particular, for all $s\geq -1$, we define $\theta_s : G_{s-1}(\mathfrak{p})  \rightarrow \operatorname{Aut}_R ( B/\mathfrak{p}^{s+1})$ and $\operatorname{ker} (\theta_s ) = G_s ( \mathfrak{p})$. %We note that when $\mathfrak{p} \subseteq \mathfrak{q}$


==> chapters/ramify.tex <==
\section{Characterization of the ramification}
Let $k$ be a field and let $B$ be a $k-$algebra. 
\begin{lemma}
\label{lem:Gmtofibre}
Let us fix a prime ideal $\mathfrak{p}$ of $B$, $s \in \mathbb{N}^\ast$ and an automorphism $\sigma \colon B\rightarrow B$ of $R-$algebras such that for all $b \in B$, $\sigma (\mathfrak{p}) =\mathfrak{p}$ and  $\sigma (b)\in b \in \mathfrak{p}$. If for all $b \in B$, $\sigma(b)- b \in \mathfrak{p}^{s+1}  \, $ then $\underline{J_m(\sigma ) \otimes \operatorname{id}_{k(\mathfrak{p})}}|_{\underline{J_m(B)}_\mathfrak{p}}$  $=\operatorname{id}_{\underline{J_m(B)}_\mathfrak{p} }$ for all $m\leq s$. %acts trivially on $\mathcal{L}_s(B)\otimes_B$ $k(\mathfrak{p})$ 
%if and only if for all $b \in B$, $\sigma(b)\equiv b \pmod{\mathfrak{p}^{s+1}}  \, .$
\end{lemma}

\begin{proof} 


%Suppose $B= k [ x_1, \cdots, x_n]/ I$.  %Let $\mathfrak{p}$ a be a prime ideal of $B$ we have that there is a $\mathfrak{q}$ prime ideal of $ k [ x_1, \cdots, x_n]$ such that $I \subseteq \mathfrak{q}$ and $\mathfrak{p}=\frac{\mathfrak{q}}{I}$.
%We have that, for all $b \in B$, 
%$$\sigma^\ast\psi(b) = \psi(b) + \psi(\sigma(b)-b) \, . $$
Let $C$ be a $k$-algebra, $\psi\in \underline{J_m(B)}_\mathfrak{p}(C)$ and $b \in B$. In particular, we have \\ $\psi \in  \operatorname{Hom}_k(B, C[t]/(t^{m+1}))$ and $\psi(\mathfrak{p})\subseteq \overline{t} C[t]/(t^{m+1})$. Therefore $\psi(\mathfrak{p}^{m+1})\subseteq \overline{t}^{m+1} C[t]/(t^{m+1}).$
Thus, if  $\sigma( b )- b \equiv 0 \pmod{\mathfrak{p}^{m+1}} $, then 
$\psi ( \sigma( b )- b) = 0 $ for all $\psi\in \underline{J_s(B)}_\mathfrak{p}(C)$. 
%

%Let $\{f_i\colon i\in I\}$ be a set of generators of $\mathfrak{p}$.

%Then, there is a polynomial $p^{b}=\sum_{r=s+1}^{m} p_r^b\in B [(x_i)_{i\in I}]$, where $p_r^b$ is either $0$ or a homogeneous polynomial of degree $r$, such that $\sigma(b)-b=p^b((f_i)_{i\in I})$; it follows that 
%$$ \psi(\sigma(b)-b) = \widetilde{p^b}((\psi(f_i))_{i\in I}) \, , $$
%where, for a polynomial $g= \sum_{J \mbox{ multiindex}} a_J\underline{x}^J \in B[\underline{x}]$, we set $\widetilde{g} = \sum_{J \mbox{ multiindex}} \psi(a_J)\underline{x}^J \in \left( C[t]/(t^{s+1}) \right)[\underline{x}]$.
%Since $f_i \in \mathfrak{p}$, there is $u_i\in C[t]/(t^{s+1})$ such that $\psi(f_i)=\overline{t} u_i$, hence 
%$$ \forall r\geq s+1, \quad  \widetilde{p_r}^b((\psi(f_i))_{i\in I})= \widetilde{p_r^b}((\overline{t}u_i)_{ i\in I})=\overline{t}^r \widetilde{p_r^b}((u_i )_{i\in I})=0 \, ,$$
%therefore $\psi(\sigma(b)-b)=0$ and $\sigma^\ast(\psi)=\psi$.
%
%For the other direction, let us first consider the case where $B$ is a Noetherian algebra.
%Now assume that $\exists b\in B$ such that $\sigma(b)-b \in \mathfrak{p}^m\backslash \mathfrak{p}^{m+1}$ for some $m\leq s$. Consider the composition of morphisms
%$$ B \rightarrow B_\mathfrak{p} \rightarrow \widehat{B_\mathfrak{p}} \rightarrow k(\mathfrak{p})[x_1,\dots, x_n]/(I+ (x_1,\dots, x_n)^{m+1}) \, , $$
%where the first one is the localisation with respect to the prime $\mathfrak{p}$, the second one is the $\mathfrak{p}-$adic completion and the last one is given by \ref{cor:CohenStructQuot}.
%Since $\sigma(b)-b\in \mathfrak{p}^m\backslash \mathfrak{p}^{m+1}$, the composition above sends it to a non-zero element $f	\in (x_1,\dots, x_n)^m$.
%
%%Now notice that if $\dim B \geq 1$, then $\bigcap_{m>0} \mathfrak{p}^m$
%
%% We can write $ \sigma(b)-b = \sum_{r = d}^m p_r((f_i)_{i\in I}) $ for some integers $d \leq s$ and $m$ and homogeneous polynomials $p_r\in B\backslash \mathfrak{p}[(x_i)_{i\in I}]$ such that $\forall d\leq r\leq m, \, \deg(p_r)=r$, where the degree is given by $\deg(x_i)= v_{\mathfrak{p}}(f_i)\geq 1$, for $i\in I$. Let $\overline{p_r}\in k(p)[(x_i)_{i\in I}]$ be the reduction of $p_r$ modulo $\mathfrak{p}$; by construction $\overline{p_d}\neq 0$. Since $p_d$ is a polynomial, it depends on a finite number of variables, that we call $\{x_1,\dots, x_n\}$.
%
%\luigi{Now I start sharing a vague idea, maybe we can turn this into a proof. I will assume $B$ to be of finite type, because extending to the general case is subtler than I tought (and there are weird cases, like: for all m, $y_m= polynomial(y_{m+1})$).}
%
%Say that $B=k[y_1,\dots, y_N]/\Omega$, with $y_1=f_1, \dots, y_n=f_n$. Fix an algebraic closure $F$ of $k(p)$. Let us find $a=(a_1,\dots, a_N)\in V(\Omega)\subseteq \mathbb{A}^N(F)$ such that $\overline{p_d}(f_1(a),\dots, f_n(a))\neq 0$. \luigi{We have to prove that $\overline{p_d}(f_1,\dots,f_n)\notin \sqrt{\Omega}$, *OR* maybe work over some infinitesimal extension of $F$ and prove that it does not belong to $\Omega$}
%
%Consider the map $\psi\colon B \rightarrow F[t]/(t^{s+1})$ sending $y_j\mapsto y_j+\mathfrak{p} + t a_j$ (Here it seems useful an assumption on the possibility of choosing all the $f_j$ in $p\backslash p^2$ (so the $v_p(f_j)=1$ for all $j$, but maybe for this we need B regular at p, maybe not). Then  $\sigma^\ast\psi(b)=\psi(b)+\psi(\sigma(b)-b)$ and 
%$$ \psi(\sigma(b)-b) \cong p_d((f_j(a))_j) \pmod t^{d+1} $$
%so it is not 0.
%
%\luigi{stopped here, many gaps to fill.}
\end{proof}

\luigi{A thickened version of the previous lemma. Seems useful for $G_2$ when m=1, s=2}.

\begin{lemma}
Let us fix a prime ideal $\mathfrak{p}$ of $B$, $s \in \mathbb{N}^\ast$ and an automorphism $\sigma \colon B\rightarrow B$ of $R-$algebras such that for all $b \in B$, $\sigma (\mathfrak{p}) =\mathfrak{p}$. If for all $b \in B$, $\sigma(b)- b \in \mathfrak{p}^{s+1}  \, $ then 
$$\underline{J_m(\sigma)}|_{\underline{J_m(B)}_{B/\mathfrak{p}^{s-m+1}}} =\operatorname{id}_{\underline{J_m(B)}_{B/\mathfrak{p}^{s-m+1}} }$$
for all $m\leq s$.
\end{lemma}

\begin{proof}
Given an arbitrary $R-$algebra $C$ and $\psi\in \underline{J_m(B)}_\mathfrak{p}(C)$, we have that 
$$\psi(\mathfrak{p})\subseteq (t)+\left( \iota^C_m(\tau_{m,0}(\psi(\mathfrak{p}))) \right)  \, ,$$
therefore
$$\psi(\mathfrak{p}^{s+1})\subseteq \sum_{j=0}^{s+1} (t^j)\left( \iota^C_m(\tau_{m,0}(\psi(\mathfrak{p}^{s-j+1}))) \right) \, .$$

Clearly $\tau_{m,0}(\psi(\mathfrak{p}^{s-m+1}))=0$, therefore $\iota^C_m(\tau_{m,0}(\psi(\mathfrak{p}^{s-j+1})))=0$ for $j\leq m$, while for $j>m$ we have that $t^j=0$.
It follows that $\psi(\mathfrak{p}^{s+1})=0$.

Hence, for all $b\in B$ we have that
$$ \underline{J_m}(\sigma)(\psi)(b)= \psi(\sigma(b))= \psi(b)+ \psi(\sigma(b)-b)=\psi(b)  \, , $$
where the last equality follows from the assumption that $\forall b\in B$, $\sigma(b)-b\in \mathfrak{p}^{s+1}$.
\end{proof}

\luigi{This is the "other arrow" according to my promise in the file that i sent. The above thing implies that, given $\sigma\in G_s(p)$ then for all m, for all $q\in \Spec (L_m(B) \otimes k(p)) \subseteq \Spec (L_m(B) \otimes B/p^{s-m+1})$, then $L_m(\sigma)\in G_{s-m+1}(q)$.}

\begin{lemma}
\label{lem:redfibretoG1}
  Let $k$ be a field, $B$ be a local Noetherian $k$-algebra with maximal ideal $ \mathfrak{m}$, and $\sigma: B \rightarrow B$ be an automorphism of the $k$-algebra $B$ such that for all $b \in B$, $\sigma ( b) - b \in  \mathfrak{m}$. If $\mathcal{L}_1 (\sigma ) \otimes \operatorname{id}_{k(\mathfrak{m})}|_{ \mathcal{L}_1(B)_{ \mathfrak{m}, red}} = id_{ \mathcal{L}_1(B)_{ \mathfrak{m}, red}} $. Then for all $b \in B$, $\sigma (b)-b\in \mathfrak{m}^2$.  
\end{lemma}

\begin{proof} 
Assume that there is $b \in B$, $\sigma ( b) - b \in B \backslash  \mathfrak{m}^2$. We first note that we have $\sigma ( b) - b \in \mathfrak{m} \backslash  \mathfrak{m}^2$. Indeed, by assumption $\sigma ( b) - b \in \mathfrak{m}$. We will prove that $ \mathcal{L}_1(\sigma)|_{\mathcal{L}_1(B)_{ \mathfrak{m}, red}} \neq id_{ \mathcal{L}_1(B)_{ \mathfrak{m}, red}}$. \\
For this, it is enough to prove that there is $C$ reduced $k(\mathfrak{m})$-algebra and a $k(\mathfrak{m})$-algebra morphism $\Psi: B\rightarrow C[t]/(t^2)$ such that $\Psi^{-1} ((t)/ (t)^2)= \mathfrak{m}$, ${\tau}^B_{1,0} (\Psi(B \backslash \mathfrak{m}) ) \subseteq C^\times$ and $\Psi \circ \sigma \neq \Psi$. Given such $\Psi$, $\Psi  ( \mathfrak{m}^2) =0$, thus $\Psi$ descends to a morphism $\widetilde{\Psi}:  B/\mathfrak{m}^2\rightarrow C[t]/(t^2)$  such that $\widetilde{\Psi}^{-1} ( (t)/ (t)^2 ) = \mathfrak{m}/\mathfrak{m}^2$ and ${\tau}^B_{1,0}  (\widetilde{\Psi} ((B/\mathfrak{m}^2) \backslash (\mathfrak{m}/\mathfrak{m}^2)) ) \subseteq C^\times$. Conversely, given $\widetilde{\Psi} : B/ \mathfrak{m}^2 \rightarrow  C[t]/(t^2)$ such that $\widetilde{\Psi}^{-1} ( (t)/ (t)^2 ) = \mathfrak{m}/\mathfrak{m}^2$ and ${\tau}^B_{1,0}  (\widetilde{\Psi} ((B/\mathfrak{m}^2) \backslash (\mathfrak{m}/\mathfrak{m}^2)) ) \subseteq C^\times$, then there is $\Psi: B \rightarrow  C[t]/(t^2)$ such that $\Psi = \widetilde{\Psi} \circ \pi_{0, 2}$ where $\pi_{0, 2} : B \rightarrow  {B}/{ \mathfrak{m}^2}$ is the canonical quotient map. We have that the canonical projection map $\pi_{2, 1}: {B}/{ \mathfrak{m}^2} \rightarrow {B}/{ \mathfrak{m}}$ is not an isomorphism. Indeed, if $\pi_{2,1}$ is an isomorphism then $\mathfrak{m}=\mathfrak{m}^2$ and ${B}/{ \mathfrak{m}^2}= {B}/{ \mathfrak{m}}$. So, the action induced by $\sigma$ on ${B}/{ \mathfrak{m}^2}$ is trivial, but this contradicts our assumption. \\
By Cohen theorem (see \cite[Theorem 10.160.8]{stack}), since $B$ is noetherian, we have $B/ \mathfrak{m}^2$ noetherian and the $\mathfrak{m}$-adic completion of $\widehat{B/ \mathfrak{m}^2} \simeq B/ \mathfrak{m}^2$, we have that $B/ \mathfrak{m}^2$ is a $k(\mathfrak{m})$-vector space.
Since $\pi_s$ is not an isomorphism and $ \mathfrak{m}/\mathfrak{m}^2$ is a $k(\mathfrak{m})$-vector space,. We have the direct sum decomposition $B/ \mathfrak{m}^2= k( \mathfrak{m})\cdot 1 \oplus \mathfrak{m}/\mathfrak{m}^2$. Indeed, given $\alpha \in B/ \mathfrak{m}^2$, then $\alpha - \pi_{0, 1} ( \alpha) \cdot 1 \in  \mathfrak{m}/\mathfrak{m}^2.$ %Moreover, clearly we have the direct sum decomposition $ \mathfrak{m}/\mathfrak{m}^2 = k( \mathfrak{m}) \cdot (\sigma (b) -b) \oplus V(\mathfrak{m})$ for some $k( \mathfrak{m})$-subspace $V(\mathfrak{m})$. 
We choose $\mathcal{B}=\{ \sigma (b) -b , b_i \}_{i \in I}$ to be a base for $ \mathfrak{m}/\mathfrak{m}^2 $ over $k( \mathfrak{m})$. 
%there is some non-zero element $x_1, \cdots, x_r\in \mathfrak{p}$ that generates 
%then ${\mathfrak{p}}/{\mathfrak{p}^2}$ is a $k( \mathfrak{p})$-vector subspace of the $k( \mathfrak{p})$-vector space $B/ \mathfrak{p}^2$. So that, $\mathfrak{p}/\mathfrak{p}^2$ is a direct summand of $B/ \mathfrak{p}^2$. We write $B/ \mathfrak{p}^2=\mathfrak{p}/\mathfrak{p}^2 \oplus V( \mathfrak{p})$. 
We construct 
$$ \begin{array}{llll} \widetilde{\Psi}: &B / \mathfrak{m}^2 & \rightarrow & F[t]/ (t^2) \\
& b & \mapsto & \pi_{2, 1} ( b) + [t]_2 D( b)
\end{array}$$
where $D$ is the $k (\mathfrak{m})$-linear functional defined on the basis $\mathcal{B}$ as $D ( \sigma(b) -b)=1$ and $D (u_i)=0$ for all $i \in I$. 
We now prove that $ \widetilde{\Psi}$ is a $k(\mathfrak{m})$-algebra morphism. We already know that $\widetilde{\Psi}$ is a $k(\mathfrak{m})$-linear as a sum of two linear morphisms. Let $b, c \in B$. We write $b= b_0+ b_1$ and $c= c_0+ c_1$ where $b_0, c_1 \in k( \mathfrak{m})\cdot 1$ and $b_1, c_1\in \mathfrak{m}/ \mathfrak{m}^2$. We have
$$\widetilde{\Psi} ( bc )= \widetilde{\Psi} ( b_0c_0 + b_1c_0 + b_0c_1 + b_1c_1 )$$  but $b_1c_1\in \mathfrak{m}^2$, so $b_1c_1=0; $
Therefore, 
$$ \widetilde{\Psi}( bc ) = \widetilde{\Psi} (b_0c_0) +  \widetilde{\Psi}(b_1c_0) +  \widetilde{\Psi}(x_0y_1)$$
Since $b_0, c_0 \in k( \mathfrak{m})\cdot 1$,there are $\alpha, \beta\in k( \mathfrak{m})$ such that $b_0= \alpha \cdot 1$, $b_0= \beta \cdot 1$ implies 
then $b_0c_0= \alpha \beta \cdot 1\in k( \mathfrak{m})\cdot 1$, we have $ \widetilde{\Psi} (b_0c_0) = \pi_{2,1} (b_0c_0)=\pi_{2,1} (b_0)\pi_{2,1} (c_0) $. Moreover, since $b_1, c_1 \in \mathfrak{m}/ \mathfrak{m}^2$, and that $\pi_{2, 1}$ is a $k(\mathfrak{m})$-algebra morphism that vanishes in $\mathfrak{m}/ \mathfrak{m}^2$ while $D$ vanishes in $k( \mathfrak{m})\cdot 1$, we obtain 
$$\widetilde{\Psi}(b_1c_0) +  \widetilde{\Psi}(x_0y_1)= [t]_1 [D(b_1 c_0) + D(b_0c_1)]$$
So that, 
$$\widetilde{\Psi}( bc ) = \pi_{2,1} (b_0)\pi_{2,1} (c_0) + [t]_1 [\pi_{2,1} (c_0)D(b_1 ) + \pi_{2,1} (b_0)D(c_1)]$$
On the other hand, we have
$$\begin{array}{lll} \widetilde{\Psi}( b ) \widetilde{\Psi}( c )&=& (\pi_{2,1} (b)+ [t]_1 D(b) )(\pi_{2,1} (c)+ [t]_1 D(c) ) \\
&=&  \pi_{2,1} (b)\pi_{2,1} (c ) + [t]_1 [D(b) \pi_{2,1} (c)+ \pi_{2,1} (b) D(c ) ] \\
&=&  \pi_{2,1} (b_0) \pi_{2,1} (c_0) + [t]_1 [\pi_{2,1} (c_0) D(b_1)+ \pi_{2,1} (b_0)D(c_1)]
\end{array}$$
Thus, $\widetilde{\Psi}( bc )= \widetilde{\Psi}( b ) \widetilde{\Psi}( c )$.
We have $\widetilde{\Psi}^{-1} ( (t)/ (t)^2 ) = \mathfrak{m}/\mathfrak{m}^2$. since given $b \in B /\mathfrak{m}^2$, we have $\widetilde{\Psi} (b) \in(t)/ (t)^2$ if and only if $b \in \mathfrak{m}/\mathfrak{m}^2$. We also have that ${\tau}^B_{1,0} (\widetilde{\Psi} ((B/\mathfrak{m}^2) \backslash (\mathfrak{m}/\mathfrak{m}^2)) ) \subseteq F^*$, since ${\tau}^B_{1,0} \circ \widetilde{\Psi}= \pi_{2,1}$. Finally, $(\widetilde{\Psi}  \circ \sigma ) (b)- \widetilde{\Psi}  (b) = \widetilde{\Psi} ( \sigma ( b) -b ) = [t]_1 D (\sigma (b) -b)\neq 0$. Therefore, $\Psi \circ \sigma \neq \Psi$, it follows that $\mathcal{L}_1 (\sigma ) \otimes \operatorname{id}_{k(\mathfrak{m})} |_{ \mathcal{L}_1(B)_{ \mathfrak{m}, red}} \neq id_{ \mathcal{L}_1(B)_{ \mathfrak{m}, red}} $. 

\end{proof}

\begin{remark}
Combining Lemma \ref{lem:Gmtofibre} and Lemma \ref{lem:redfibretoG1} we have an interesting consequence on the characterization on the first ramification group of an action.
Let $(B, \mathfrak{p})$ be an algebra that satisfies the hypothesis of those lemmas and let $G$ be a group acting on them. On one hand, Lemma \ref{lem:Gmtofibre} says that $\forall \sigma\in G_1(\mathfrak{p})$, $\mathcal{L}_1(\sigma)$ is trivial on $\mathcal{L}_1(B)_{k(\mathfrak{p})}$, in particular $\forall \mathfrak{q}\in \Spec \mathcal{L}_1(B)_{k(\mathfrak{p})}$, $\sigma\in G_0(\mathfrak{q})$; therefore we have the inclusion $\displaystyle G_1(p)\subseteq \bigcap_{\mathfrak{q}\in \Spec \mathcal{L}_1(B)_{k(\mathfrak{p})} } G_0(\mathfrak{q})$.
On the other hand, if $\sigma\in G_0(\mathfrak{q})$ for all $\mathfrak{q}\in \Spec \mathcal{L}_1(B)_{k(\mathfrak{p})}$, then $\mathcal{L}_1(\sigma)$ is trivial on $\mathcal{L}(B)_{\mathfrak{p}, red}$, indeed for $x\in \mathcal{L}_1(B)_{k(\mathfrak{p})}$, we have that $\mathcal{L}_1(\sigma)(x) -x \in \sqrt{0}= \bigcap_{\mathfrak{q}\in \Spec \mathcal{L}_1(B)_{k(\mathfrak{p})} } \mathfrak{q}$; in other words this means that $\mathcal{L}_1(\sigma)|_{\mathcal{L}_1(B)_{k(\mathfrak{p})}/\sqrt{0}}= \mathbf{id}_{\mathcal{L}_1(B)_{k(\mathfrak{p})}/\sqrt{0}}$. It follows by Lemma \ref{lem:redfibretoG1} that $\sigma\in G_1(\mathfrak{p})$.
Therefore we have an equality
$$ G_1(\mathfrak{p}) = \bigcap_{\mathfrak{q}\in \Spec \mathcal{L}_1(B)_{k(\mathfrak{p})} } G_0(\mathfrak{q}) \, . $$

\luigi{If $\mathcal{L}_1(B)_{k(\mathfrak{p})}$ is of finite type over $k(\mathfrak{p})$ (which happens whenever $B$ is finitely generated/$k$, or, more generally, should happen when $B_\mathfrak{p}$ is Noetherian, due to Cohen), then Jacobson = $\sqrt{0}$, so in the equality above we can only consider the maximal spectrum. This is useful for the existence of some functors. The hypotesis of $B$ being of finite type over $k$ is very mild in alg.geom.}
\end{remark}







\begin{exmp} \begin{enumerate}
\item Let $B=k[x]/ (x^2-y)^2$. We consider $\sigma : B \rightarrow B$ sending $ [x]$ to $ [x+ (x^2 -y) x]$. It is an involution $\sigma^2 ([x]) = \sigma ( [x+ (x^2 -y) x]) = [x+ (x^2 -y) x +  (x^2 -y) x]=[x]$. 
\begin{enumerate} 
\item Suppose that $k =\mathbb{F}_2(y)$ and set $\mathfrak{p}:= \frac{ (x^2-y)}{(x^2-y)^2}$. We have that $\sigma ( [x]) -  [x])\notin \mathfrak{p}^2$. We have $\mathcal{L}_1(\sigma)_{k ( \mathfrak{p})}  ([x_0]) = [x_0]$ and $\mathcal{L}_1(\sigma)_{k ( \mathfrak{p})}  ([x_1]) = [x_1]$. 
\item Suppose that $k =\mathbb{F}_2(y)[z]/(y^2-z)$ where $z= y^2$. Let $\mathfrak{m}= \frac{ (x-z)}{(x^2-y)^2}$ be a maximal ideal containing $\mathfrak{p}:= \frac{ (x^2-y)}{(x^2-y)^2}$. $\sigma ( [x]) -  [x] \in \mathfrak{m}^2$. We have $\mathcal{L}_1(\sigma)_{k ( \mathfrak{p})}  ([x_0]) = [x_0]$ and $\mathcal{L}_1(\sigma)_{k ( \mathfrak{p})}  ([x_1]) = [x_1]$.
\end{enumerate} 
Let $B=k[x,z]$. $(z-a) \in Spec (B)$. 
\item  $B=k[x,y]/ (x^2y-z^2)^2$. We consider $\sigma : B \rightarrow B$ sending $ [x]$ to $ [x+ (x^2y -z)^2 x]$ and $[y]$ to $[y]$. It is an involution $\sigma^2 ([x]) = \sigma ( [x+ (x^2y -z)^2 x]) = [x+ (x^2 y-z)^2 x +  (x^2y -z)^2 x]=[x]$. We have that $\sigma ( [x]) -  [x])\notin \mathfrak{p}^3$. We have $\mathcal{L}_1(\sigma)_{k ( \mathfrak{p})}  ([x_0]) = [x_0]$ and $\mathcal{L}_1(\sigma)_{k ( \mathfrak{p})}  ([x_1]) = [x_1]$. 

$$\begin{array}{ccc} && [x_0 + x_1[t]+ ((x_0 + x_1[t])^2(y_0 + y_1[t]) -z) (x_0 + x_1[t])]\\
&=& [x_0 + x_1[t]+ (x_0^2(y_0 + y_1[t]) -z) (x_0 + x_1[t])]\\
&=& [x_0 + x_1[t]+ (x_0^2y_0  -z + x_0^2 y_1[t]) (x_0 + x_1[t])]\\
&=& 	[x_0 + (x_0^2y_0  -z) x_0 + (x_1+ (x_0^2y_0  -z)x_1+ x_0^3 y_1)[t]]
\end{array}
$$

$$\begin{array}{ccc} && [x_0 + x_1[t]+ ((x_0 + x_1[t])^2(y_0 + y_1[t]) -z) (x_0 + x_1[t])]\\
&=& [x_0 + x_1[t]+ (x_0^2(y_0 + y_1[t]) -z)^2 (x_0 + x_1[t])]\\
&=& [x_0 + x_1[t]+ (x_0^2y_0  -z + x_0^2 y_1[t])^2 (x_0 + x_1[t])]\\
&=& 	[x_0 + x_1[t]+ (x_0^2y_0  -z)^2 (x_0 + x_1[t])]\\
\end{array}
$$ 
\end{enumerate} 
\end{exmp} 

\begin{lemma} 
 Let $B = k \oplus (\oplus_{i=1}^r x_i k) \oplus ( \oplus_{1\leq i\leq j \leq r} x_i \cdot x_j  k/ \mathbf{L})$ where $\mathbf{L}$ is a linear subspace of $\oplus_{1\leq i\leq j \leq r} x_i \cdot x_j k$. Let $\sigma : B \rightarrow B$ be an automorphism of $k$-algebras such that $ \sigma( x_i) - x_i = \sum_{1\leq j \leq l \leq r } h_{jl}^i \cdot x_j x_l$ for all $i\in \{ 1, \cdots, r\}$ and assume that there is $i_0 \in \{ 1, \cdots, r\}$ such that $ \sum_{1\leq j \leq l \leq r } h_{jl}^{i_0} \cdot x_j x_l \neq 0$. (In other words, $\sigma \in G_1 ( (\overline{x} )) \backslash G_2 (( \overline{x}) )$. 
 Then there exists $\mathfrak{q} \in \operatorname{Spec} ( \mathcal{L}_1(B) \otimes_B B/ \mathfrak{m})$, there exists $\alpha \in \mathcal{L}_1(B)$ such that $ \mathcal{L}_1(B) (\alpha) - \alpha \notin \mathfrak{q}^2$ (In other words, $ \mathcal{L}_1(\sigma) \notin G_1 (\mathfrak{q})$), .  
 

 \end{lemma}
 
 
 
\newpage
\begin{definition}
For any $M$ $A$-module , we define $Sym(M)$ to be the quotient of the tensor algebra of $M$ denoted $T(M)$ by the two-sided ideal $\mathfrak{I}$ generated by the elements $x y - y x $ of $T(M)$, where $x , y $ run through $M$. 
We recall that $T(M)= \oplus_{n \in \mathbb{N}} T^n ( M)$ where $T^0(M)= A$, $T^n (M) = M\otimes \cdots \otimes M$ $n$ times, for any $n \in \mathbb{N}$.  

\luigi{Here I am a bit confused and need to think about the changes that could be made in this definition: what is the product that gives the algebra structure in T(M), the shuffle product? Or a non-commutative product that simply puts two elementary tensors next to each other?  In the first case, I think that quotienting with respect to that ideal is not enough (e.g. in char 2), in the second case I really don't know what to do, but maybe in that case it is correct. Could you send me the link to Manin's work on tensor algebras?  Another option could be to forget of the tensor algebra and define the symmetric algebra via universal property.}
\end{definition} 


\sophie{define $\eta (\mathfrak{p})$. and intersection of $G_s (\mathfrak{p})$. primary ideal. }
\begin{lemma}\label{sym}
Let $B$ and $C$ be $R$-algebra. 
We have 
$$\begin{array}{clll} Hom_{ \mathbf{Alg}_R} \left( B ,  C[t]/(t^2) \right)& \simeq &Hom_{ \mathbf{Alg}_R}( Sym ( \Omega^1_{B/R}), C) \\
&\simeq&  \{ (f, D) | f: B \rightarrow C \in Hom_{ \mathbf{Alg}_R} ( B, C) , D \in Der_R( B , C) \}\end{array}
.$$
In particular, we have $ \mathcal{L}_1 ( B) \simeq Sym^* ( \Omega^1_{B/R})$ as $R$-algebras and $ \mathcal{L}_1 ( B)_{k(\mathfrak{p})} / (\underline{x}_1)^2_{k(\mathfrak{p})} \simeq  k(\mathfrak{p}) \oplus \Omega^1_{B/R}\otimes_B k(\mathfrak{p})$ as $R$-modules.  
\end{lemma}
\begin{proof}
Let $ \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})=  \{ (f, D) | f: B \rightarrow C \in Hom_{ \mathbf{Alg}_R} ( B, C) , D \in Der_R( B , C) \}$.
We start by proving that 
$$Hom_{ \mathbf{Alg}_R} \left( B ,C[t]/(t^2) \right) \simeq   \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p}).$$
Let $g \in Hom_{ \mathbf{Alg}_R} \left( B , C[t]/(t^2) \right)$ we have $g(b) = f_g(b) + \bar{t} D_g(b)$ for some map $f_g: B \rightarrow C$ and $D_g : B \rightarrow C$. Since $g$ and $f_g$ are $R$-linear, so are $f_g$ and $D_g$. Now, since $g$ is a ring morphism, we also have that for all $a,b \in B$, we have $g(ab) = g(a) g(b)$. That is $f_g(ab) + \bar{t} D_g(ab)= (f_g(a) + \bar{t} D_g(a))(f_g(b) + \bar{t} D_g(b))= f_g(a) f_g(b) + \bar{t} (D_g(a) f_g(b) + f_g(a) D_g(b))$. As a consequence, $f_g$ is a $R$-algebra morphism and $D_g: B \rightarrow C$ is a $R$-derivation with respect to the structure of $B$-module on $C$ given by $f_g: B \rightarrow C$. Conversely, given a pair $(f, D)$ such that $f : B \rightarrow C \in Hom_{ \mathbf{Alg}_R} ( B, C)$ and $D \in Der_{R}( B , C)$. We define the map $g_{(f, D)}: B \rightarrow  C[t]/(t^2)$, such that $g_{(f, D)}(b) = f(b) + \bar{t} D(b)$. Using the above computations, we prove that $g_{(f, D)}\in Hom_{ \mathbf{Alg}_R} \left( B , C[t]/(t^2) \right)$.  This defines a bijective map $\Phi$ from $Hom_{ \mathbf{Alg}_R} \left( B ,C[t]/(t^2) \right)$ to $ \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})$ sending $g$ to $(f_g, D_g)$ whose inverse send $(f, D)$ to $g_{(f,D)}$.\\
It remains to prove that 
$$Hom_{ \mathbf{Alg}_R}( Sym ( \Omega^1_{B/R}), C)  \simeq  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p}) $$
Let $d : B\rightarrow \Omega^1_{B/R}$ be a $B$-derivation. 
Given a morphism $g :  Sym ( \Omega^1_{B/R}) \rightarrow C$.  We denote $\iota_1: B \rightarrow Sym ( \Omega^1_{B/R}) $ and $\iota_2:  \Omega^1_{B/R} \rightarrow Sym ( \Omega^1_{B/R}) $ to be the canonical injection. We prove that $(\tilde{f}_g, \tilde{D}_g)\in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})$ where $\tilde{f}_g= g \circ \iota_1$ and $\tilde{D}_g= g \circ \iota_2\circ d $. Since $g$, $\iota_1$ and $\iota_2$ are $R$-linear so are $f$ and $\tilde{D}_g$. Since $g$ is a ring map we have $\tilde{f}_g(ab)= \tilde{f}_g(a) \tilde{f}_g(b)$ and $g \circ \iota_2( a c) = g( ac) = \tilde{f}_g(a) g(c)$, for all $a,b \in B$ and $c\in  \Omega^1_{B/R}$. Thus, $(\tilde{f}_g, \tilde{D}_g) \in   \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})$. Conversely, let $(f, D)\in \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})$, by the universal property of $\Omega^1_{B/R}$, there is a $R$-linear map $h : \Omega^1_{B/R}\rightarrow C$ such that $ D = h \circ d$ (see \cite[Definition 1.2]{Qing} ). Now, using the universal property of $ Sym ( \Omega^1_{B/R})$ (see \cite[\S 6.1, Proposition 1]{NB} ), we obtain a $B$-algebra homomorphism $\tilde{g}_{(f,D)}:  Sym ( \Omega^1_{B/R}) \rightarrow C$ such that $h= \tilde{g}_{(f,D)} \circ \iota_2$. This defines a bijective map $\Psi_d$ from $Hom_{ \mathbf{Alg}_R}( Sym ( \Omega^1_{B/R}), C)$ to $  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})$ sending $g$ to $(\tilde{f}_g, \tilde{D}_g)$ whose inverse send $(f, D)$ to $\tilde{g}_{(f,D)}$. We have that $ {\epsilon_m}_C^B\circ \Phi^{-1} \circ \Psi_d$
is a bijective map from $Hom_{ \mathbf{Alg}_R}( Sym ( \Omega^1_{B/R}), C)$ to $Hom_{ \mathbf{Alg}_R} \left( \mathcal{L}_1 ( B) , C \right)$. 

%We obtain that $\Psi_d^{-1} \circ \Phi \circ {\eta_m}_{\mathcal{L}_1(B)}^B(Id_{ \mathcal{L}_1(B)})$ is an $R$-algebra isomorphism from  $Sym^* ( \Omega^1_{B/R})$ to $ \mathcal{L}_1 ( B)$.  We have 
%$$\Psi_d^{-1} \circ \Phi \circ {\eta_m}_{\mathcal{L}_1(B)}^B(Id_{ \mathcal{L}_1(B)})={\epsilon_m}_{Sym ( \Omega^1_{B/R})}^B (g_{(Id_B , d)} )$$
%%We recall that $g_{(Id_B , d)} (b) = b + d(b) \bar{t}$, for all $b \in B$ and 
%We recall $ {\eta_m^B}_C(Id_{ \mathcal{L}_1(B)}) : B  \rightarrow \mathcal{L}_1(B) [t]/ (t^{m+1})$ sending $[x_i]_{I}$ to $\sum_{j=0}^m [x_{i,j}]_{\mathcal{L}_m(I)} [t]_m^j$, for all $i \in \{ 1, \cdots, n\}$. 
%Thus $\Phi \circ {\eta_m}_{\mathcal{L}_1(B)}^B(Id_{ \mathcal{L}_1(B)})= (f, D)$ where $f: B \rightarrow  \mathcal{L}_1(B)$ and $d: B \rightarrow  \mathcal{L}_1(B)$. 
%
%We have $ {\epsilon_m^B}_C(g_{(Id_B , d)}) : \mathcal{L}_m(B) \rightarrow Sym^* ( \Omega^1_{B/R}) $ sending $[x_{i,0}]_{\mathcal{L}_m(I)}$ to $ [x_i]_I$ and $[x_{i,1}]_{\mathcal{L}_m(I)}$ to $d( [x_i]_I)$. 

We obtain that $\Theta:= {\epsilon_m}_{Sym ( \Omega^1_{B/R})}^B\circ \Phi^{-1} \circ \Psi_d (Id_{ Sym ( \Omega^1_{B/R})})$ is an $R$-algebra isomorphism from $ \mathcal{L}_1 ( B)$ to $Sym^* ( \Omega^1_{B/R})$.  We have 
$$\Theta= {\epsilon_m}_{Sym ( \Omega^1_{B/R})}^B\circ \Phi^{-1} \circ \Psi_d (Id_{ Sym ( \Omega^1_{B/R})})={\epsilon_m}_{Sym ( \Omega^1_{B/R})}^B (g_{(\iota_1 , \iota_2 \circ d)} )$$
%We recall that $g_{(Id_B , d)} (b) = b + d(b) \bar{t}$, for all $b \in B$ and 
We have $\Theta : \mathcal{L}_m(B) \rightarrow Sym^* ( \Omega^1_{B/R}) $ sending $[x_{i,0}]_{\mathcal{L}_m(I)}$ to $ \iota_1 ([x_i]_I)$ and $[x_{i,1}]_{\mathcal{L}_m(I)}$ to $\iota_2 (d( [x_i]_I))$. 
Therefore, $\Theta_{k(\mathfrak{p})} ( (\underline{x}_1)^2_{k(\mathfrak{p})} ) = \frac{\oplus_{n\geq 2} T^n ( \Omega^1_{B/R})}{\mathfrak{I}\cap \oplus_{n\geq 2} T^n ( \Omega^1_{B/R})} $ leading to the isomorphism $ \mathcal{L}_1 ( B)_{k(\mathfrak{p})} / (\underline{x}_1)^2_{k(\mathfrak{p})} \simeq  k(\mathfrak{p}) \oplus \Omega^1_{B/R}\otimes_B k(\mathfrak{p})$ as $R$-modules.  
\end{proof} 
\begin{lemma} \label{derfinsep}
Given $k \subseteq F \subseteq L$ fields, with $L/F$ finite separable. Given $C$ $F$-vector space. Given $D$ in $Der_k(F, C)$, then exists a unique $\widetilde{D}$ in $Der_k(L, C)$ that extends $D$.
\end{lemma} 

\begin{proof} 
Since $L/F$ is finite separable, there exists a $y\in L$ such that $F(y)= L$ and its minimal polynomial $p(x)$ is separable. We write $p(x) = \sum_{i=0}^r a_i x^i$. We have $p(y) =  \sum_{i=0}^r a_i y^i=0$. We want to extend $\overline{D}$ to a derivation $\widetilde{D} \in Der_k ( L, C)$.  If such $\widetilde{D} $ exists, 
$\widetilde{D}  (p(y) ) =0$. That is $p'(y) \widetilde{D} (y) =0 $. Since $p(x)$ is separable, $p'(y)\neq 0$ and $\widetilde{D} (y)=0$. Also setting $\widetilde{D}= \overline{D}$ over $F$ and $\widetilde{D} (y)=0$ defines a derivation. 
%We set $ \Phi_C (D) := \widetilde{D}$. 
%We also define 
%$$\begin{array}{rrll} \Psi_C :& ( k(\mathfrak{p}), C) & \rightarrow  &Der_k ( k[T], C)\\
%& D & \mapsto & \Psi_C( D)
%\end{array}$$
%where $ \Psi_C (D) $ is defined as follows. Using the same notation and reasoning as above, we can prove that $D(y)=0$. Thus we can set $\overline{D}$ to be the restriction of $D$ to $k(T)$ correstricted to $k(T)$ and $\Psi_C( D) (b)= \overline{D}\left( \frac{b}{1}\right)$, for all $b \in k[T]$. 
%Clearly $\Phi_C$ and $\Psi_C$ are inverse of each others.
\end{proof} 

\begin{corollary}  \label{tr} 
Given $k \subseteq F \subseteq L$ fields, with $L/F$ finite separable and $F= k(T)$ where $T$ is a transcendence basis for $F$ over $k$. Given $C$ $F$-vector space. Given $D$ in $Der_k(k[T], C)$, then exists a unique $\widetilde{D}$ in $Der_k(L, C)$ that extends $D$. In particular, any derivation $D$ in $Der_k ( L, C)$ where $C$ is a $F$-algebra is uniquely determined by its images of $t$, for any $t \in T$ that can be chosen arbitrarily and $dim_k (Der_k ( L, C))= |T| = \operatorname{tr}(L/k)$. 
\end{corollary} 
\begin{proof}
We know that a derivation $D$ in $Der_k ( k[T], C)$ is uniquely determined by the image of $t$, for any $t \in T$ that can be chosen arbitrarily (see for instance, \cite[Example 1.6]{Qing}). Moreover, by Lemma \ref{locder}, $D$ can be uniquely extended to a derivation $\overline{D}$ in  $Der_k ( k(T), C)$. The result is then a consequence of Lemma \ref{derfinsep}
\end{proof} 

\begin{definition}(Lemma)
Let $k$ be a field and $F$ be a finitely generated field extension over $k$ where $char(k)=p>0$. Let $E= kF^p$ be the compositum of $k$ and $F^p$ in $F$. We have $[F:E]=p^e$ where $e\in \mathbb{N}$. We have $F=E(x_1 , \cdots , x_e)$ where $x_i^p =t_i\in E$ for all $i \in \{ 1, \cdots, e\}$,  and $[E(x_1 , \cdots, x_{i} ) : E(x_1, \cdots , x_{i-1})]=p$, for all $i \in \{ 2, \cdots, e\}$. For any $C$ $F$-module
$$Der_k(F, C) = C^e.$$ Equivalently, $\Omega^1_{F/k} \simeq F^e$. 
\end{definition} 
\begin{proof}
We know by definition of $E$ that every element $z\in E$ is such that $z^p \in E$. Therefore $F$ is algebraic over $E$ and since it is finitely generated, $[F:E]=p^e$, for some $e \in \mathbb{N}$. Using induction on $e$, one can prove without difficulty that $F=E(x_1 , \cdots , x_e)$ where $x_i^p =t_i\in E$ for all $i \in \{ 1, \cdots, e\}$,  and $[E(x_1 , \cdots, x_{i} ) : E(x_1, \cdots , x_{i-1})]=p$, for all $i \in \{ 2, \cdots, e\}$. Now, let $C$ be a $F$-module and $D \in Der_k(F, C)$, we have $D|_{F^p} \equiv 0$. Indeed, for all $x\in F^p$, there is $a \in F$ such that $x=a^p$. Thus $D(a^p) = p \cdot a^{p-1}  \cdot D(a) =0$. Thus, since $D|_k\equiv 0$, $D_E \equiv 0$. 
So that the map 
$$\begin{array}{lrll} \Phi : & Der_k(F, C) & \rightarrow & C^e \\ 
& D & \mapsto & (D(x_i))_{i \in \{ 1, \cdots, e\}} \end{array}$$
is bijective. 
%Then it suffice to set $D(x_i)= c_i $ where $c_i \in C$ for all $i \in \{ 1, \cdots, e\}$ to determine uniquely a derivation and any derivation are obtained like this. This proves that  $Der_k(F, C) = C^e,$ as required.
\end{proof} 

\begin{lemma}\label{graded} Let $B$ be algebra over $k$ and $\mathfrak{p}$ be a prime ideal of $B$ such that $k(\mathfrak{p})$ is separably generated over $k$. 
Then there exists a section to the canonical morphism $\pi_{2,1, \mathfrak{p}} : N_2(\mathfrak{p}) \rightarrow k( \mathfrak{p})$ and $N_2 (\mathfrak{p}) \simeq k(\mathfrak{p}) \oplus \mathfrak{p}_\mathfrak{p} / \mathfrak{p}^2_\mathfrak{p} $ as algebra. %where $Gr(N_n (\mathfrak{p})) = k(\mathfrak{p}) \oplus \mathfrak{p}_\mathfrak{p} / \mathfrak{p}^2_\mathfrak{p} \oplus \cdots \oplus \mathfrak{p}^{n-1}_\mathfrak{p} / \mathfrak{p}^n_\mathfrak{p}$, for all $n \in \mathbb{N}$.\sophie{define associated graded algebra}
\end{lemma} 
\begin{proof} 
If $k(\mathfrak{p})$ is separably generated over $k$ then $k(\mathfrak{p})$ is formally smooth over $k$ (see for instance \cite[Lemma 10.158.8.]{Stack}). Therefore by definition of formal smoothness, 
%we can prove by induction on $n$ that there is a section $\phi_ n : k(\mathfrak{p}) \rightarrow N_n ( \mathfrak{p})$ to the canonical morphism $\pi_{n,1, \mathfrak{p}} : N_n(\mathfrak{p}) \rightarrow k( \mathfrak{p})$ and $N_n (\mathfrak{p}) \simeq Gr(N_n (\mathfrak{p}) )$. For $n=1$ the results is trivial. We suppose that the result is true for $n-1$ and we want to prove it remains to be true for $n$. 
By definition of formal smoothness of $k(\mathfrak{p})$ over $k$, we know there is a a morphism $\psi :  k(\mathfrak{p}) \rightarrow N_2(\mathfrak{p})$ making the following diagram 
$$\xymatrix{ k(\mathfrak{p}) & \ar[l] N_{2}(\mathfrak{p})\\
k(\mathfrak{p} ) \ar[ru]^\psi \ar[u]^{id}  & \ar[l] k \ar[u]  } $$ 
commute. %where $\phi_{n-1}: k( \mathfrak{p}) \rightarrow N_{n-1} (\mathfrak{p}) $ is the section given by the induction hypothesis. 
This proves the existence of the section and that $N_2(\mathfrak{p}) \simeq  k(\mathfrak{p} ) \oplus \mathfrak{p}_\mathfrak{p} / \mathfrak{p}^2_\mathfrak{p}$. %From the induction hypothesis we also deduce that $N_n(\mathfrak{p})\simeq Gr(N_n (\mathfrak{p}))$. This concludes the proof of the Lemma.  
\end{proof} 
%\begin{lemma} 
%Let $B$ be algebra over $k$ and $\mathfrak{p}$ be a prime ideal of $B$ such that $k(\mathfrak{p})$ is separably generated over $k$. $$\xymatrix{ 0 \ar[r]& \mathfrak{p}^{n}_\mathfrak{p} / \mathfrak{p}^{n+1}_\mathfrak{p} \ar[r] & \Omega^1_{ N_{n+1}( \mathfrak{p})/k} \otimes_{N_{n+1}( \mathfrak{p})} N_{n}(\mathfrak{p})  \ar[r]& \Omega^1_{ N_{n} ( \mathfrak{p})/k} \ar[r]& 0 }$$
%splits for every $n \in \mathbb{N}$. 
%\end{lemma} 
\begin{lemma} \label{irreduc}
Let $B$ be algebra over $k$ and $\mathfrak{p}$ be a prime ideal of $B$ such that $k(\mathfrak{p})$ is separably generated over $k$.   Then %$\mathcal{L}_1 (B) \otimes_B B/\mathfrak{p}$ is irreducible. In particular, 
$\mathcal{L}_1 (B) \otimes_B  k ( \mathfrak{p})  \simeq F_{d+t} ( k ( \mathfrak{p}))$ where $d=dim_{k(\mathfrak{p})}(\mathfrak{p}_\mathfrak{p} / \mathfrak{p}^2_\mathfrak{p})$ and $t= tr(k ( \mathfrak{p}) /k)$ for all $n\in \mathbb{N}$.  In particular, we have $\mathcal{L}_1 (B) \otimes_B  k ( \mathfrak{p}) $ is irreducible and $\mu^B_{0,1}(\mathfrak{p})$  is a prime ideal of $\mathcal{L}_1 (B)$. %and we have a bijection between the maximal ideal of $B$ and those $\mathcal{L}_1 (B)$ given by the map sending a maximal ideal $\mathfrak{m}$ of $B$ to $\mu^B_{0,1}(\mathfrak{p})$ whose inverse sends $\mathfrak{P}$ to ${\mu^B_{0,1}}^{-1}  (\mathfrak{P})$. 
%is a free $k ( \mathfrak{p})$-algebra. In particular, it is irreducible.
\end{lemma} 
\begin{proof} Let $C$ be a $k ( \mathfrak{p})$-algebra. We denote $f : k ( \mathfrak{p}) \rightarrow C $ the structural $k ( \mathfrak{p})$-algebra map. %turning $C$ into $k ( \mathfrak{p})$-algebra and 
%$\pi_\mathfrak{p} : B_\mathfrak{p} \rightarrow B_\mathfrak{p}/ \mathfrak{p}_{\mathfrak{p}}$. 
%We have $\mathcal{L}_1 (B) \otimes_B B/\mathfrak{p} (C)=\{ \psi :B \rightarrow \}  $
%We want to prove that $\mathcal{L}_1 (B) \otimes_B k ( \mathfrak{p})$ is a free algebra. To do that we prove that there is $r\in \mathbb{N}$ such that 
%$$Hom_{k ( \mathfrak{p})} ( \mathcal{L}_1 (B) \otimes_B k ( \mathfrak{p})  , C ) = C^r.$$ 
By Lemma \ref{Nsp}, we have 
$$Hom_{N_{2} (\mathfrak{p}) } ( \mathcal{L}_1 (B) \otimes_B k(\mathfrak{p})  , C ) \simeq  Der_{k} ( N_{2} (\mathfrak{p})   , C)  .$$
%$$\begin{array}{lll} && Hom_{k ( \mathfrak{p})} ( \mathcal{L}_1 (B) \otimes_B k ( \mathfrak{p}) , C ) \\
%&\simeq&  \{\psi \in \operatorname{Hom}_k(B, C[t]/(t^{2}))  \colon  p_1^B \circ \psi= f \circ \zeta_{\mathfrak{p}}  \} \\
%%p_s^B ( \psi (B \backslash \mathfrak{p}) ) \subseteq C^\times
%&\simeq &\{  \psi\in \operatorname{Hom}_k(B_\mathfrak{p}, C[t]/(t^{2})): \psi ( b) = \psi_0 (b) + [t] \psi_1(b), \  \psi_0 = f \circ \pi_\mathfrak{p} \}\\
%&\simeq& \{ \widetilde{\psi} \in \operatorname{Hom}_k(B_\mathfrak{p}/ \mathfrak{p}^2 , C[t]/(t^{2})):   \widetilde{\psi} ( b) = \widetilde{\psi}_0 (b) + [t]  \widetilde{\psi}_1(b), \   \widetilde{\psi}_0 = f \circ \pi_{2, \mathfrak{p}}  \}\\
%&\simeq& Der_{k} ( B_\mathfrak{p}/ \mathfrak{p}^2  , C)  
%\end{array}
% $$
By Lemma \ref{graded}, since $k(\mathfrak{p})/k$ is separably generated, we have $N_2 (\mathfrak{p}) \simeq  k(\mathfrak{p}) \oplus \mathfrak{p}_\mathfrak{p} / \mathfrak{p}^2_\mathfrak{p}$. %\oplus \cdots \oplus \mathfrak{p}^{n-1}_\mathfrak{p} / \mathfrak{p}^n_\mathfrak{p}$. 
%We now prove the result by induction on $n$. 
%For $n=1$, we have by the universal property of the derivation we have 
%$$Hom_{N_2( \mathfrak{p})} ( \Omega_{N_2( \mathfrak{p})/k} , C) \simeq Der_k (N_2( \mathfrak{p}) , C) .$$
%Moreover we have, for any $C$ $N_2(\mathfrak{p})$-module
%$$ Hom_{N_2( \mathfrak{p})} ( \Omega_{N_2( \mathfrak{p})/k} \otimes_B k(\mathfrak{p}), C)\simeq Hom_{N_2( \mathfrak{p})} ( \Omega_{N_2( \mathfrak{p})/k} , C).$$ 
%We prove the result for $n=1$. 
%Since from the above $N_2 (\mathfrak{p}) \simeq  k(\mathfrak{p}) \oplus \mathfrak{p}_\mathfrak{p} / \mathfrak{p}^2_\mathfrak{p}$,
By \cite[Theorem 58 (The second fundamental exact sequence)]{Matsumura}, we know that 
the following exact sequence 
\begin{equation} \label{seq} \xymatrix{ 0 \ar[r]& \mathfrak{p}_\mathfrak{p} / \mathfrak{p}^2_\mathfrak{p} \ar[r] & \Omega^1_{ N_2( \mathfrak{p})/k} \otimes_{N_2( \mathfrak{p})} k(\mathfrak{p})  \ar[r]& \Omega^1_{ k ( \mathfrak{p})/k} \ar[r]& 0 }
\end{equation}
splits. 
Moreover, since $ \Omega^1_{ k ( \mathfrak{p})/k}\simeq k ( \mathfrak{p})^t$, by Corollary \ref{tr} and $\mathfrak{p}_\mathfrak{p} / \mathfrak{p}^2_\mathfrak{p}\simeq k ( \mathfrak{p})^{d}$ by definition of $d$. 

Therefore, noting that $C$ has a natural structure of $N_2 (\mathfrak{p})$-algebra via the canonical map $\pi_{2,1, \mathfrak{p}}$. 
$$\begin{array}{lll} Hom_{k (\mathfrak{p}) } ( \mathcal{L}_1 (B) \otimes_B k (\mathfrak{p})  , C )&\simeq &Der_k (N_2( \mathfrak{p}) , C) \\
&  \simeq& Hom_{N_2( \mathfrak{p})} ( \Omega_{N_2( \mathfrak{p})/k} \otimes_{N_2(\mathfrak{p})} k(\mathfrak{p}), C)\simeq C^{t+ d_2}\end{array} $$
and $  \mathcal{L}_1 (B) \otimes_B k (\mathfrak{p})\simeq  F_{d+t} ( k ( \mathfrak{p}))$. 

Noting that $\mathcal{L}_1(B) \otimes_B k(\mathfrak{p}) \simeq \mathcal{L}_1(B)/\mu_{0,1}^B (\mathfrak{p})$. By the above, we know that $\mathcal{L}_1(B) \otimes_B k(\mathfrak{p})$ is an integral domain. So that $\mu_{0,1}^B (\mathfrak{p})$ is a prime ideal of $ \mathcal{L}_1(B)$.

%This proves the initialisation step for the induction. 
%Now we suppose that the result is true for $n-1$ and we prove the result remains true for $n$. Since the sequence \ref{seq} split, by \cite[Theorem 63]{Matsumura}, we know that the canonical map $$\xymatrix{ 0 \ar[r]& \mathfrak{p}^{n-1}_\mathfrak{p} / \mathfrak{p}^n_\mathfrak{p} \ar[r] & \Omega^1_{ N_n( \mathfrak{p})/k} \otimes_{N_n( \mathfrak{p})} N_{n-1}(\mathfrak{p})  \ar[r]& \Omega^1_{ N_{n-1} ( \mathfrak{p})/k} \ar[r]& 0 }$$splits.


% Let $\mathcal{B}= \{ b_1 , \cdots, b_n\}$ be a basis for $\mathfrak{p}/\mathfrak{p}^2$ as a $k ( \mathfrak{p})$-vector space.  \sophie{justification of map from $k (\mathfrak{p})$ to $B_\mathfrak{p}/ \mathfrak{p}^2$. }
% \sophie{We have $\mathfrak{p}/\mathfrak{p}^2= < a_1 , \cdot , a_n >$  as a $k ( \mathfrak{p})$-vector space. Choosing $\psi_1 ( a_i)$ determine the map. 
% $\psi_1$ is a $k$-linear derivation. $\tilde{\psi}$ defined over $\mathfrak{p}^2$ is zero is that enough to prove that it is for saying it is a $k(\mathfrak{p})$-linear map?  $K(\mathfrak{p}) / k(t_1, t_2, \cdots , t_s)$ finite separable is important. $D: k(t_1, \cdot , t_s) \rightarrow C$ is determined by an arbitrary choice of $D(t_i)$. Use that derivation on a ring and derivation on fraction field are in bijection. plus use that derivation on polynomial ring are generated by $dx_i$. By the primitive element theorem $k( \mathfrak{p})= k(t_1, \cdots , t_s) [x]/ (f)$, $f(x) = x^n + c_1 x^{n-1}+ \cdots + c_n$. Let $y$ be the generator of the field extension. $y^n + c_1 y^{n-1}+ \cdots + c_n=0$
%   $\tilde{D}  (y^n + c_1 y^{n-1}+ \cdots + c_n) =0$, $\tilde{D}  (y) f'(y) + d=0$. 
% this prove that $\tilde{D}$ is unique.  Prove that the extension of $\tilde{D}$ is well defined. 
% $ Der_{k} ( B_\mathfrak{p}/ \mathfrak{p} , C)  = Der_{k} (k(\mathfrak{p}) , C)$. 
%  
%  we want to extend $D$ to $\tilde{D}$, $\tilde{D}( f(x))=0$ is linear in $y$ $\tilde{D} (x) = y \in C$. $D$ can be extended uniquely to $\tilde{D}: k(\mathfrak{p}) \rightarrow C$
%So that $Hom_{k ( \mathfrak{p})} ( \mathcal{L}_1 (B) \otimes_B k ( \mathfrak{p}) , C ) \simeq C^{r+s}$. free implies irreducibility. $A$ is domain then $A[x]$ is domain. 
%} 
\end{proof} 

\sophie{ looking at the closed point equivalent to prime equivalent to generic point} 



\begin{definition} (Lemma) \label{locder}
 Let $B$ be a finitely presented algebra over $k$, we write $B= k[x_1, \cdots, x_n]/ I$. 
\begin{enumerate}
\item We denote $\widehat{B_{\mathfrak{p}}}$ be the $\mathfrak{p}$-adic completion of $B$ where $\mathfrak{p}$ is a prime ideal. 
\item We denote $\mathfrak{p}_a$ for $\mathfrak{p}A_a$ and $\mathfrak{p}_\mathfrak{p}$ for $\mathfrak{p}A_\mathfrak{p}$.
\item Given a $k$-derivation $D_i : A \rightarrow B$ and $S$ (resp. $T$) be a multiplicative set of $A$ (resp. B) such that $D_i (S) \subseteq T$. We can define a $k$-derivation $\widetilde{D_i}^S : S^{-1} A \rightarrow T^{-1} B$ by setting for all $a \in A$ and $b\in S$, $\widetilde{D_i}^S\left( \frac{a}{b}\right) := \frac{D_i(a)}{b} - \frac{ a D_i(b)}{b^2}$ and we have $\widetilde{D_i}^S\left( \frac{a}{1}\right)= \frac{D_i(a)}{1}$. When $S=\{ a^n | n \in \mathbb{N}\}$, we write $\widetilde{D_i}^a$ for $\widetilde{D_i}^S$ and when $S= A \backslash \mathfrak{p}$, we write  $\widetilde{D_i}^\mathfrak{p}$ for $\widetilde{D_i}^S$.  Such a derivation is uniquely determined. Thus, this correspondence defines a bijection 
$$Der_k ( A, B)   \simeq Der_k ( S^{-1}A, T^{-1} B)$$

\sophie{I have to do this better} \luigi{I would put this definition outside this list since it seems to address something different.}
\item Let $J$ be an ideal of $B$. We define the maximal spectrum at $J$ to be the set 
$$  \operatorname{Specm}_{J} ( B) = \{ \mathfrak{m} \in  \operatorname{Specm}(B) | J \subseteq \mathfrak{m}\}= V(J) \cap  \operatorname{Specm} ( B) $$ %\luigi{The information about I is already contained in $B$, do you mean that I should be a different ideal $J \subseteq B$?}
\item We define the maximal separable spectrum to be 
$$  \operatorname{Specm}_{ \operatorname{sep}/k} ( B)  =  \{ \mathfrak{m} \in  \operatorname{Specm}(B) | k(\mathfrak{m})/ k \text{ is separable } \}$$
%\item We define the set of {\emph separable rational maximal ideals} to be $$ \operatorname{R}_{ \operatorname{sep}} ( B) = \left\{ \frac{\langle x_1-a_1 , \cdots , x_n - a_n \rangle}{I} | a_i \in k^{ \operatorname{sep}} , \forall i \in \{ 1, \cdots, n \}  \right\}$$ \luigi{I think I would omit this one, you see the notion of rational point is already specific and this makes confusion, because the rational point is a k-point, not $ k^{sep}$. On the other hand, that ideal makes sense only if $a_i\in k$. Finally this notion is redundant with the notion of specmsep that we defined above; if we ever need to base-change to $k^{sep}$ we can alwyas say/prove that m in specmsep is the contraction of one of those ideals, if we ever need it.}
\end{enumerate} 
\end{definition}





\begin{remark}
For any $ \mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(B)$, any maximal above $\mathfrak{m}$ in $\bar{k} [x_1, \cdots , x_n]$ is in $ \operatorname{R}_{ \operatorname{sep}} ( B)$.
\end{remark} 

\begin{lemma} \label{fs} Let $A= k[x_1, \cdots, x_n]$ be a polynomial ring in $n$-indeterminates, $\mathfrak{p}$ be prime ideal of $A$ and $\bar{k}$ be an algebraic closure of $k$. The following statements are equivalent:
\begin{enumerate}
\item $k(\mathfrak{p})$ is formally smooth over $k$; 
\item there are $r \in \mathbb{N}$ and $k$-derivations $D_i\in Der_k (A/\mathfrak{p} , A)$ and $g_i \in A$, for all $i \in \{ 1, \cdots r \}$ such that $\mathfrak{p}A_\mathfrak{p}= \langle \frac{g_1}{1} , \cdots, \frac{g_r}{1}\rangle$, $det ( D_i (g_j) )\notin \mathfrak{p}$;
\item there are $r \in \mathbb{N}$, $I \subseteq \{ 1, \cdots, n \}$, $g_i \in A$, for all $i \in I$ such that $\mathfrak{p}A_\mathfrak{p}= \langle (\frac{g_i}{1})_{i \in I} \rangle$, $det ((\frac{\partial }{\partial x_i}  \left( \frac{g_i}{1}\right))_{i \in I} )\notin \mathfrak{p}$
%\item there are $r \in \mathbb{N}$ and $k$-derivatives $D_i\in Der_k (k(\mathfrak{p}), A)$ and $g_i \in A$, for all $i \in \{ 1, \cdots r \}$ such that $\mathfrak{p}A_\mathfrak{p}= \langle \frac{g_1}{1} , \cdots, \frac{g_r}{1}\rangle$, $det ( D_i \left(\frac{g_i}{1}\right) )\notin \mathfrak{p}$;
%\item there are $r \in \mathbb{N}$ and $k$-derivatives $D_i\in Der_k (\widehat{B_{\mathfrak{p}}}^{\mathfrak{p}} , B)$ and $g_i \in B$, for all $i \in \{ 1, \cdots r \}$ such that $\mathfrak{p}B_\mathfrak{p}= \langle \frac{g_1}{1} , \cdots, \frac{g_r}{1}\rangle$, $det ( D_i (g_i) )\notin \mathfrak{p}$, $a\in B$;
\item $k(\mathfrak{p})$ is separable over $k$; 
\item $k(\mathfrak{p})$ is separably generated over $k$; 
 \item $k(\mathfrak{p}) \otimes \bar{k}$ is reduced;
\item $ \operatorname{Specm}_{\operatorname{ \operatorname{sep}}}(A) \cap V ( \mathfrak{p}) $ is dense in $V(\mathfrak{p})$;
 \item $\mathfrak{p} =\cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(A) \cap V ( \mathfrak{p})} \mathfrak{m}$.
 \end{enumerate} 
%The equivalence $(1)-(6)$ is true when $A$ is noetherian smooth algebra over $k$. 
% When $char(k) =p >0$, the above statements are also equivalent to 
% \begin{enumerate} 
% \item[(8)] $k(\mathfrak{p}) \otimes k^{1/p}$ is reduced.
% \end{enumerate} 
\end{lemma} 
\begin{proof}
Let $S= \{ x_1 , \cdots ,x_n\}$, we write $k[S]:= k[x_1, \cdots, x_n ]$. Let $\mathfrak{p} \in \operatorname{Spec} ( k[S])$. 

%By Noether normalization lemma, $k[x_1, \cdots, x_n ]/ \mathfrak{p}$ is an algebra of finite type over the field $k$ and is an integral domain, so the transcendence degree of its fraction field is equal to the Krull dimension of $k[x_1, \cdots, x_n ]/ \mathfrak{p}$. More precisely, there exist $T$ subset of $S= \{ x_1, \cdots, x_n\}$ such that $k( \mathfrak{p})$ is finite over $k(T)$. %We call $\zeta_p : k[x_1, \cdots, x_n ] \rightarrow k( \mathfrak{p})$ is the residue field canonical morphism.
$(1) \Leftrightarrow (2)$ is guaranteed by \cite[Theorem 64]{Matsumura} applied to $A=k[x_1, \cdots, x_n ] $, $B=A/\mathfrak{p}$ at the prime ideal $(0)$, since $A$ is smooth over $k$. 

$(2) \Leftrightarrow (3)$ By assumption, there are $r \in \mathbb{N}$ and $k$-derivatives $D_i\in Der_k (A/\mathfrak{p}, A)$ and $g_i \in A$, for all $i \in \{ 1, \cdots r \}$ such that $\mathfrak{p}A_\mathfrak{p}= \langle \frac{g_1}{1} , \cdots, \frac{g_r}{1}\rangle$, $det ( (D_i \left(\frac{g_j}{1}\right))_{i,j \in \{ 1, \cdots , r\} })\notin \mathfrak{p}$.  
By the second fundamental exact sequence for the module of differential (see \cite[Theorem 58]{Matsumura}), we know that the $(\epsilon_\mathfrak{p} \circ \frac{\partial g_i}{\partial x_i})_{i \in \{ 1, \cdots , n \}}$ generate $\Omega_{A/ \mathfrak{p}/k}$. In particular, there is $I \subseteq \{ 1, \cdots, n \}$ of cardinality $r$ such that $det (\left( \frac{\partial }{\partial x_i} \left(\frac{g_i}{1}\right) \right)_{i \in I} )\notin \mathfrak{p}$. The converse is trivial.


%$(2) \Leftrightarrow (3)$ follows directly from the fact that given a $k$-derivation $D : A/ \mathfrak{p}\rightarrow A$, we can define a derivation $\tilde{D} : k(\mathfrak{p}) \rightarrow A$ by setting $\tilde{D}\left( \frac{a}{b}\right) := \frac{D(a)}{b} - \frac{ a D(b)}{b^2}$ and we have $\tilde{D}\left( \frac{a}{1}\right)= D(a)$. Conversely, given a $k$-derivation $D : k(\mathfrak{p}) \rightarrow A$ composing on the right by the canonical localization map $\iota : A/ \mathfrak{p} \rightarrow k(\mathfrak{p})$, we obtain a $k$-derivation $\overline{D}$ such that $D\left( \frac{a}{1}\right)= \overline{D}(a)$.\\ 
$(1) \Leftrightarrow (4)$ See \cite[Corollary 2.4.6]{Smooth} or \cite[Theorem 62]{Matsumura} or \cite[Lemma 10.158.8.]{Stack}.


$(4) \Leftrightarrow (5)$ Since by the Normalization theorem we have that there is a set of linearly independent elements $T$ of $k(\mathfrak{p})$ over $k$ such that $k(\mathfrak{p})$ is finite over $k(T)$ for any prime ideal of $A$.

 $(1) \Leftrightarrow (6)$ See \cite[(27.F) Lemma 3]{Matsumura}  

$(7) \Leftrightarrow (8)$ by definition of density in $V(\mathfrak{p})$ with respect to the Zariski Topology. 

$(5) \Rightarrow (7)$ We set $R =A/\mathfrak{p}$.  We know that there is a  $T \subseteq F$ %$T=\iota (\mathcal{T})$ where $\mathcal{T}$ is a subset of $ k[S ]/ \mathfrak{p}$ and $\iota : k[S ]/ \mathfrak{p} \rightarrow  k(\mathfrak{p})=( k[S ]/ \mathfrak{p})_{(0)}$ 
such that $k(\mathfrak{p}) / k( T)$ is finite separable. We denote $\overline{k[T]}$ to be the integral closure of $k[T]\subseteq F$. By construction $\operatorname{Frac}(\overline{k[T]})=\operatorname{Frac}(R)$. By Lemma \ref{birational}, there is $f \in R \backslash \{ 0 \} $ and $g \in \overline{ k[T]} \backslash \{ 0 \} $, $R_f \simeq \overline{ k[T]}_g$. Since $\Spec ( R_f)$ is not empty and $R$ is irreducible, $\Spec ( R_f)$  is dense in $\Spec(R)$. Similarly, $\Spec (\overline{ k[T]}_g)$ is dense in $\Spec (\overline{ k[T]})$.
%There are two open subset $U\subseteq \Spec (R)$ and $U' \subseteq \Spec ( \overline{k [T]})$ open such that $U \simeq U'$. 
Therefore, $\Specm_{\sep} (R)$  dense in $\Spec (R)$ if and only if $\Specm_{\sep} (\overline{ k[T]})$  dense in $\Spec (\overline{ k[T]})$. 

%We now assume that $k(\mathfrak{p})$ is separably generated over $k$. We can choose $T \subseteq F$, such that $k(\mathfrak{p}) / k( T)$ is finite separable. 
By Lemma \ref{seplemma}, we know that $\Specm_{\sep /k } (\overline{ k[T]})$ is dense in $\Spec (\overline{ k[T]})$. Thus by the reasoning above  $\Specm_{\sep /k } (R)$  dense in $\Spec (R)$. 

$(6) \Rightarrow (5)$ We assume $k(\mathfrak{p})\otimes_k \bar{k}$ is not reduced. We set $C= A/ \mathfrak{p} \otimes \bar{k}$. $C$ is not reduced \cite[Chapter 3. Exercise 5]{AM}. %We  set $C_{red} = C/ \sqrt{0_C}$ the reduced ring. 
Let $\mathfrak{m}$ be a maximal ideal containing $\mathfrak{p}$. We prove that $k(\mathfrak{m}) \otimes_k \bar{k} $ is not reduced. Using \cite[Theorem 4.21]{CTP} that $k(\mathfrak{m}) \otimes_k \bar{k} \simeq k(\mathfrak{m}) \otimes_{k[(x_i)]/ \mathfrak{p} }C\simeq k(\mathfrak{m}) \otimes_{k }C $. 
 %We have $ \sqrt{0_C} \otimes_k k(\mathfrak{m}) \subseteq \sqrt{0_{ k(\mathfrak{m}) \otimes_{k }C}}$. 
 Since $k(\mathfrak{m}) $ is faithfull flat over $k$ and $\sqrt{0_C}  \neq \{0\}$ by assumption, we have $\sqrt{0_C} \otimes_k k(\mathfrak{m})\neq \{ 0\} $. Thus since $ \sqrt{0_C} \otimes_k k(\mathfrak{m}) \subseteq \sqrt{0_{ k(\mathfrak{m}) \otimes_{k }C}}$, $k(\mathfrak{m}) \otimes_k \bar{k} $ is not reduced. 

%Thus, from the above we have a natural map from $k[T]$ to $R_f$ defined as the composite $k[T] \rightarrow \overline{k[T]}\rightarrow \overline{k[T]}_g \simeq R_f$ and \\$\Specm_{\sep / k(T) } (R_f \otimes_{k[T]} k(T))$ is dense in $\Spec (R_f\otimes_{k[T]} k(T))$. %Let $\varphi : R \rightarrow R_f\otimes_{k[T]} k(T)$ be the canonical map defined by the tensor product and the localization.  Since $k(\mathfrak{p})/k(T)$ is finite, $R_f \otimes_{k[T]} k(T)= k(\mathfrak{p})$ and $k(\mathfrak{p})/k(T)$ is separable by definition of $ \Specm_{\sep / k(T) } (R_f \otimes_{k[T]} k(T))$.
% $\varphi (\mathfrak{p})$ is a maximal ideal in $\Specm_{\sep} (R_f \otimes_{k[T]} k(T))$. That is, $R_f\otimes_{k[T]} k(T)/\varphi (\mathfrak{p})$ is separable. 
%Suppose that $k(\mathfrak{p})$ is separately generated over $k$. This means that there is a subset $T=\iota (\mathcal{T})$ where $\mathcal{T}$ is a subset of $ k[S ]/ \mathfrak{p}$ and $\iota : k[S ]/ \mathfrak{p} \rightarrow  k(\mathfrak{p})=( k[S ]/ \mathfrak{p})_{(0)}$ such that $k(\mathfrak{p}) / k( T)$ is separable. Moreover, $|T|$ is the transcendence degree of $k(\mathfrak{p})$ fraction field of $k[S ]/ \mathfrak{p}$. By Noether normalization lemma, $k[S]/ \mathfrak{p}$ is an algebra of finite type over the field $k$ and is an integral domain, so the transcendence degree of its fraction field is equal to the Krull dimension of $k[x_1, \cdots, x_n ]/ \mathfrak{p}$. In particular $k(\mathfrak{p})$ is finite over $k(T)$. Since $k(\mathfrak{p})$ is finite and separable over $k(T)$, by the primitive element theorem, we know that there exists $y= \iota ( z) \in k( \mathfrak{p})$ whose minimal monic polynomial $p(T)(x)$ and where $z \in k[S ]/ \mathfrak{p}$. We write $p(T)(x) = x^n + \frac{a_1(T)}{b(T)}x^{n-1} + \cdots + \frac{a_n(T)}{b(T)}$. where $a_i(T) \in k[T]$ and $b (T) \in k[T]^*$. We obtain $p(T)'(x)= nx^{n-1} + (n-1) \frac{a_1(T)}{b(T)}x^{n-2} + \cdots + \frac{a_{n-1}(T)}{b(T)}$. Since $k(\mathfrak{p})$ is separable over $k(T)$, we know that $p(T)(x)$ and $p(T)'(x)$ are coprime. Thus, there are $\alpha (T)(x), \gamma(T)(x) \in k[T][x]$ and $ \beta(T), \delta(T)   \in k[T]^*$, such that 
%$$ \frac{\alpha(T)(x)}{\beta(T)} p(T)(x) + \frac{\gamma (T)(x) }{\delta(T)} p(T)'(x) \equiv 1.$$ 
%We set 
%$$Z = Z_{sep} (\beta) \cup Z_{sep} (\delta)  \cup Z_{sep} (b) $$
%where $Z_{sep} (q) = \{ \underline{a} \in {k^{sep}}^{|T|} |   q( \underline{a}) =0\}$ for $q \in k[T]$. 
%
%Let $\underline{c}=(c_1 , \cdots, c_{|T|})  \in {k^{sep}}^{|T|}\backslash Z$. We have 
%$$\frac{\alpha(\underline{c})(x)}{\beta(\underline{c})} p(\underline{c})(x) + \frac{\gamma( \underline{c})(x)  }{\delta( \underline{c})} p(\underline{c})'(x) =1$$
%Writing $T= \{t_1 , \cdots , t_{|T|} \}$. Let $\mathfrak{m}_{\underline{c}}= k[T] \cap < t_1- c_1, \cdots , t_{|T|} - c_{|T|}>$. We have $\mathfrak{m}_{\underline{c}}$ is a maximal ideal in $k [T]$ (see for instance Conrad). We set $R := k[S]/\mathfrak{p} \otimes_{k[T]} k( \mathfrak{m}_{\underline{c}})$. We have 
%$$ R \simeq k( \mathfrak{m}_{\underline{c}}) [ S \backslash \mathcal{T}]/ \varphi ( \mathfrak{p}) $$ 
%where $\varphi$ is the canonical map from $k[S]$ to $k(\mathfrak{m}_{\underline{c}}) [ S \backslash \mathcal{T}]$.

%Thus, since $p(x)$ is irreducible by definition, that means that $p'(x)\neq0$. 
%
%We set 
%$$A =\cap_{i \in I} \{ \underline{a} \in k^{sep} |  a_i(  \underline{a})= 0 \} $$
%where $I= \{ 1 ,\cdots , n-1\}$ when $char(k) =0$ and $I = \{ i \in \{ 1 ,\cdots , n-1\}| p \nmid n -i \}$.
%and 
%$$B = \{ \underline{b} \in k^{sep} |  a_i(  \underline{b})= 0 \} .$$


%Suppose that $k(\mathfrak{p})$ is separably generated over $k$. Therefore, $k(\mathfrak{p})$ is finite separable over $k(T)$. 
%
%\luigi{This is not correct, because T has been fixed above and then you are using the definition of "separably generated" to assert that exists a trascendent base T' such that k(p)/k(T') is separable. Nothing allows you to take T=T'.
%Indeed take the example $p=(x-y^2) \subseteq k[x,y]$, with char 2. T can both be the singleton $\{x\}$ and the singleton $\{y\}$, while $k(p)=k(y)$. If $T=\{y\}$ then $k(p)/k(T)$ is separable. 
%If $T=\{x\}$ then not.}
%
%Thus, by the primitive element theorem, we know that any finite separable extension admits a primitive element therefore there exists $z \in k( \mathfrak{p})$ such that $k(\mathfrak{p})= k(T)(z)$ and the minimal polynomial $p(X)$ of $z$ over $k(T)$ is separable. Moreover, %we have $k(\mathfrak{p})\otimes_{k(T)} k(T)^{sep} = k(T)^{deg( k(\mathfrak{p})/ k(T))}$ and 
%%
%the image $\mathfrak{P}$ of $\mathfrak{p}$ in $k(T) [ S \backslash T] \simeq k(T) \otimes_{k[T]} k[x_1, \cdots , x_n]$ is a maximal ideal in $k(T) [ S \backslash T]$. Indeed if it was not then the transcendental degree of $k(\mathfrak{P})\simeq k(\mathfrak{p})$ over $k(T)$ would be strictly greater than $0$ and that would constitute a contradiction. %Indeed, we have $\mathfrak{P}$ is the kernel of the map $k(T) [ S \backslash T] \rightarrow k(T) \otimes_{k[T]} k(\mathfrak{p})$. Moreover the following diagram 
%%$$\xymatrix{ 0 \ar[r] & \mathfrak{P} \ar[d] \ar[r]  & k(T) [ S \backslash T] \ar@{->>}[d]\ar[r] & k(T) \otimes_{k[T]} k(\mathfrak{p})  \ar[d]^{\simeq}    \\ 0 \ar[r] & \langle p(X) \rangle  \ar[r] & 
%% k(T)[X] \ar[r] & k(T)(z) \ar[r] & 0 }$$ 
%%
%%the image of $\mathfrak{p}$ in $k[x_1, \cdots , x_n]$ is $\langle p(X) \rangle$ maximal ideal of $k(T) [ z]$. 
%We have $\langle p(X) \rangle k(T)^{sep} [ X] =\cap_{b \in Z} \langle X- b\rangle $ where $ Z$ is the (finite) set of zeros of $p(X)$.  We denote $\iota$ the canonical map from $k(T)^{sep} [ S \backslash T]$ and $  k(T)^{sep} [ X]$ induced by the canonical map from $k(T) [ S \backslash T]$ and $  k(T) [ X]$
%\luigi{What is the canonical map? Where do you send the xi for i out of T?}
%
%%$$\xymatrix{ k(\mathfrak{P}) \ar[r]^{\overline{\Phi}} & k( \mathfrak{p})=k(T)(z) \\ 
%%k(T)[ S \backslash T] \ar@{->>}[u] \ar[r]^{\Phi} & k(T)[ X] \ar@{->>}[u]}$$
%%Let $w = \phi^{-1} ( z)$. Given 
%
% that in turn induces the isomorphism $k(\mathfrak{P})\simeq k(\mathfrak{p})$. We have that 
% $$\mathfrak{P}k(T)^{sep} [ S \backslash T]  =\iota^{-1} ( \langle p(X) \rangle  k(T)^{sep} [ X] ) = \cap_{\underline{a} \in \iota^{-1}(Z)} \langle x_i - a_i\rangle_{i \in S\backslash T} .$$ Finally, we obtain 
%$$\mathfrak{p} k^{sep} [S] =  \bigcap_{(a_i)_{i \in T}  \in {k^{sep}}^T } \bigcap_{(a_i)_{S\backslash T} \in \iota^{-1}(Z)} \langle x_i - a_i\rangle_{i \in S}$$
%
%\luigi{I need to see how iota is defined, in order to understand the last equality... I thought a little bit, but I didn't came with a definition that suits.}

%$(7) \Rightarrow (5)$ We suppose that $\mathfrak{p} =\cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(A) \cap V ( \mathfrak{p})} \mathfrak{m}$. This equality induce an injective morphism $$ \phi : A / \mathfrak{p} \rightarrow \prod_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(A) \cap V ( \mathfrak{p})} A / \mathfrak{m} $$

%Suppose that $\mathfrak{p}k^{sep}[x_1, \cdots , x_n] = \cap_{\mathfrak{m}\in {\mathscr{M}_{sep}}} \mathfrak{m}$ where $\mathscr{M}_{sep} = \{ \langle x_1-a_1 , \cdots , x_n - a_n \rangle | a_i \in k^{sep} , \forall i \in \{ 1, \cdots, n \}  \}$. We denote $\eta : k[x_1, \cdots, x_n] \rightarrow k(T) [ S \backslash T]$ and $\mathfrak{P}= \eta ( \mathfrak{p})$. We can deduce $\mathfrak{P}k^{sep}(T)[S \backslash T] \simeq \cap_{\mathfrak{m}\in {\mathscr{M}_{sep}}} \eta(\mathfrak{m})$.




\end{proof}

\begin{lemma} \label{ss-1}Let $k$ be a field.
%Let $B$ be a finitely presented algebra over $k$, $\mathfrak{p}$ be prime ideal, $s\in \mathbb{N}$ and $f \in B$.  
Let $A= k[x_1, \cdots, x_n]$ be a polynomial ring in $n$-indeterminates, $\mathfrak{p}$ be prime ideal of $A$, $s\in \mathbb{N}$ and $f \in A$. 
We assume that $k(\mathfrak{p})$ separably generated over $k$. By Lemma \ref{fs}, we can choose $I \subseteq \{ 1, \cdots, n \}$, $g_i \in A$, for all $i \in I$ such that $\mathfrak{p}A_\mathfrak{p}= \langle (\frac{g_i}{1})_{i \in I} \rangle$, $det ((\frac{\partial }{\partial x_i}  \left( \frac{g_j}{1}\right))_{i \in I} )\notin \mathfrak{p}$. 
Then there is $a \notin \mathfrak{p}$ such that the following equivalence is satisfied  %$a\in B$ and such that we have $f \in \mathfrak{p}_a^s$ if and only if $f\in \mathfrak{p}_a^{s-1}$ and $D_i (f) \in \mathfrak{p}_a^{s-1}$, for all $i \in \{ 1, \cdots, r\}$.  In particular, 
$f \in \mathfrak{p}_a^s$ if and only if $f\in {\mathfrak{p}_a}^{s-1}$ and $\widetilde{\frac{\partial }{\partial x_i}}^a (f) \in {\mathfrak{p}_a}^{s-1}$, for all $i\in \{ 1, \cdots, r\}$. In particular, we have $\frac{f}{1} \in {\mathfrak{p}_\mathfrak{p}}^s$ if and only if $f\in \mathfrak{p}_\mathfrak{p}^{s-1}$ and $\widetilde{\frac{\partial }{\partial x_i}}^{\mathfrak{p}} (f) \in \mathfrak{p}_\mathfrak{p}^{s-1}$, for all $i\in I$.
\end{lemma} 

\begin{proof}
Let $A= k[x_1, \cdots, x_n]$, $\mathfrak{p}$ be prime ideal, $s\in \mathbb{N}$ and $f \in A$. 



%We can define a derivation $\widetilde{D_i} : k(\mathfrak{p}) \rightarrow A_\mathfrak{p}$ by setting $\widetilde{D_i}\left( \frac{a}{b}\right) := \frac{D_i(a)}{b} - \frac{ a D_i(b)}{b^2}$ and we have $\widetilde{D_i}\left( \frac{a}{1}\right)= \frac{D_i(a)}{1}$. So that $det ( \widetilde{D_i} \left(\frac{g_i}{1}\right) )\neq 0$

%Conversely, given a $k$-derivation $D : k(\mathfrak{p}) \rightarrow A$ composing on the right by the canonical localization map $\iota : A/ \mathfrak{p} \rightarrow k(\mathfrak{p})$, we obtain a $k$-derivation $\overline{D}$ such that $D\left( \frac{a}{1}\right)= \overline{D}(a)$.\\ 

%We have that $\mathcal{L}_1 (A)_{k(\mathfrak{p})}$ is a polynomial ring over $k(\mathfrak{p})$. Therefore, $\mathcal{L}_1 (A)_{k(\mathfrak{p})}$ is smooth over $k(\mathfrak{p})$. By Lemma \ref{sym}, any $\widetilde{D_i}\in Der_k (k(\mathfrak{p}), A_\mathfrak{p})$, there is a  $k(\mathfrak{p})$-module morphism $ f_{\widetilde{D_i}} : \mathcal{L}_1 (A)_{k(\mathfrak{p})} \rightarrow k(\mathfrak{p})$ lifts into a $k(\mathfrak{p})$-morphism $\widetilde{ f}_{\widetilde{D_i}} : \mathcal{L}_1 (A)_{k(\mathfrak{p})} \rightarrow \widehat{A_\mathfrak{p}}$. Again by Lemma \ref{sym}, to $\widetilde{ f}_{\widetilde{D_i}}$ induces a $k$-derivation $\mathbf{D}_i : \widehat{A_\mathfrak{p}} \rightarrow  A$ with $\mathbf{D}_i \left( \frac{g_i}{1}\right)= \widetilde{D_i}  \left( \frac{g_i}{1}\right)$. Thus, $det ( {\mathbf{D}_i}\left( \frac{g_i}{1}\right) )\neq 0$.

 Clearly, $f \in \mathfrak{p}^s$ implies $f\in {\mathfrak{p}}^{s-1}$ and $\frac{\partial g_i}{\partial x_i}  (f) \in {\mathfrak{p}}^{s-1}$, for all $i\in \{ 1, \cdots, n\}$.
 
 We now prove the converse. Let $r \in \mathbb{N}$, $I \subseteq \{ 1, \cdots, n \}$, $g_i \in A$, for all $i \in I$ such that $\mathfrak{p}A_\mathfrak{p}= \langle (\frac{g_i}{1})_{i \in I} \rangle$, $det ((\frac{\partial}{\partial x_i}  \left( \frac{g_j}{1}\right))_{i \in I} )\notin \mathfrak{p}$. Since $\mathfrak{p}A_\mathfrak{p}= \langle (\frac{g_i}{1})_{i \in I} \rangle$ and $\mathfrak{p}$ is finitely generated, we have $\mathfrak{p} = \langle (g_i)_{i \in I} , (h_j)_{i \in J}\rangle$ for some $J$ finite set and $h_j \in A$ for all $j \in J$.
 Since $\mathfrak{p}A_\mathfrak{p}= \langle (\frac{g_i}{1})_{i \in I} \rangle$, then there is $\delta \in A$ such that for all $j \in J$, $\frac{h_j}{1} = \sum_{i\in I} \frac{a_{i,j}}{\delta} \frac{g_i}{1}$, where $a_{i,j} \in A$, for all $(i,j)\in I \times J$. We set $a= det ((\frac{\partial}{\partial x_i}  \left( \frac{g_j}{1}\right))_{i,j \in I} )\delta$. We have $\mathfrak{p}_a= \langle (\frac{g_i}{1})_{i \in I} \rangle$. We prove that if $f\in {\mathfrak{p}_a}^{s-1}$ and $\widetilde{\frac{\partial }{\partial x_i}}^a \left(\frac{f}{1}\right) \in {\mathfrak{p}_a}^{s-1}$, for all $i\in \{ 1, \cdots, r\}$ then $\frac{f}{1} \in \mathfrak{p}_a^s$. We write $\frac{f}{1}= \sum_{\underline{k}\in K} a_{\underline{k}} \frac{g_{k_1}}{1} \cdots \frac{g_{k_{s-1}}}{1} $, where $K$ is a subset of $I^{s-1}$ and $a_{\underline{k}} \in A$ for all $k \in K$.  Let $(l_1, \cdots, l_{s-1})\in I^{s-1}$. We have 
 $$\widetilde{\frac{\partial }{\partial x_{l_s}}}^a\left( \cdots \left(\widetilde{ \frac{\partial }{\partial x_{l_1}}}^a\left( \frac{f}{1}\right)\right)\right)=\sum_{\underline{k}\in K} \sum_{\sigma \in S_{s-1}}  a_{\underline{k}} {\widetilde{\frac{\partial }{\partial x_{l_{\sigma(1)}}}}^a\left( \frac{g_{k_1}}{1} \right)} \cdots {\widetilde{\frac{\partial }{\partial x_{l_{\sigma(s)}}}}^a\left( \frac{g_{k_{s-1}}}{1}\right)}+ \rho \in \mathfrak{p}_a$$ 
 where $\rho \in \mathfrak{p}_a$. So that $\sum_{\underline{k}\in K} \sum_{\sigma \in S_{s-1}}  a_{\underline{k}} {\widetilde{\frac{\partial }{\partial x_{l_{\sigma(1)}}}}^a\left( \frac{g_{k_1}}{1} \right)} \cdots {\widetilde{\frac{\partial }{\partial x_{l_{\sigma(s)}}}}^a\left( \frac{g_{k_{s-1}}}{1}\right)} \in \mathfrak{p}_a$.
 
 Setting $M=(\frac{\partial}{\partial x_i}  \left( \frac{g_j}{1}\right))_{i,j \in I}$.
 Since by assumption $det(M) \notin \mathfrak{p}_a$ the determinant of the Kronecker product of $M$ with itself $s-1$ times $M^{\otimes(s-1)}$ is also not in $\mathfrak{p}_a$. So that, $a_{\underline{k}} \in \mathfrak{p}_a$ for all $k \in K$, since $\zeta_{\mathfrak{p}_a} (det(M^{\otimes(s-1)}) ) \in \left( A_a/ \mathfrak{p}_a\right)^\times$ why definition of $a$. 
 %We suppose that $f\in ({\mathfrak{p}A_\mathfrak{p}})^{s-1}$ and $\mathbf{D}_i (f) \in ({\mathfrak{p}A_\mathfrak{p}})^{s-1}$, for all $i\in \{ 1, \cdots, r\}$. We want to prove that $f \in ({\mathfrak{p}A_\mathfrak{p}})^s$.

\end{proof} 


\begin{cor} Let $k$ be a field.
Let $B$ be a finitely presented algebra over $k$, $\mathfrak{p}$ be prime ideal and $s\in \mathbb{N}$.  
%Let $A= k[x_1, \cdots, x_n]$ be a polynomial ring in $n$-indeterminates, $\mathfrak{p}$ be prime ideal of $A$, $s\in \mathbb{N}$. 
We assume that $k(\mathfrak{p})$ separably generated over $k$. 
Then there is $a \in A$, $ \mathfrak{p}_a^{s} = \cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})} \mathfrak{m}_a^s. $ 
In particular, $ \mathfrak{p}_\mathfrak{p}^{s} = \cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})} \mathfrak{m}_\mathfrak{p}^s. $ 
\end{cor} 

\begin{proof}
We assume that $k(\mathfrak{p})$ separably generated over $k$. By Lemma \ref{fs}, we know that  $\mathfrak{p} =\cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})} \mathfrak{m}$; Therefore, by definition of $\operatorname{Specm}_{\operatorname{sep}}(R)$, we have $k(\mathfrak{m})/k$ is separably generated. 

We first prove the result for $A= k[x_1, \cdots, x_n]$ be a polynomial ring in $n$-indeterminates by induction on $s$.  For $s=1$, the result is true by assumption.
By Lemma \ref{fs}, we can choose $I \subseteq \{ 1, \cdots, n \}$, $g_i \in A$, for all $i \in I$ such that $\mathfrak{p}A_\mathfrak{p}= \langle (\frac{g_i}{1})_{i \in I} \rangle$, $det ((\frac{\partial }{\partial x_i}  \left( \frac{g_j}{1}\right))_{i \in I} )\notin \mathfrak{p}$. Since $\mathfrak{p}A_\mathfrak{p}= \langle (\frac{g_i}{1})_{i \in I} \rangle$ and $\mathfrak{p}$ is finitely generated, we have $\mathfrak{p} = \langle (g_i)_{i \in I} , (h_j)_{i \in J}\rangle$ for some $J$ finite set and $h_j \in A$ for all $j \in J$.
 Since $\mathfrak{p}A_\mathfrak{p}= \langle (\frac{g_i}{1})_{i \in I} \rangle$, then there is $\delta \in A$ such that for all $j \in J$, $\frac{h_j}{1} = \sum_{i\in I} \frac{a_{i,j}}{\delta} \frac{g_i}{1}$, where $a_{i,j} \in A$, for all $(i,j)\in I \times J$. We set $a= det ((\frac{\partial}{\partial x_i}  \left( \frac{g_j}{1}\right))_{i,j \in I} )\delta$ as in the proof of Lemma \ref{ss-1}. We suppose that the result is true for $s-1$, that is $ \mathfrak{p}_a^{s-1} = \cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})} \mathfrak{m}_a^{s-1}$. We prove the result for $s$. Using Lemma \ref{ss-1} multiple times and the induction assumption, we obtain that the following statements are equivalent:
 \begin{enumerate} 
 \item $f \in \mathfrak{p}_a^{s}$ 
 \item  $f \in \mathfrak{p}_a^{s-1}$ and $\widetilde{\frac{\partial }{\partial x_i}}^a (f) \in {\mathfrak{p}_a}^{s-1}$, for all $i\in \{ 1, \cdots, r\}$.
 \item $f \in \mathfrak{m}_a^{s-1}$ and $\widetilde{\frac{\partial }{\partial x_i}}^a (f) \in {\mathfrak{m}_a}^{s-1}$, for all $i\in \{ 1, \cdots, r\}$ and for all $\mathfrak{m}\in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})$.
 \item $f \in \mathfrak{m}_a^{s}$ for all $\mathfrak{m}\in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})$.
 \end{enumerate}
 This concludes the proof by induction.
Now we prove the result for $B$ a finitely presented algebra over $k$. We have $B= \frac{ k[x_1, \cdots, x_n]}{\mathfrak{a}}$. Given $\mathfrak{P}$ a prime ideal of $B$, by the ideals correspondence, we know that there is $\mathfrak{p}$ ideal of $A$ such that $\mathfrak{P} = \frac{ \mathfrak{p}}{\mathfrak{a}}$. Without loss of generality, we can assume that $\mathfrak{p}$ is the prime ideal as in the first part of the proof and keep the same notation. We set $\mathcal{S}'= \{ \mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})|  \frac{\mathfrak{m}+ \mathfrak{a}}{\mathfrak{a}} \text{ is a maximal ideal of $B$}\}$. We note that for any ideal in $ \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})$ but not in $ \mathcal{S}'$ with have $\frac{\mathfrak{m}+ \mathfrak{a}}{\mathfrak{a}} = B$.
 Now $\mathfrak{P}_{\bar{a}} = \frac{ \mathfrak{p}_a}{\mathfrak{a}_a}$. We have $\mathfrak{P}_{\bar{a}}=\cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})}  \frac{\mathfrak{m}_a+ \mathfrak{a}_a}{\mathfrak{a}_a}=  \cap_{\mathfrak{m} \in  \operatorname{Specm}_{ \mathcal{S}'}}  \frac{\mathfrak{m}_a+ \mathfrak{a}_a}{\mathfrak{a}_a}$ and $\mathfrak{M}_a= \frac{\mathfrak{m}_a+ \mathfrak{a}_a}{\mathfrak{a}_a}$ where $\mathfrak{M}= \frac{\mathfrak{m}+ \mathfrak{a}}{\mathfrak{a}}$. We note that $k( \mathfrak{M}) = k (\mathfrak{m})$ is separable over $k$, for any $\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})'$. Therefore 
$$\begin{array}{lll} \mathfrak{P}_{\bar{a}}^s  &=& \left( \frac{ \mathfrak{p}_a}{\mathfrak{a}_a}\right)^s = 
  \frac{ \mathfrak{p}_a^s + \mathfrak{a}_a}{\mathfrak{a}_a}=   \frac{\cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})} \mathfrak{m}_a^s+ \mathfrak{a}_a}{\mathfrak{a}_a}\\
  &=& \frac{\cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})} (\mathfrak{m}_a^s+ \mathfrak{a}_a)}{\mathfrak{a}_a}= \cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})} \left( \frac{\mathfrak{m}_a}{\mathfrak{a}_a}\right)^s\\
  &=&  \cap_{\mathfrak{m} \in  \mathcal{S}'} \left( \frac{\mathfrak{m}_a}{\mathfrak{a}_a}\right)^s=\cap_{\mathfrak{m} \in  \mathcal{S}'} {\mathfrak{M}_a}^s \end{array}$$
 This concludes the proof. 
\end{proof}
We can deduce the following corollary directly from the previous result.
\begin{cor}\label{specmsep}
Let $B$ be a finitely presented algebra over $k$, $\mathfrak{p}$  be prime ideal of $B$ and $s\in \mathbb{N}$.  
%Let $A= k[x_1, \cdots, x_n]$ be a polynomial ring in $n$-indeterminates, $\mathfrak{p}$ be prime ideal of $A$, $s\in \mathbb{N}$. 
We assume that $k(\mathfrak{p})$ separably generated over $k$. %By Lemma \ref{fs}, we know there is $ \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p}) \subseteq \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})$, $\mathfrak{p} =\cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})} \mathfrak{m}$ and $h \in B$; 
We have $G_s (\mathfrak{p} ) =\cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(R) \cap V ( \mathfrak{p})} G_s (\mathfrak{m})$. 
\end{cor}




 
%\begin{definition}(Lemma) \label{phidef}
%Let $s\in \mathbb{N}$, $R$ be a commutative unitary ring, $A := R[\underline{x}]$, $\mathfrak{a}$ ideal of $A$, $B := A/ \mathfrak{a}$, $\mathfrak{p}$ be a prime ideal of $B$ and $C$ be a $B$-algebra with $\rho_C:  B \rightarrow C$. We set $\mathfrak{a}_s:= \mu_{0,s}^A( \mathfrak{a})$. 
%\begin{enumerate} 
%\item We have the following $R$-algebra isomorphism
%$$ \mathcal{L}_s( A) \simeq^{\varphi_{s,A}} { A[ (\underline{x}_i)_{1\leq i\leq s}]};$$ 
%$$ \mathcal{L}_s( A)/\mathfrak{a}_s \simeq^{\overline{\varphi}_{s,A,\mathfrak{a}}} { B[ (\underline{x}_i)_{1\leq i\leq s}]};$$ 
%$$ \mathcal{L}_s( B) \simeq^{{\varphi}_{s, B, \mathfrak{a}}} { B[ (\underline{x}_i)_{0\leq i\leq s}]}/\overline{ \mathcal{L}_s( \mathfrak{a})};$$
%and 
%$$ \mathcal{L}_s( B) \otimes_{B} C \simeq^{\widetilde{\varphi}_{s,B,\mathfrak{a}, C}} { C[ (\underline{x}_i)_{0\leq i\leq s}]}/\overline{ \mathcal{L}_s( \mathfrak{a})}^{C}$$
%where \begin{itemize} 
%\item $\varphi_{s,A} $ is the $R$-algebra isomorphism sending $\underline{x}_0$ to $\underline{x}$ and $\underline{x}_i$ to $\underline{x}_i$ for all $i \in \{ 1, \cdots, s\}$. We note that $\varphi_{s,A} ( \mathfrak{a}_s) = \mathfrak{a}$;
%\item $\overline{\varphi}_{s, A , \mathfrak{a}} $  is the $R$-algebra isomorphism sending $[\underline{x}_0]_{\mathfrak{a}_s}$ to $[\underline{x}]_{\mathfrak{a}}$ and $[\underline{x}_i]_{\mathfrak{a}_s}$ to $\underline{x}_i$ for all $i \in \{ 1, \cdots, s\}$;
%\item $\overline{ \mathcal{L}_s( \mathfrak{a})}= {\overline{\varphi}_{A , \mathfrak{a}}(  \mathcal{L}_s( \mathfrak{a})/ \mathfrak{a}_s)}$;
%\item $\varphi_{s, B, \mathfrak{a}} $  is the $R$-algebra isomorphism sending $[\underline{x}_0]_{ \mathcal{L}_s(\mathfrak{a})}$ to $[\underline{x}]_{\mathfrak{a}}$ and $[\underline{x}_i]_{ \mathcal{L}_s(\mathfrak{a})}$ to $[\underline{x}_i]_{ \overline{\mathcal{L}_s(\mathfrak{a})}}$ for all $i \in \{ 1, \cdots, s\}$; 
%\item $\overline{ \mathcal{L}_s( \mathfrak{a})}^C= \pi_C (\overline{ \mathcal{L}_s( \mathfrak{a})}) $ with $\pi_C $ is the canonical map from $B[ (\underline{x}_i)_{1\leq i\leq s}]$ to $C[ (\underline{x}_i)_{1\leq i\leq s}]$;
%\item $\widetilde{\varphi}_{s, B,\mathfrak{a}, C} $  is the $R$-algebra isomorphism sending $[\underline{x}_0]_{ \mathcal{L}_s(\mathfrak{a})}\otimes c $ to $c [\underline{x}]_{\mathfrak{a}}$ and $[\underline{x}_i]_{ \mathcal{L}_s(\mathfrak{a})}\otimes c $ to $c[\underline{x}_i]_{ \overline{\mathcal{L}_s(\mathfrak{a})}}$ for all $i \in \{ 1, \cdots, s\}$; 
%%\item $\overline{ \mathcal{L}_1( \mathfrak{a})}^{\mathfrak{p}} = \pi_{\mathfrak{p}} (\mathcal{L}_1( \mathfrak{a})}^{\mathfrak{p})$, where $\pi_{\mathfrak{p}}: $
%\end{itemize} 
%\item Given $B= R[\underline{x}] / \mathfrak{a}$ and $s\in \mathbb{N}$. 
%%, $C$ $B$-algebra with $\pi_C.
%%$\mathfrak{p}$ be a prime ideal of $R[\underline{x}]$. %and a family of $R$-derivation $D=(D_i)_{i \in \{1, \cdots, r\}}$ of $A$ into $A /\mathfrak{p}$. 
%We define {\sf the Taylor map of order 1 on $B$ along $\mathfrak{a}$ at $\mathfrak{p}^s$}  to be the map $$ T_{1, B, \mathfrak{a}, \mathfrak{p}^s} : \frac{B_\mathfrak{p}}{\mathfrak{p}^s} \rightarrow   
% \mathcal{L}_1(B)_{\mathfrak{p}^s}/ (\underline{x}_{1} )^2_{\mathfrak{p}^s}  $$ defined as the composite of the isomorphism $$\overline{ \widetilde{\varphi}_{1, B, \mathfrak{a} ,A/\mathfrak{p}^s}^{-1} }: ({ A/ \mathfrak{p} [ \underline{x}_1]}/\overline{ \mathcal{L}_1( \mathfrak{a})}^{A/\mathfrak{p}^s}) / \overline{(\underline{x}_{1} )^2_{\mathfrak{p}^s}} \rightarrow  \mathcal{L}_1(B)_{\mathfrak{p}^s}/ (\underline{x}_{1} )^2_{\mathfrak{p}^s} $$ is the quotient isomorphism induced by the isomorphism $ \widetilde{\varphi}_{1, B,\mathfrak{a}, \mathfrak{p}^s} ^{-1}$ where \\$\overline{(\underline{x}_{1} )^2_{\mathfrak{p}^s}}= \widetilde{\varphi}_{1, B,\mathfrak{a}, \mathfrak{p}^s} ((\underline{x}_{1} )^2_{\mathfrak{p}^s} )$ and the map 
% $$
%\overline{\tau}_{1,B, \mathfrak{a}, A/\mathfrak{p}^s} : \frac{B_\mathfrak{p}}{\mathfrak{p}^s}  \rightarrow   (({ A/\mathfrak{p}^s[ \underline{x}_1]})/\overline{ \mathcal{L}_1( \mathfrak{a})}^{A/\mathfrak{p}^s}) / \overline{(\underline{x}_{1} )^2_{\mathfrak{p}^s}}$$ sending $[[f]_{\mathfrak{a}}]_{\mathfrak{p}^s}$ to $[[ [f]_{\mathfrak{p}^s} +\sum_{i=1}^n  [ \frac{\partial }{\partial x_{i} } (f) x_{i,1}]_{\mathfrak{p}^s}  ]_{ \overline{ \mathcal{L}_1( \mathfrak{a})}^{A/\mathfrak{p}^s}}]_{\overline{(\underline{x}_{1} )^2_{\mathfrak{p}^s}}} $. 
%
%We note that $\overline{\tau}_{1,B, \mathfrak{a}, A/\mathfrak{p}^s}$ is well defined since by definition of $ \mathcal{L}_1( \mathfrak{a})$, $f \in \mathfrak{a}$ implies $\overline{\tau}_{1,B, \mathfrak{a}, A/\mathfrak{p}^s}(f) \in \overline{ \mathcal{L}_1( \mathfrak{a})}^{A/\mathfrak{p}^s}$.
%\end{enumerate} 
%%Moreover, for all $C$ $B/I$-algebra, we have 
%%$$  \mathcal{L}_1( B/I) \otimes_{B/I} C\simeq { C[ (\underline{x}_i)_{1\leq i\leq s}]}/{\pi_C (\overline{\varphi} (  \mathcal{L}_1( I)/ I_s))}$$
%%where $\pi_C $ is the canonical map from $B/I[ (\underline{x}_i)_{1\leq i\leq s}]$ to $C[ (\underline{x}_i)_{1\leq i\leq s}]$. 
%\end{definition}


\begin{definition}
\begin{enumerate}
\item We define the Taylor map at $\mathfrak{p}$ or order $s$ denote $ {T}_{\mathfrak{p},s}$ to be the $k$-algebra morphism induced by ${\eta_m^B}_C(\iota_{\mathfrak{p}, s})$ the  from $N_{s+1}({\mathfrak{p}})$ to $\mathcal{L}_1 (B)_{N_s( \mathfrak{p})}[t]/(t^2)$ where $\iota_{\mathfrak{p}, s}: \mathcal{L}_1 (B) \rightarrow \mathcal{L}_1 (B)_{N_s( \mathfrak{p})}$  the canonical map sending $b$ to $b \otimes1$.
\item We defined a $k$-linear map $\ell_s$ from $Im({T}_{\mathfrak{p},s})$ to ${\mathcal{L}_1(B)}_{N_s(\mathfrak{p})} $ sending $a+[t]b$ to $a+b$ and we refer to $\ell_s \circ {T}_{\mathfrak{p},s}$ that we denote $\tau_{\mathfrak{p}, s}$ as the $k$-linear Taylor map and we have $\ell_s \circ {T}_{\mathfrak{p},s}$. $\ell_s$ is a one-to-one map.
\end{enumerate}
\end{definition}

\begin{definition}
Any $\sigma: B \rightarrow B$ be an automorphism of the $R$-algebra $B$ such that for all $b \in B$, $\sigma ( b) - b \in  \mathfrak{p}$ induces an action $\widetilde{{\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}}$ on $Im({T}_{\mathfrak{p},s})$ define by $\widetilde{{\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}} ({T}_{\mathfrak{p},s} (x)) = {T}_{\mathfrak{p},s}( \sigma_s (x))$, for all $x \in B_{\mathfrak{p}}$. 
% ${T}_{\mathfrak{p},s}$ becomes a $G$-equivariant map and the following diagram is commutative
%$$ \xymatrix{ {\mathcal{L}_1(B)}_{N_s(\mathfrak{p})} \ar[rr]^{\mathcal{L}_1(\sigma)\otimes \sigma_s } &&  {\mathcal{L}_1(B)}_{N_s(\mathfrak{p})}\\
% Im({T}_{\mathfrak{p},s}) \ar[u]_{\ell_s}  \ar[rr]^{\widetilde{{\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}} } && \ar[u]_{\ell_s}  Im({T}_{\mathfrak{p},s}) \\
%N_{s+1}(\mathfrak{p})   \ar[u]_{{T}_{\mathfrak{p},s}} \ar[rr]^{\sigma_s} &&   \ar[u]_{{T}_{\mathfrak{p},s}}N_{s+1}(\mathfrak{p})
% } $$
% In particular, if $\mathcal{L}_1(\sigma)$  and $\sigma_s$ are the identity map then $ \widetilde{{\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}}$ is the identity map. 
\end{definition}
\begin{lemma} \label{tangent}
Let $k$ be a field, $B$ be a finitely presented $k$-algebra, and $\mathfrak{p}$ be a prime ideal of $B$. 
%We assume that $\mathfrak{p}$ is finitely generated,  and $k(\mathfrak{p})$ is separably generated over $k$. \\
Suppose $B= k [x_1 , \cdots ,  x_n]/ \mathfrak{a}$, $\mathfrak{a}$ is an ideal of $k [x_1 , \cdots ,  x_n] $.
%$\bullet$  $\mathfrak{p}$ is finitely generated,  and $k(\mathfrak{p})$ is separably generated over $k$. \\
%We have $B= k[\underline{x}]/\mathfrak{a}$ and $\mathfrak{p} = \mathfrak{P}/\mathfrak{a}$ where $\mathfrak{P}$ is is a prime ideal of $k[\underline{x}]$. %We suppose that $k(\mathfrak{P}) $ is separably generated over $k$.
\begin{enumerate}
\item $\widetilde{\varphi}_{s, B,\mathfrak{a}} :  {\mathcal{L}_1(B)}_{N_s(\mathfrak{p})} \rightarrow  N_s(\mathfrak{p})[ \underline{x}_1]/\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})})$  is the $R$-algebra isomorphism sending $[\underline{x}_0]_{ \mathcal{L}_s(\mathfrak{a})}\otimes c $ to $c [\underline{x}]_{\mathfrak{a}}$ and $[\underline{x}_i]_{ \mathcal{L}_s(\mathfrak{a})}\otimes c $ to $c[\underline{x}_i]_{ \overline{\mathcal{L}_s(\mathfrak{a})}}$ for all $i \in \{ 1, \cdots, s\}$ where  $\pi_{N_s(\mathfrak{p})} $ is the canonical map from $B[ (\underline{x}_i)_{1\leq i\leq s}]$ to $N_s(\mathfrak{p})[ (\underline{x}_i)_{1\leq i\leq s}]$, $\overline{ \mathcal{L}_s( \mathfrak{a})}= {\overline{\varphi}_{s, A , \mathfrak{a}}(  \mathcal{L}_s( \mathfrak{a})/ \mathfrak{a}_s)}$ and $\overline{\varphi}_{s, A , \mathfrak{a}}: \mathcal{L}_s( A)/\mathfrak{a}_s \rightarrow { B[ (\underline{x}_i)_{1\leq i\leq s}]}$  is the $R$-algebra isomorphism sending $[\underline{x}_0]_{\mathfrak{a}_s}$ to $[\underline{x}]_{\mathfrak{a}}$ and $[\underline{x}_i]_{\mathfrak{a}_s}$ to $\underline{x}_i$ for all $i \in \{ 1, \cdots, s\}$; We denote $\overline{\mathcal{L}_1(\sigma)\otimes \sigma_s}$ to be the map $\overline{\mathcal{L}_1(\sigma)\otimes \sigma_s} ( \widetilde{\varphi}_{s, B,\mathfrak{a}} (x) ) = \widetilde{\varphi}_{s, B,\mathfrak{a}} ( (\mathcal{L}_1(\sigma)\otimes \sigma_s) (x)) $, for all $x \in \mathcal{L}_1(B)_{N_s(\mathfrak{p})}$.
\item $\widetilde{\varphi}_{s, B,\mathfrak{a}} \circ \tau_{\mathfrak{p},s} : $ sends $[f]_{\mathfrak{a}}$ to $[ [f]_{\mathfrak{p}^s} +\sum_{i=1}^n  [ \frac{\partial }{\partial x_{i} } (f) x_{i,1}]_{\mathfrak{p}^s}  ]_{\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})})}$. 
\item $\ell_s$ is a one-to-one map.
 ${T}_{\mathfrak{p},s}$ becomes a $G$-equivariant map and the following diagram is commutative
$$ \xymatrix{ N_s(\mathfrak{p})[ \underline{x}_1]/\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})}) \ar[rr]^{\overline{\mathcal{L}_1(\sigma)\otimes \sigma_s} } && N_s(\mathfrak{p})[ \underline{x}_1]/\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})}) \\
{\mathcal{L}_1(B)}_{N_s(\mathfrak{p})}  \ar[u]^{\widetilde{\varphi}_{s, B,\mathfrak{a}} } \ar[rr]^{\mathcal{L}_1(\sigma)\otimes \sigma_s } && \ar[u]_{\widetilde{\varphi}_{s, B,\mathfrak{a}} } {\mathcal{L}_1(B)}_{N_s(\mathfrak{p})}\\
 Im({T}_{\mathfrak{p},s}) \ar[u]^{\ell_s}  \ar[rr]^{\widetilde{{\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}} } && \ar[u]_{\ell_s}  Im({T}_{\mathfrak{p},s})\\ N_{s+1}(\mathfrak{p})   \ar[u]^{{T}_{\mathfrak{p},s}} \ar[rr]^{\sigma_{s+1}} &&   \ar[u]_{{T}_{\mathfrak{p},s}}N_{s+1}(\mathfrak{p})
 } $$
 In particular, if $\mathcal{L}_1(\sigma)$  and $\sigma_s$ are the identity map then $ \widetilde{{\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}}$ is the identity map. 
\end{enumerate} 
\end{lemma} 
\begin{proof}
\begin{enumerate} 
\item is not hard to prove. 
\item follows from Lemma \ref{Nsp}. 
\item We denote  %$ [{f_\sigma}(\underline{x})]_{\mathfrak{a}}:= \sigma ([f(\underline{x})]_{\mathfrak{a}}) $ and  
$[{x_i}_\sigma (\underline{x})]_{\mathfrak{a}}= \sigma ([{x_i}]_{\mathfrak{a}})$. 
We obtain $$[{{x_i}_\sigma} ( \underline{x_0}+[t]_1 \underline{x_1})]_{\mathfrak{a}}=\left[ {{x_i}_\sigma}(\underline{x_0}) +\left( \sum_{i=1}^n    \frac{\partial}{\partial x_i} ({x_i}_\sigma(\underline{x_0})) x_{i,1} \right) [t]_1\right]_{\mathfrak{a}}$$
We have $ {\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}([x_{i,0}]_{\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})})}) = [ {{x_i}_\sigma}(\underline{x_{0}}) ]_{\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})})}$ and  \\ ${\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}([ x_{i,1}]_{\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})})}) =  [\sum_{i=1}^n    \frac{\partial}{\partial x_j} ({x_i}_\sigma({\underline{x_{0}}})) x_{j,1} ]_{\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})})}$.

By (2), we have  $\widetilde{\varphi}_{s, B,\mathfrak{a}} \circ \tau_{\mathfrak{p},s}  ( [f(\underline{x})]_{\mathfrak{a}}) = [[f(\underline{x})]_{\mathfrak{p}^s} + \sum_{i=1}^n    [\frac{\partial}{\partial x_i} (f(\underline{x}))]_{\mathfrak{p}^s} x_{i,1}]_{\overline{ \mathcal{L}_1( \mathfrak{a})}^{A/\mathfrak{p}}}$. Thus, this implies
$$\begin{array}{lll} &&{\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}(\widetilde{\varphi}_{s, B,\mathfrak{a}} \circ \tau_{\mathfrak{p},s}  ( [f(\underline{x})]_{\mathfrak{a}})))\\
&=&{\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}([[f(\underline{x})]_{\mathfrak{p}^s} + \sum_{i=1}^n    [\frac{\partial}{\partial x_i} (f(\underline{x}))]_{\mathfrak{p}^s} x_{i,1}]_{\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})})}) \\
&=&  [[f(\underline{{{x}_\sigma}}(\underline{x}))]_{\mathfrak{p}^s} + \sum_{i=1}^n    [\frac{\partial}{\partial x_i} (f(\underline{{{x}_\sigma}}(\underline{x})))]_{\mathfrak{p}^s} \sum_{j=1}^n    \frac{\partial}{\partial x_j} ({x_i}_\sigma(\underline{{x_{0}}})) x_{j,1}]_{\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})})}\\
&=& \widetilde{\varphi}_{s, B,\mathfrak{a}} \circ \tau_{\mathfrak{p},s} (f({{x}_1}_\sigma(\underline{x}), \cdots , {{x}_n}_\sigma(\underline{x}))) =\widetilde{\varphi}_{s, B,\mathfrak{a}} \circ \tau_{\mathfrak{p},s} ( \sigma ([f(\underline{x})]_{\mathfrak{a}})).
\end{array}$$
This proves the commutativity of the diagram. 
\end{enumerate} 
\end{proof}
%\begin{thm} 
%Let $k$ be a field. 
%We have $$\xymatrix{ 0 \ar[r] & \operatorname{Ker} (T_{\mathfrak{p}, s} ) \ar[r] & B_\mathfrak{p} \ar[r] & \mathcal{L}_1 (B)_{N_s( \mathfrak{p})}[t]/(t^2) }$$
%\end{thm} 
 \begin{thm} \label{mt}
Let $k$ be a field, $B$ be a finitely presented $k$-algebra, and $\mathfrak{p}$ be a prime ideal of $B$. 
We assume that $\mathfrak{p}$ is finitely generated,  and $k(\mathfrak{p})$ is separably generated over $k$. Then $T_{\mathfrak{p}, s}$ is a one-to-one. %$\operatorname{Ker} (T_{\mathfrak{p}, s} )=\operatorname{Ker} (\tau_{\mathfrak{p}, s} ) = \mathfrak{p}^{s+1}$.
%$\bullet$ $B= k [x_1 , \cdots ,  x_n]/ \mathfrak{a}$, $\mathfrak{a}$ is an ideal of $k [x_1 , \cdots ,  x_n] $, \\
%$\bullet$  $\mathfrak{p}$ is finitely generated,  and $k(\mathfrak{p})$ is separably generated over $k$. \\
%We have $B= k[\underline{x}]/\mathfrak{a}$ and $\mathfrak{p} = \mathfrak{P}/\mathfrak{a}$ where $\mathfrak{P}$ is is a prime ideal of $k[\underline{x}]$. We suppose that $k(\mathfrak{P}) $ is separably generated over $k$.
%The Taylor map $ {T}_{B, \mathfrak{a}, \mathfrak{p},s}$ is one-to-one. Moreover, given $\sigma: B \rightarrow B$ be an automorphism of the $R$-algebra $B$ such that for all $b \in B$, $\sigma ( b) - b \in  \mathfrak{p}$, ${T}_{1,B, \mathfrak{a}, \mathfrak{p}^s}$ makes the following diagram
%$$ \xymatrix{ B_\mathfrak{p}/ \mathfrak{p}^s  \ar[d]^{{T}_{1,B, \mathfrak{a}, \mathfrak{p}^s} } \ar[rr]^{\widetilde{\sigma}} &&  \ar[d]^{{T}_{1,B, \mathfrak{a}, \mathfrak{p}^s} }  B_\mathfrak{p}/ \mathfrak{p}^s  \\
% \mathcal{L}_1(B)_{\mathfrak{p}^s}\ar[rr]_{{\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}} / (\underline{x}_{1} )^2_{\mathfrak{p}^s}&& \mathcal{L}_1(B)_{\mathfrak{p}^s}/ (\underline{x}_{1} )^2_{\mathfrak{p}^s}
%}$$
%commute. In particular, $\mathcal{L}_1(\sigma)_{\mathfrak{p}^s} ( \operatorname{Im} ({T}_{1,B, \mathfrak{a}, \mathfrak{p}^s}))  \subseteq  \operatorname{Im} ({T}_{1,B, \mathfrak{a}, \mathfrak{p}^s})$. 
 %Moreover $\mathcal{L}_1(\mathfrak{p})_{ k(\mathfrak{p})}^2 = ( (x_{1,j}^2)_{0\leq j \leq 1})$. 
\end{thm} 
\begin{proof} 
We first prove that the result for $A= k [x_1 , \cdots ,  x_n]$. 

By Lemma \ref{tangent}, we obtain $
 \widetilde{\varphi}_{s, A, (0)} \circ \tau_{\mathfrak{p},s}: N_{s+1} ({\mathfrak{p}}) \rightarrow   N_s( \mathfrak{p}) [ \underline{x}_1]$ sending $[f]_{\mathfrak{p}^{s+1}} $ to $[f]_{\mathfrak{p}^s} + \sum_{i=1}^n   [\frac{\partial}{\partial x_i} (f)]_{\mathfrak{p}^s} x_{i,1}$. 
We have that $\operatorname{ker}( \widetilde{\varphi}_{s, A, (0)} \circ \tau_{\mathfrak{p},s}) = \{  f \in A | f \in\mathfrak{p}^{s} \text{ and } \frac{\partial}{\partial x_i} (f) \in \mathfrak{p}^{s} \}= \{ [0]_{\mathfrak{p}^{s+1}} \} $, by Lemma \ref{ss-1}.
 
 %Moreover, we have $\tau_{1,A, \mathfrak{p}, \widetilde{D}}$ induce a one-to-one map $\overline{\tau_{1,A, \mathfrak{p}, {D}}} : A_\mathfrak{p} /  \mathfrak{p}^2 A_\mathfrak{p} \rightarrow   (k( \mathfrak{p})  [ \underline{x}_1])/ (\underline{x}_{1} )^2_{k(\mathfrak{p})}$.


%We now consider the map $
%\overline{\tau_{1,A, \mathfrak{p}, {D}}} : A  /  \mathfrak{p}^2  \rightarrow   (A/ \mathfrak{p} [ \underline{x}_1])/(\underline{x}_{1} )^2_{\mathfrak{p}}$ sending $[f]_{ \mathfrak{p}^2 } $ to\\
% $[[f]_\mathfrak{p} + \sum_{i=1}^r  {D}_i(f) x_{i,1}]_{(\underline{x}_{1} )^2_{k(\mathfrak{p})}}$. 
%
%The following diagram is commutative 
%$$\xymatrix{  A/ \mathfrak{p}^2 \ar[rr]^{\overline{\tau_{1,A, \mathfrak{p}, {D}}} } \ar[d]_{\iota_\mathfrak{p}}  && (A/ \mathfrak{p} [ \underline{x}_1] )/(\underline{x}_{1} )^2_{\mathfrak{p}} \ar[d]^{\iota_\mathfrak{\pi_{0,1} ( \mathfrak{p} )}} \\
%A_\mathfrak{p}/  \mathfrak{p}^2 A_\mathfrak{p} \ar[rr]^{\overline{\tau_{1,A, \mathfrak{p}, \widetilde{D}}}} && (k( \mathfrak{p})  [ \underline{x}_1])/ (\underline{x}_{1} )^2_{k(\mathfrak{p})}}.$$
%
%Since $\iota_\mathfrak{\pi_{0,1} ( \mathfrak{p} )}$ and $\iota_\mathfrak{p}$ can be identified up to isomorphism to localization map at a multiplicative subset that does not contain $0$ nor zero divisor, those maps are injective. Chasing the diagram, we obtain that $\overline{\tau_{1,A, \mathfrak{p}, {D}}}$ is injective from the injectivity of $\overline{\tau_{1,A, \mathfrak{p}, \widetilde{D}}}$.

%We denote $\overline{T}_{B/ \mathfrak{p}^2} : B/ \mathfrak{p}^2 \rightarrow \mathcal{L}_1(B)_{ k(\mathfrak{p})}/ (x_{1,1}^2 , \cdots , x_{1,n}^2)_{k(\mathfrak{p})}$.
Now let us consider the general case. Let $\mathfrak{P}$ be a prime ideal of $B$. From the correspondence theorem for a prime ideal, we write $\mathfrak{P}= \mathfrak{p}/\mathfrak{a}$ where $\mathfrak{p}$ is a prime ideal of $ k[{\bf x}]$ containing $\mathfrak{a}$. 
We also have $A / \mathfrak{p}^s \simeq B/ \mathfrak{P}^s$. 

We now consider the map $
\widetilde{\varphi}_{s, B,\mathfrak{a}} \circ \tau_{\mathfrak{P},s} : N_{s+1}(\mathfrak{p}) \rightarrow   N_s(\mathfrak{p}) [ \underline{x}_1] /\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})})$ sending \\ 
$[[f]_{\mathfrak{a}}]_{\mathfrak{p}^{s+1}}$ to $[[f]_{\mathfrak{p}^s} + \sum_{i=1}^n    [\frac{\partial}{\partial x_i} (f)]_{\mathfrak{p}^s} x_{i,1}]_{\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})})}$. 
We prove that $  \operatorname{ker}(\widetilde{\varphi}_{s, B,\mathfrak{a}} \circ \tau_{\mathfrak{P},s})=\{ [[0]_{\mathfrak{a}}]_{\mathfrak{p}^{s+1}}\}$. To prove the result it is enough to prove that $( \widetilde{\varphi}_{s, A, (0)} \circ \tau_{\mathfrak{p},s})^{-1} ( \pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})})) = \{ [[0]_{\mathfrak{a}}]_{\mathfrak{p}^{s+1}}\}$. 
By definition of $\widetilde{\varphi}_{s, B,\mathfrak{a}} \circ \tau_{\mathfrak{P},s}$ and $\pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})})$, we have $( \widetilde{\varphi}_{s, A, (0)} \circ \tau_{\mathfrak{p},s})^{-1} (\langle \pi_{N_s(\mathfrak{p})} (\overline{ \mathcal{L}_s( \mathfrak{a})}) \rangle ) =( \widetilde{\varphi}_{s, A, (0)} \circ \tau_{\mathfrak{p},s})^{-1} ( \widetilde{\varphi}_{s, B,\mathfrak{a}} \circ \tau_{\mathfrak{P},s} ( \mathfrak{a})) =\{ [[0]_{\mathfrak{a}}]_{\mathfrak{p}^{s+1}}\}$. This proves that $ker(\widetilde{\varphi}_{s, B,\mathfrak{a}} \circ \tau_{\mathfrak{P},s})=\{ [[0]_{\mathfrak{a}}]_{\mathfrak{p}^{s+1}}\}$.


%That is $f({\bf x} ) = \sum_{k=1}^s r_{k}({\bf x} ) s_k ({\bf x} )$ where $r_k({\bf x} )\in  \mathfrak{p}$ and $ s_k ({\bf x} ) \in k[{\bf x}]$. We have $\partial f ({\bf x} )/ \partial {x_i} ({\bf x} )  = \sum_{k=1}^s ( \partial r_k / \partial {x_i}({\bf x} ) s_k ({\bf x} ) + r_{k}({\bf x} )( \partial s_k / \partial {x_i}({\bf x} ))$. 
%Since $\sum_{k=1}^sr_{k}({\bf x} )( \partial s_k / \partial {x_i}({\bf x} )) \in  \mathfrak{p} $, we obtain $\sum_{k=1}^s  \partial r_k / \partial {x_i}({\bf x} ) s_k ({\bf x} )\in \mathfrak{p}$.  Then $f({\bf x} )\in \mathfrak{p}^2$. 


%In any case, there I am assuming that k is perfect, if you prefer.
%In case of perfect field your question boils down to asking if p is regular in B. SO f\in p is also in p^2 if and only if d_j(f) \in p for all j. THIS is the jacobian criterion of regularity over an algebraically closed field and p maximal. If k is not algebraically closed and p is still maximal, just tensorize by overline{k} and you lose no information bevause of perfectness. If p is not maximal, then, you still tensorize with \overline{k} and then you choose a point \overline{p} that "lifts" p. \overline{p} is regular if and only if there is a maximal that contains that and it is regular; and in that case the maximal ideals that contain p with that property are an open subset of V(p), so you throw a closed subset and assume that all the maximal that contain p have that property. Then you write p as the intersection of all maximals that contain p (you can do that in the finitely gen case;  notice that we have the fin gen in L_1 \otimes B/q^2 just by assumning that q is fin gen in B, so it is bery mild condition that doesn not require that B is itself noetherian); morevover p^2 is the intersection of the squares of the maximal ideals. Thus if what i said holds for regular maximals it holds also for all the regular primes.

%$f = q p+r$
%
%$f=p(a, b) + (x-a) f_y(a,b) + (y-b) f_x(a,b)$. 

\end{proof} 
\begin{cor}\label{Lram}
 Let $k$ be a field, $B$ be a finitely presented $k$-algebra $\mathfrak{P}$ prime ideal of $B$, and $k(\mathfrak{p})$ is separably generated over $k$ and $\sigma: B \rightarrow B$ be an automorphism of the $k$-algebra $B$ such that for all $b \in B$, $\sigma ( b) - b \in  \mathfrak{P}$.  $\mathcal{L}_1 (\sigma ) \otimes \operatorname{id}_{\mathfrak{P}^s}|_{ \mathcal{L}_1(B)_{\mathfrak{p}^s}/ (\underline{x}_{1} )^2_{\mathfrak{p}^s}} = id_{\mathcal{L}_1(B)_{\mathfrak{p}^s}/ (\underline{x}_{1} )^2_{\mathfrak{p}^s}} $  if and only if for all $b \in B$, $\sigma (b)-b\in \mathfrak{P}^s$.  
\end{cor}
\begin{proof}
Suppose $ \sigma (b)-b\in \mathfrak{P}^s$, for all $b\in B$. That is, $\tilde{\sigma} = Id$. From the commutativity of the diagram in Theorem \ref{mt}, we obtain that $\mathcal{L}_1 (\sigma ) \otimes \operatorname{id}_{\mathfrak{P}^s}|_{ \mathcal{L}_1(B)_{\mathfrak{p}^s}/ (\underline{x}_{1} )^2_{\mathfrak{p}^s}} = id_{\mathcal{L}_1(B)_{\mathfrak{p}^s}/ (\underline{x}_{1} )^2_{\mathfrak{p}^s}} $. We prove the converse by contrapositive, we suppose that there exists $b \in B$ such that $\tilde{\sigma}(b) \neq b$ then again by the commutativity of the diagram in Theorem \ref{mt}, ${\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}(T_{1,B , \mathfrak{a},\mathfrak{p}^s} ( b))= {T}_{1,B, \mathfrak{a}, \mathfrak{p}^s}  ( \tilde{\sigma}(b)) \neq  {T}_{1,B, \mathfrak{a}, \mathfrak{p}^s}  ( b )$. Proving that $\mathcal{L}_1 (\sigma ) \otimes \operatorname{id}_{\mathfrak{P}^s}|_{ \mathcal{L}_1(B)_{\mathfrak{p}^s}/ (\underline{x}_{1} )^2_{\mathfrak{p}^s}} \neq id_{\mathcal{L}_1(B)_{\mathfrak{p}^s}/ (\underline{x}_{1} )^2_{\mathfrak{p}^s}} $
\end{proof}

\begin{cor}
 Let $B$ be a finitely presented algebra over $k$, $\mathfrak{p}$  be prime ideal of $B$, $s\in \mathbb{N}$ and $k(\mathfrak{p})$ is separably generated over $k$. We have $\mu_{0,1}^B (\mathfrak{p})$ is a prime ideal of $\mathcal{L}_1(B)$ and
$$G_{s}(\mathfrak{p}) = G_{s-1} (\mu_{0,1}^B (\mathfrak{p})) .$$
Moreover
$G_s (\mathfrak{p} ) =\cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(B) \cap V ( \mathfrak{p})} G_s (\mathfrak{m})$
and 
$G_s (\mu_{0,1}^B (\mathfrak{p}) ) =\cap_{\mathfrak{n} \in  \operatorname{Specm}_{\operatorname{sep}}(B) \cap V (\mathfrak{p} \mathcal{L}_1(B))} G_s (\mathfrak{n})=\cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(B) \cap V ( \mathfrak{p})} G_s (\mu_{0,1}^B (\mathfrak{m})) $.
\end{cor} 

\begin{proof} 
%Noting that $\mathcal{L}_1(B) \otimes_B k(\mathfrak{p}) \simeq \mathcal{L}_1(B)/\mu_{0,1}^B (\mathfrak{p})$. By Lemma \ref{irreduc}, we know that $\mathcal{L}_1(B) \otimes_B k(\mathfrak{p})$ is an integral domain. So that 
By Lemma \ref{irreduc}, we have $\mu_{0,1}^B (\mathfrak{p})$ is a prime ideal. By Corollary \ref{Lram}, we have that $G_{s}(\mathfrak{p}) = G_{s-1} ( \mu_{0,1}^B (\mathfrak{p})) .$
The equalities $G_s (\mathfrak{p} ) =\cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(B) \cap V ( \mathfrak{p})} G_s (\mathfrak{m})$
and 
$G_s (\mu_{0,1}^B (\mathfrak{p})) =\cap_{\mathfrak{n} \in  \operatorname{Specm}_{\operatorname{sep}}(B) \cap V (\mu_{0,1}^B (\mathfrak{p}))} G_s (\mathfrak{n})$ follow from Corollary \ref{specmsep}. The last equality follows from the fact $\mu_{0,1}^B (\mathfrak{p})  =\cap_{\mathfrak{m} \in  \operatorname{Specm}_{\operatorname{sep}}(B) \cap V ( \mathfrak{p})} \mu_{0,1}^B (\mathfrak{m})$ that is true since $\mu_{0,1}^B$ is injective. 
\end{proof} 


\begin{definition} 
Let $B$ be a $A$-algebra. We say that $B$ is a normal $A$-algebra. If $B$ is integrally closed over $A$ in $Frac(B)$. 
\end{definition} 
\begin{lemma}
\label{lem:locnormal}
Let $A$ be a Noetherian domain and let $A\subseteq B$ be a normal $A$-algebra. Then for $a\in A\backslash \{0\}$, $B_a$ is a normal $A_a-$algebra.
\end{lemma}
\begin{proof} Let $a\in A\backslash \{0\}$. 
We first prove that $B_a$ is integral over $A_a$. Let $\frac{b}{a^n}\in B_a$ where $b \in B$ and $n \in \mathbb{N} \cup \{ 0 \}$. Since $b\in B$, there exists a monic polynomial $\mu \in A[t]$ such that $\mu (b)=0$. We choose such a polynomial $\mu$. Then, the polynomial  $\displaystyle \mu_n(t) \colon = \frac{\mu (a^nt)}{a^{n\deg(r)}}\in A_a[t]$ is monic and vanishes in $\displaystyle \frac{b}{a^n}$. This concludes the proof. 

%For $b\in B$ there exist a monic polynomial $r \in A[t]$ such that $r (b)=0$. For $n\in \N$, the polynomial $\displaystyle r_n(t) \colon = \frac{r(a^nt)}{a^{n\deg(r)}}\in A_a[t]$ is monic and vanishes in $\displaystyle \frac{b}{a^n}$, therefore $B_a$ is integral over $A_a$.
On the other hand, given $c\in \Frac(B)$ and a monic polynomial $\lambda \in A_a[t]$ such that $\lambda (c)=0$, there exists $m\in \N$ such that the monic polynomial $\displaystyle \lambda_m (t)\colon = a^{m\deg(\lambda)}\cdot \lambda \left(\frac{t}{a^m}\right)$ has coefficients in $A$. Since $\lambda_m(a^m c)=a^{m\deg(\lambda)}\lambda(c)=0$, we infer that $a^mc\in B$, hence $c\in B_a$, which concludes our proof. 
\end{proof}
\begin{lemma}
\label{lem:densityfreealg}
Let $k$ be a field, then $\Specm_{\sep}(k[t_1,\dots,t_n])$ is dense in $\Spec(k[t_1,\dots, t_n])$.
\end{lemma}
\begin{proof}
It is enough to prove for any arbitrary $h\in k[t_1,\dots, t_n]\backslash \{0\}$ there exist \\
$\mathfrak{m}\in \Specm_{\sep}(k[t_1,\dots, t_n]_h)$. 
To prove this statement, we proceed by induction on $n$.
Clearly, if $n=1$, the result is true, because $k^{sep}$ is an infinite field and $h\neq 0$ has always a finite number of solutions.
Now assume that the result is true for all polynomials in $k[t_1,\dots,t_{n-1}]$. We prove the result for all polynomials in $k[t_1,\dots,t_{n}]$. Let $h \in k[t_1,\dots,t_{n}] \backslash \{ 0 \}$. We write
$$ h=\sum_{j=0}^m h_j x_n^j \, ,$$
where $h_j\in k[t_1,\dots, t_{n-1}]$ for all $0\leq j\leq m $. Since $h\neq 0$, we have $h_j\neq 0$ for some $j \in \{ 0 , \cdots , m\}$. Therefore, by inductive hypothesis, there are $\alpha_1,\dots,\alpha_{n-1}\in {k^{\sep}}$ such that $h_j(\alpha_1,\dots,\alpha_{n-1})\neq 0$; in particular the polynomial $h(\alpha_1,\dots,\alpha_{n-1}, t)\in k^{\sep}[t]$ is not $0$. Hence there is some $\alpha_{n}\in k^{\sep}$ such that $h(\alpha_1,\dots, \alpha_n)\neq 0$. Consider the morphism
\begin{align*}
\varphi_{\alpha} \colon k[t_1,\dots, t_n] &\rightarrow k^{\sep} \\
t_i & \mapsto \alpha_i \, .
\end{align*}
Let $\mathfrak{m}\colon = \ker(\varphi_{\alpha})$; then it is a maximal ideal with separable residue field since $k[t_1,\dots, t_n]/\mathfrak{m}$ embeds in $k^{\sep}$. Moreover $h\notin \mathfrak{m}$ as $h(\alpha_1,\dots,\alpha_n)\neq 0$. This concludes the proof.
\end{proof}



\begin{lemma} \label{seplemma}
Let $k$ be a field and $F/k(t_1,\dots, t_n)$ be a finite separable field extension. Let $\mathcal{O}_F$ be the integral closure of $k[t_1,\dots,t_n]$ in $F$. Then $\Specm_{\sep}(\mathcal{O}_F)$ is a dense subset of $\Spec(\mathcal{O}_F)$.
\end{lemma}

\begin{proof}
Since $F/k(t_1,\dots, t_n)$ is a finite separable extension, by the primitive element's theorem, there exists an irreducible polynomial $f\in k(t_1,\dots, t_n)[x]$ such that $F\cong k(t_1,\dots, t_n)[x]/(f)$; without loss of generality, we may assume that $f$ is monic with coefficients in $k[t_1,\dots, t_n]$, i.e. $F/k(t_1,\dots,t_n)$ is generated by an element $y\in \mathcal{O}_F$ such that $f(y)=0$.
Let $\iota \colon k[t_1,\dots, t_n][x]/(f) \hookrightarrow \mathcal{O}_F$ be the embedding of $k[t_1,\dots,t_n]-$algebras induced by the morphism of $k[t_1,\dots,t_n]-$algebras $k[t_1,\dots,t_n,x]\rightarrow \mathcal{O}_F$ sending $x$ to $y$. 
We tensor the following exact sequence by $k(x_1, \cdots, x_n)$ over $k[x_1, \cdots, x_n]$
$$ \xymatrix{ 0 \ar[r] & k[t_1 , \cdots , t_n] [x] / (x) \ar[r] & \mathcal{O}_F \ar[r] & \coker ( \iota) \ar[r] & 0 .} $$
Since the induced map 
$$\iota\otimes \mathbf{id}_{k(t_1,\dots,t_n)} \colon k(t_1,\dots, t_n)[x]/(f) \longrightarrow \mathcal{O}_F \otimes_{k[t_1,\dots, t_n]} k(t_1,\dots, t_n) \cong F $$
is an isomorphism, we obtain
$$\coker (\iota ) \otimes_{k[t_1,\dots, t_n]} k(t_1,\dots, t_n) = 0 .$$
Since $\mathcal{O}_F$ is a finitely generated over $k[t_1,\dots, t_n]-$module, there is $ g\in k[t_1,\dots,t_n]\backslash \{0\} $ such that $g\cdot \coker(\iota)=0$;
%Since 
%$$\iota\otimes \mathbf{id}_{k(t_1,\dots,t_n)} \colon k(t_1,\dots, t_n)[x]/(f) \tilde{\rightarrow} \mathcal{O}_F \otimes_{k[t_1,\dots, t_n]} k(t_1,\dots, t_n) \cong F $$
%is an isomorphism and since $\mathcal{O}_F$ is a finitely generated $k[t_1,\dots, t_n]-$module, we infer that there is $ g\in k[t_1,\dots,t_n]\backslash \{0\} $ such that $g\cdot \coker(\iota)=0$; 
in other words, $\iota$ induces also an isomorphism of $k[t_1,\dots, t_n]_g-$algebras $\iota_g \colon k[t_1,\dots, t_n]_g[x]/(f) \tilde{\rightarrow} \mathcal{O}_{F,g}$. Up to replacing $g$ with one of its multiples, we assume that the discriminant of $f$ divides $g$.  %\luigi{Maybe I don't really need this fact, so the above lemma can be canceled.}
Since $g\neq 0$, $\Spec(\mathcal{O}_{F,g})$ is a dense open subset of $\Spec(\mathcal{O}_F)$, therefore it is enough to prove that $\Specm_{\sep}(\mathcal{O}_{F,g})$ is dense in $\Spec(\mathcal{O}_{F,g})$ in order to achieve our conclusion.
For $\mathfrak{m}\in \Specm_{\sep}(k[t_1,\dots, t_n]_g)$, the residue field of any $\mathfrak{n}\in \Specm(\mathcal{O}_{F,g})$ containing $\mathfrak{m}$ is separable over $k$. Indeed we have that 
$$ \mathcal{O}_{F,g}/\mathfrak{m}\mathcal{O}_{F,g} \cong k[t_1,\dots, t_n]_g[x]/(f) \otimes_{k[t_1,\dots, t_n]_g} k(\mathfrak{m})=k(\mathfrak{m})[x]/(f(c_1,\dots,c_n,x))  \, , $$
where $c_i= t_i +\mathfrak{m}\in k(\mathfrak{m})$; since we assumed that the discriminant of $f$ divides $g$ and that $g\notin \mathfrak{m}$, we infer that $f(c_1,\dots,c_n,x)$ has distinct roots in a fixed algebraic closure of $k(\mathfrak{m})$, therefore $k(\mathfrak{n})/k(\mathfrak{m})$ is separable, which, in turns, means that $k(\mathfrak{n})/k$ is separable.
%Now let $D(h)\subseteq \Spec(\mathcal{O}_{F,g})$ be the nonempty basic open subset where 
%Let $h\in \mathcal{O}_{F,g}\backslash\{0\}$.
%%$U\subseteq \Spec(\mathcal{O}_{F,g})$ be a non-empty open subset; up to shrinking $U$ we may assume that its complement is $V(h)$ for some $h\in \mathcal{O}_{F,g}\backslash\{0\}$. 
%We write $h= h_1 \cdots h_s$, where $h_i$ are irreducible (possibly repeated), so that $\mathfrak{p}_i\colon = (h_i)\subseteq \mathcal{O}_{F,g}$ are non-zero prime ideals. Let $\mathfrak{q}_i=\mathfrak{p}_i\cap k[t_1,\dots, t_n]_g$; the composition of maps
%$$ k[t_1,\dots, t_n]_g\hookrightarrow \mathcal{O}_{F,g}\rightarrow k(\mathfrak{p}_i) \, ,$$
%with kernel $\mathfrak{q}_i$, induces an injection of fields $k(\mathfrak{q}_i)\subseteq k(\mathfrak{p}_i)$; since $\mathcal{O}_{F,g}$ is the integral closure of $k[t_1,\dots, t_n]_g$ in $F$ because of Lemma \ref{lem:locnormal}, it follows that $\trdeg(k(\mathfrak{q}_i))= \trdeg(k(\mathfrak{p}_i))<n$, hence $\mathfrak{q}_i\neq(0)$. Thus, the open set $V\colon = \Spec(k[t_1,\dots, t_n]_g)\backslash \overline{ \{\mathfrak{q}_1,\dots,\mathfrak{q}_s\} }$ is non-empty.
%Hence, by Lemma \ref{lem:densityfreealg}, we infer that there exists $ \mathfrak{m}\in V\cap\Specm_{\sep}(k[t_1,\dots, t_n]_g)$, therefore $\Specm_{\sep}(\mathcal{O}_{F,g})\cap \Spec ({\mathcal{O}_{F,gh}})$ is not empty, as it contains any $\mathfrak{n}\in \Specm(\mathcal{O}_{F,g})$ containing $\mathfrak{m}\mathcal{O}_{F,g}$.


Let $h\in \mathcal{O}_{F,g}\backslash\{0\}$. Noting that $\mathcal{O}_{F,g}$ is the integral closure of $k[t_1,\dots, t_n]_g$ in $F$ because of Lemma \ref{lem:locnormal}, we denote by $p(x)$ the minimal polynomial of $h$ over $k[x_1, \cdots , x_n]_g$. Since $p$ is irreducible, $p(0)\neq 0$. Hence, by Lemma \ref{lem:densityfreealg}, we infer that there exists $ \mathfrak{m}\in \Specm_{\sep}(k[t_1,\dots, t_n]_{g})$ such that $p(0) \notin  \mathfrak{m}$. For any $\mathfrak{n}\in \Specm(\mathcal{O}_{F,g})$ containing $\mathfrak{m}\mathcal{O}_{F,g}$, then $h \notin \mathfrak{n}$, concluding the proof. %use contraction: $p(h)=h \cdot q(h) + p(0)\in \mathbb{n}$ 

\end{proof}


\begin{lemma} \label{birational} Let $A$ (resp. $B$) be an algebra over finite type over $k$ that is also integral domains. Suppose that we have two embedding $\iota_A : A \rightarrow F$ (resp. $\iota_B : B \rightarrow F$) inducing isomorphism $\widetilde{\iota_A }: Frac(A) \rightarrow F$ (resp. $\widetilde{\iota_B}: Frac (B) \rightarrow F$), when localizing at $(0)$ such that $\iota_A  = \widetilde{\iota_A } \circ \nu_A$ (resp. $\iota_B  = \widetilde{\iota_B } \circ \nu_B$) where $ \nu_A : A \rightarrow Frac(A) $ (resp. $ \nu_B : B \rightarrow Frac(B) $) is the canonical localization morphism . Then there is $c \in A$ and $ d \in B$ such that $A_c \simeq B_d$. 
 \end{lemma} 
 \begin{proof} Since by assumption $A$ and $B$ are algebras over finite type over $k$, we can consider two surjections $\phi_A : k[(x_i)_{i \in I}] \rightarrow A$ and $\phi_B : k[(y_j)_{j \in J}] \rightarrow B$. Up to removing generators, we assume none of the $x_i$ or $y_j$ goes to $0$ via those maps. $A'=\iota_A(A)$ (resp. $B' = \iota_B(B))$ are subring of $F$ isomorphic to $A$ (resp. $B$). We have $Frac( A')= Frac(B')= F$. 
Now $\iota_A \circ \phi_A (x_i) = \frac{f_i}{g_i}$, for some $f_i$, $g_i$ in $B'$ with $g_i \neq 0$, for all $i \in I$ and  $\iota_B \circ \phi_B (y_j) = \frac{p_j}{q_j}$, for some $p_j$, $q_j$ in $A'$ with $q_j \neq 0$, for all $j \in J$. 
Let $b$ in $B'$ be the product of $\prod_{i \in I} g_i$ and $a$ in $A'$ the product $\prod_{j \in J}q_j$. We note that by assumption, neither $a$ nor $b$ is zero.
Therefore, by the universal property of localization, we have an embedding $\iota_{A'} : A' \rightarrow B'_b$ and $\iota_{B'} : B' \rightarrow  A'_a$, so that $b \in A'_a$ and $a \in B'_b$.  Thus, by the universal property of localization, we deduce that there are two embedding $\iota_{A'_a} :  A'_a \rightarrow (B'_{b})_{\frac{a}{1}}$ and $\iota_{B'_b} :B'_b \rightarrow  (A'_{a})_{\frac{b}{1}}$. Again, by the universal property of the localization, we can deduce the existence of an embedding  $\iota_{(A'_{a})_{\frac{b}{1}}} : (A'_{a})_{\frac{b}{1}} \rightarrow (B'_{b})_{\frac{a}{1}}$ and an embedding  $\iota_{(B'_{b})_{\frac{a}{1}}} : (B'_{b})_{\frac{a}{1}}\rightarrow (A'_{a})_{\frac{b}{1}}  $ that are inverses of each other proving the result.

%$\iota_A$ (resp. $\iota_B$) induces canonical localization morphism $\overline{\iota_A}^b: A_{\iota_A^{-1} (b)a} \rightarrow B_{b\iota_B^{-1} (a)}$ (resp. $\overline{\iota_B}^a: B_{b\iota_B^{-1} (a)} \rightarrow A_{\iota_A^{-1} (b)a}$) such that $ i_b \circ \overline{\iota_A}^b = \iota_A$ (resp. $ i_a \circ \overline{\iota_B}^a = \iota_B$), $i_b : B_b \rightarrow F$ (resp. $i_a : A_a \rightarrow F$) are the canonical localization morphism. Those morphisms are inverse of each others, proving the result.

%A c B_b c F (resp. B c A_a c F).

%Since A c B_b, a is an element of B_b, and b is an element of A_a.

%So consider A_(ab) and B_(ab). They are isomorphic.
\end{proof} 

%
%\begin{lemma} 
%
%\end{lemma}
%\begin{proof}
%For any $N_s(\mathfrak{p})$-algebra $C$, 
%we have $$\begin{array}{lll} \operatorname{Hom}_k( \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p}) , C)   \simeq Der_{k} ( N_{s+1}(\mathfrak{p}) , C) \,  \\
%%&\simeq & \{\psi \in \operatorname{Hom}_k(B, C[t]/(t^{2}))  \colon \mathfrak{p}= \psi^{-1}(\overline{t} C[t]/(t^{2})) \text{ and } p_1^B ( \psi (B \backslash \mathfrak{p}) ) \subseteq C^\times \} \, 
% \end{array}$$
%  $\mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p})$ is a $N_s(\mathfrak{p})$-algebra. Thus 
%  $$\begin{array}{lll} \operatorname{Hom}_k( \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p}) , \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p}))   \simeq Der_{k} ( N_{s+1}(\mathfrak{p}) , \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p})) \,  \\
%%&\simeq & \{\psi \in \operatorname{Hom}_k(B, C[t]/(t^{2}))  \colon \mathfrak{p}= \psi^{-1}(\overline{t} C[t]/(t^{2})) \text{ and } p_1^B ( \psi (B \backslash \mathfrak{p}) ) \subseteq C^\times \} \, 
% \end{array}$$
% Therefore we know that there is a $k$-derivation from $N_{s+1}(\mathfrak{p}) $ to $\mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p})$  that is the image of $id_{\mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p})}$ by the bijection above. We denote this derivation $D_s$. 
%
% 
%
% 
%
%%$$ \xymatrix{ \operatorname{Hom}_k( \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p}) , \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p})) \ar[d]^{} \ar[rr]_{{\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}} &&  \ar[d]^{}  \operatorname{Hom}_k( \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p}) , \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p}))) \\
%%Der_{k} ( N_{s+1}(\mathfrak{p}) , \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p}))  \ar[rr]_{{\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}}^{\widetilde{\sigma}}&&Der_{k} ( N_{s+1}(\mathfrak{p}) , \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p})) 
%%}$$
%$$\mathscr{M}_s :=\{\psi \in \operatorname{Hom}_k(B, C[t]/(t^{2}))  \colon  \tau_{0,s}^B \circ \psi= \eta \circ \zeta_{\mathfrak{p},s}  \} .$$
%
%%$$ \xymatrix{ \operatorname{Hom}_k( \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p}) , \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p})) \ar[d]^{} \ar[r]_{} &   \mathscr{M}_s  \ar[r]_{} &  Der_{k} ( N_{s+1}(\mathfrak{p}) , \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p}))   \ar[dd]^{\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}}  \\
%%\mathscr{M}_s \ar[d] && \\
%%Der_{k} ( N_{s+1}(\mathfrak{p}) , \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p}))  \ar[rr]_{}^{\widetilde{\sigma}}&&Der_{k} ( N_{s+1}(\mathfrak{p}) , \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p})) 
%%}$$
%%
%%$$\xymatrix{ \operatorname{Hom}_k( \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p}) , \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p}))  \ar[r] 
%%
%%$\psi= \psi_0 + \psi_1 [t]$ sends to $\tilde{\psi_1}\circ \tilde{\sigma}$ on the one hand and to $\mathcal{L}_1(\sigma)_{\mathfrak{p}^s}\circ  \tilde{\psi_1}$.
%%  
%% We should be able to prove that $f \in \mathfrak{p}^{s}$ and $D_s(f) \in  \mathfrak{p}^{s}\mathcal{L}_1 (B) \otimes_B N_{s}(\mathfrak{p})$ if and only if $f \in \mathfrak{p}^{s+1}$. 
%% 
%% Consider $\overline{D_s} : N_{s+1}(\mathfrak{p}) \rightarrow \mathcal{L}_1 (B) \otimes_B N_s(\mathfrak{p})/\mathfrak{p}^{s}\mathcal{L}_1 (B) \otimes_B N_{s}(\mathfrak{p})$. 
% 
% %We should be able to prove that $\operatorname{ker}(\overline{D_s}) = \mathfrak{p}^{s}/ \mathfrak{p}^{s+1}$. 
%\end{proof} 


\begin{lemma}
Let $R$ be a formally smooth ring and $P$ a prime ideal of its such that $k(P)/k$ is separably generated. Let $f\in P$ be such that for any derivation $D\colon R\rightarrow R/P$, $D(f)=0$. Then $f\in P^2$.
\end{lemma}

\begin{proof}
Let $P/P^2=\langle \overline{g}_i \colon i\in I \rangle_R$ and let $f+P^2= \sum_{i\in I} a_i \overline{g}_i$, where $\{i\in I\colon a_i\neq 0\}$ is finite. So, denoting, for all $i\in I$, $g_i\in P$ an element such that $g_i+P^2= \overline{g}_i$, we write $f=f'+\sum_{i\in I} a_i g_i$ for some $f'\in P^2$. Our statement holds true if we prove that $a_i\in P$ for all $i\in I$. 
Now,
$$ \forall D\in \Der_R(R, R/P) \quad D(f)=\sum_{i\in I} a_i D(g_i) \, . $$
\end{proof}




\begin{lemma}
Let $B$ be an arbitrary $k-$algebra. Then there is an inductive system of finitely generated $k-$algebras $\{B_\lambda\}_{\lambda\in \Lambda}$, for some set of indices $\Lambda$, such that $B=\varinjlim_{\lambda\in \Lambda} B_\lambda$ and all the maps of the form $B_\lambda\rightarrow B_{\lambda'}$ or $B_\lambda\rightarrow B$ are injective.
\end{lemma}

\begin{proof}
$B$ is the union of all its finitely generated subalgebras.
\end{proof}


\luigi{What does it tell us in terms of Taylor maps?}



















==> chapters/ramify__sophie_marques_s_conflicted_copy_2022-12-21_.tex <==
\section{Characterization of the ramification}
Let $k$ be a field and let $B$ be a $k-$algebra. 
%\begin{lemma}[Cohen structure theorem, equicharacteristic case]
%\luigi{A reference could be stack project 10.160.8, even if they write the statement without assuming equicharacteristic.}
%Let $(R, \mathfrak{m})$ be a Noetherian complete local ring containing a field. Let $K$ be the residue field of $R$, then $R$ is isomorphic to $K[[x_1,\dots, x_n]]/I$ for some $n\in \N$ and some ideal $I$.
%\end{lemma}
%
%\begin{cor}
%\label{cor:CohenStructQuot}
%Let $(R, \mathfrak{m})$ be a Noetherian complete local ring containing a field. Let $K$ be the residue field of $R$, then exist $n\in \N$ and $I$ ideal in $K[[x_1,\dots, x_n]]$ such that $\forall m\in \N$, we have that $R/\mathfrak{m}^{m+1}\cong K[x_1,\dots, x_n]/(I+(x_1,\dots, x_n)^{m+1})$.
%\end{cor}
%
%\begin{proof}
%\luigi{I'll write a proof later.}
%\end{proof}
\sophie{ to be decided if it is true 
\begin{lemma}
Let us fix a prime ideal $\mathfrak{p}$ of $B$ and $s, t \in \mathbb{N}^\ast$ where $s \leq t$. Then, 
%we have a canonical morphism $\overline{\mu_{s,t}} : J_s(B)_
$ \pi_s$ is an isomorphism if and only if $\mu_{s, s+1}$ is an isomorphism.  
\end{lemma} 
\begin{remark} Let $B$ be an etale $R$-algebra. Let us fix a prime ideal $\mathfrak{p}$ of $B$ and an automorphism $\sigma \colon B\rightarrow B$ of $k-$algebras.  The following statement is equivalent. 
\begin{enumerate} 
\item $\sigma(b) - b \in \mathfrak{p}$, for all $b \in b$;
\item $\sigma(b) - b \in \mathfrak{p}^{s+1}$, for all $b \in b$;
\item $\sigma$ induces a automorphism on the completion of $B_\mathfrak{p}$ and this automorphism is trivial;
\item $\sigma$ induces a automorphism on the localization $B_\mathfrak{p}$ and this automorphism is trivial.
\end{enumerate}
Indeed, $(2)$ is equivalent to $(3)$ since the completion of $B_\mathfrak{p}$ is the inverse limit of the inverse system defined by $B/\mathfrak{p}^{s+1}$ and $\pi_s$. 
\begin{itemize}
\item {\bf Case 1: } $R$ is a field. In this case, since $B$ is étale, it is a product of finite field extensions of $R$. In this case, all the positive powers of a prime in $B$ coincide with the prime itself. So being trivial $\mod \mathfrak{p}$ is the same trivial mod $ \mathfrak{p}^{s+1}$ for all $s$ natural numbers.
\item {\bf Case 2:} B local, i.e. There is only one prime over $ \mathfrak{q} \in \operatorname{Spec} (R)$ and we have $\mathfrak{q}B= \mathfrak{p}$, by Definition of Etale (see Liu  Definition 3.17.) We denote $\widehat{B}$ (resp. $\widehat{R}$) the completion of $B$ (resp. $R$) and $g: R\rightarrow B$ is structural $R$-algebra morphism. By assumption, $\sigma$ is an automorphism of $B$ as $R$-algebra that is the identity on $B/\mathfrak{p}$.\\
{\bf Case 2.1:} $R$ contains a field $K$. Then both $\widehat{R}$ and $\widehat{B}$ are $K$-algebras. $\widehat{R}$ is a $k(\mathfrak{p})$-algebra and $\widehat{B}$ is a $k(\mathfrak{p})$-algebra. By Liu Prop 3.26, we have $\widehat{B}$ is equivariantly isomorphic to $ \widehat{R} \otimes_{k(\mathfrak{q})} k(\mathfrak{p})$ where the induced action of $\sigma$ on $ \widehat{R} \otimes_{k(\mathfrak{q})} k(\mathfrak{p})$ is trivial on $R$ and $k(\mathfrak{p})$. Therefore, the induced action of $\sigma$ on $B$ induces a trivial action on $\widehat{B}$ equivalently $(2)$ is satisfied from the above. \\
{\bf Case 2.2:} $R$ does not contain a field $K$.
\end{itemize}
In particular for any $G$ subgroup of $Aut_R(B)$ and $s \in \mathbb{N}^\ast$, we have $G_0(\mathfrak{p})=G_s(\mathfrak{p})$.
\end{remark} 
}
\begin{lemma}
\label{lem:Gmtofibre}
Let us fix a prime ideal $\mathfrak{p}$ of $B$, $s \in \mathbb{N}^\ast$ and an automorphism $\sigma \colon B\rightarrow B$ of $R-$algebras such that for all $b \in B$, $\sigma (\mathfrak{p}) =\mathfrak{p}$ and  $\sigma (b)\in b \in \mathfrak{p}$. If for all $b \in B$, $\sigma(b)- b \in \mathfrak{p}^{s+1}  \, $ then $\underline{J_m(\sigma ) \sigma \otimes \operatorname{id}_{k(\mathfrak{p})}}|_{\underline{J_m(B)}_\mathfrak{p}}$  $=\operatorname{id}_{\underline{J_m(B)}_\mathfrak{p} }$ for all $m\leq s$. %acts trivially on $\mathcal{L}_s(B)\otimes_B$ $k(\mathfrak{p})$ 
%if and only if for all $b \in B$, $\sigma(b)\equiv b \pmod{\mathfrak{p}^{s+1}}  \, .$
\end{lemma}

\begin{proof} 


%Suppose $B= k [ x_1, \cdots, x_n]/ I$.  %Let $\mathfrak{p}$ a be a prime ideal of $B$ we have that there is a $\mathfrak{q}$ prime ideal of $ k [ x_1, \cdots, x_n]$ such that $I \subseteq \mathfrak{q}$ and $\mathfrak{p}=\frac{\mathfrak{q}}{I}$.
%We have that, for all $b \in B$, 
%$$\sigma^\ast\psi(b) = \psi(b) + \psi(\sigma(b)-b) \, . $$
Let $C$ be a $k$-algebra, $\psi\in \underline{J_m(B)}_\mathfrak{p}(C)$ and $b \in B$. In particular, we have \\ $\psi \in  \operatorname{Hom}_k(B, C[t]/(t^{m+1}))$ and $\psi(\mathfrak{p})\subseteq \overline{t} C[t]/(t^{m+1})$. Therefore $\psi(\mathfrak{p}^{m+1})\subseteq \overline{t}^{m+1} C[t]/(t^{m+1}).$
Thus, if  $\sigma( b )- b \equiv 0 \pmod{\mathfrak{p}^{m+1}} $, then 
$\psi ( \sigma( b )- b) = 0 $ for all $\psi\in \underline{J_s(B)}_\mathfrak{p}(C)$. 
%

%Let $\{f_i\colon i\in I\}$ be a set of generators of $\mathfrak{p}$.

%Then, there is a polynomial $p^{b}=\sum_{r=s+1}^{m} p_r^b\in B [(x_i)_{i\in I}]$, where $p_r^b$ is either $0$ or a homogeneous polynomial of degree $r$, such that $\sigma(b)-b=p^b((f_i)_{i\in I})$; it follows that 
%$$ \psi(\sigma(b)-b) = \widetilde{p^b}((\psi(f_i))_{i\in I}) \, , $$
%where, for a polynomial $g= \sum_{J \mbox{ multiindex}} a_J\underline{x}^J \in B[\underline{x}]$, we set $\widetilde{g} = \sum_{J \mbox{ multiindex}} \psi(a_J)\underline{x}^J \in \left( C[t]/(t^{s+1}) \right)[\underline{x}]$.
%Since $f_i \in \mathfrak{p}$, there is $u_i\in C[t]/(t^{s+1})$ such that $\psi(f_i)=\overline{t} u_i$, hence 
%$$ \forall r\geq s+1, \quad  \widetilde{p_r}^b((\psi(f_i))_{i\in I})= \widetilde{p_r^b}((\overline{t}u_i)_{ i\in I})=\overline{t}^r \widetilde{p_r^b}((u_i )_{i\in I})=0 \, ,$$
%therefore $\psi(\sigma(b)-b)=0$ and $\sigma^\ast(\psi)=\psi$.
%
%For the other direction, let us first consider the case where $B$ is a Noetherian algebra.
%Now assume that $\exists b\in B$ such that $\sigma(b)-b \in \mathfrak{p}^m\backslash \mathfrak{p}^{m+1}$ for some $m\leq s$. Consider the composition of morphisms
%$$ B \rightarrow B_\mathfrak{p} \rightarrow \widehat{B_\mathfrak{p}} \rightarrow k(\mathfrak{p})[x_1,\dots, x_n]/(I+ (x_1,\dots, x_n)^{m+1}) \, , $$
%where the first one is the localisation with respect to the prime $\mathfrak{p}$, the second one is the $\mathfrak{p}-$adic completion and the last one is given by \ref{cor:CohenStructQuot}.
%Since $\sigma(b)-b\in \mathfrak{p}^m\backslash \mathfrak{p}^{m+1}$, the composition above sends it to a non-zero element $f	\in (x_1,\dots, x_n)^m$.
%
%%Now notice that if $\dim B \geq 1$, then $\bigcap_{m>0} \mathfrak{p}^m$
%
%% We can write $ \sigma(b)-b = \sum_{r = d}^m p_r((f_i)_{i\in I}) $ for some integers $d \leq s$ and $m$ and homogeneous polynomials $p_r\in B\backslash \mathfrak{p}[(x_i)_{i\in I}]$ such that $\forall d\leq r\leq m, \, \deg(p_r)=r$, where the degree is given by $\deg(x_i)= v_{\mathfrak{p}}(f_i)\geq 1$, for $i\in I$. Let $\overline{p_r}\in k(p)[(x_i)_{i\in I}]$ be the reduction of $p_r$ modulo $\mathfrak{p}$; by construction $\overline{p_d}\neq 0$. Since $p_d$ is a polynomial, it depends on a finite number of variables, that we call $\{x_1,\dots, x_n\}$.
%
%\luigi{Now I start sharing a vague idea, maybe we can turn this into a proof. I will assume $B$ to be of finite type, because extending to the general case is subtler than I tought (and there are weird cases, like: for all m, $y_m= polynomial(y_{m+1})$).}
%
%Say that $B=k[y_1,\dots, y_N]/\Omega$, with $y_1=f_1, \dots, y_n=f_n$. Fix an algebraic closure $F$ of $k(p)$. Let us find $a=(a_1,\dots, a_N)\in V(\Omega)\subseteq \mathbb{A}^N(F)$ such that $\overline{p_d}(f_1(a),\dots, f_n(a))\neq 0$. \luigi{We have to prove that $\overline{p_d}(f_1,\dots,f_n)\notin \sqrt{\Omega}$, *OR* maybe work over some infinitesimal extension of $F$ and prove that it does not belong to $\Omega$}
%
%Consider the map $\psi\colon B \rightarrow F[t]/(t^{s+1})$ sending $y_j\mapsto y_j+\mathfrak{p} + t a_j$ (Here it seems useful an assumption on the possibility of choosing all the $f_j$ in $p\backslash p^2$ (so the $v_p(f_j)=1$ for all $j$, but maybe for this we need B regular at p, maybe not). Then  $\sigma^\ast\psi(b)=\psi(b)+\psi(\sigma(b)-b)$ and 
%$$ \psi(\sigma(b)-b) \cong p_d((f_j(a))_j) \pmod t^{d+1} $$
%so it is not 0.
%
%\luigi{stopped here, many gaps to fill.}
\end{proof}

\luigi{A thickened version of the previous lemma. Seems useful for $G_2$ when m=1, s=2}.

\begin{lemma}
Let us fix a prime ideal $\mathfrak{p}$ of $B$, $s \in \mathbb{N}^\ast$ and an automorphism $\sigma \colon B\rightarrow B$ of $R-$algebras such that for all $b \in B$, $\sigma (\mathfrak{p}) =\mathfrak{p}$ and  $\sigma (b)\in b \in \mathfrak{p}$. If for all $b \in B$, $\sigma(b)- b \in \mathfrak{p}^{s+1}  \, $ then 
$$\underline{J_m(\sigma)}|_{\underline{J_m(B)}_{B/\mathfrak{p}^{s-m+1}}} =\operatorname{id}_{\underline{J_m(B)}_{B/\mathfrak{p}^{s-m+1}} }$$
for all $m\leq s$.
\end{lemma}

\begin{proof}
Given an arbitrary $R-$algebra $C$ and $\psi\in \underline{J_m(B)}_\mathfrak{p}(C)$, we have that 
$$\psi(\mathfrak{p})\subseteq (t)+\left( \iota^C_m(\tau_{m,0}(\psi(\mathfrak{p}))) \right)  \, ,$$
therefore
$$\psi(\mathfrak{p}^{s+1})\subseteq \sum_{j=0}^{s+1} (t^j)\left( \iota^C_m(\tau_{m,0}(\psi(\mathfrak{p}^{s-j+1}))) \right) \, .$$

Clearly $\tau_{m,0}(\psi(\mathfrak{p}^{s-m+1}))=0$, therefore $\iota^C_m(\tau_{m,0}(\psi(\mathfrak{p}^{s-j+1})))=0$ for $j\leq m$, while for $j>m$ we have that $t^j=0$.
It follows that $\psi(\mathfrak{p}^{s+1})=0$.

Hence, for all $b\in B$ we have that
$$ \underline{J_m}(\sigma)(\psi)(b)= \psi(\sigma(b))= \psi(b)+ \psi(\sigma(b)-b)=\psi(b)  \, , $$
where the last equality follows from the assumption that $\forall b\in B$, $\sigma(b)-b\in \mathfrak{p}^{s+1}$.
\end{proof}

\luigi{This is the "other arrow" according to my promise in the file that i sent. The above thing implies that, given $\sigma\in G_s(p)$ then for all m, for all $q\in \Spec (L_m(B) \otimes k(p)) \subseteq \Spec (L_m(B) \otimes B/p^{s-m+1})$, then $L_m(\sigma)\in G_{s-m+1}(q)$.}

\begin{lemma}
\label{lem:redfibretoG1}
  Let $k$ be a field, $B$ be a local Noetherian $k$-algebra with maximal ideal $ \mathfrak{m}$, and $\sigma: B \rightarrow B$ be an automorphism of the $k$-algebra $B$ such that for all $b \in B$, $\sigma ( b) - b \in  \mathfrak{m}$. If $\mathcal{L}_1 (\sigma ) \otimes \operatorname{id}_{k(\mathfrak{m})}|_{ \mathcal{L}_1(B)_{ \mathfrak{m}, red}} = id_{ \mathcal{L}_1(B)_{ \mathfrak{m}, red}} $. Then for all $b \in B$, $\sigma (b)-b\in \mathfrak{m}^2$.  
\end{lemma}

\begin{proof} 
Assume that there is $b \in B$, $\sigma ( b) - b \in B \backslash  \mathfrak{m}^2$. We first note that we have $\sigma ( b) - b \in \mathfrak{m} \backslash  \mathfrak{m}^2$. Indeed, by assumption $\sigma ( b) - b \in \mathfrak{m}$. We will prove that $ \mathcal{L}_1(\sigma)|_{\mathcal{L}_1(B)_{ \mathfrak{m}, red}} \neq id_{ \mathcal{L}_1(B)_{ \mathfrak{m}, red}}$. \\
For this, it is enough to prove that there is $C$ reduced $k(\mathfrak{m})$-algebra and a $k(\mathfrak{m})$-algebra morphism $\Psi: B\rightarrow C[t]/(t^2)$ such that $\Psi^{-1} ((t)/ (t)^2)= \mathfrak{m}$, ${\tau}^B_{1,0} (\Psi(B \backslash \mathfrak{m}) ) \subseteq C^\times$ and $\Psi \circ \sigma \neq \Psi$. Given such $\Psi$, $\Psi  ( \mathfrak{m}^2) =0$, thus $\Psi$ descends to a morphism $\widetilde{\Psi}:  B/\mathfrak{m}^2\rightarrow C[t]/(t^2)$  such that $\widetilde{\Psi}^{-1} ( (t)/ (t)^2 ) = \mathfrak{m}/\mathfrak{m}^2$ and ${\tau}^B_{1,0}  (\widetilde{\Psi} ((B/\mathfrak{m}^2) \backslash (\mathfrak{m}/\mathfrak{m}^2)) ) \subseteq C^\times$. Conversely, given $\widetilde{\Psi} : B/ \mathfrak{m}^2 \rightarrow  C[t]/(t^2)$ such that $\widetilde{\Psi}^{-1} ( (t)/ (t)^2 ) = \mathfrak{m}/\mathfrak{m}^2$ and ${\tau}^B_{1,0}  (\widetilde{\Psi} ((B/\mathfrak{m}^2) \backslash (\mathfrak{m}/\mathfrak{m}^2)) ) \subseteq C^\times$, then there is $\Psi: B \rightarrow  C[t]/(t^2)$ such that $\Psi = \widetilde{\Psi} \circ \pi_{0, 2}$ where $\pi_{0, 2} : B \rightarrow  {B}/{ \mathfrak{m}^2}$ is the canonical quotient map. We have that the canonical projection map $\pi_{2, 1}: {B}/{ \mathfrak{m}^2} \rightarrow {B}/{ \mathfrak{m}}$ is not an isomorphism. Indeed, if $\pi_{2,1}$ is an isomorphism then $\mathfrak{m}=\mathfrak{m}^2$ and ${B}/{ \mathfrak{m}^2}= {B}/{ \mathfrak{m}}$. So, the action induced by $\sigma$ on ${B}/{ \mathfrak{m}^2}$ is trivial, but this contradicts our assumption. \\
By Cohen theorem (see \cite[Theorem 10.160.8]{stack}), since $B$ is noetherian, we have $B/ \mathfrak{m}^2$ noetherian and the $\mathfrak{m}$-adic completion of $\widehat{B/ \mathfrak{m}^2} \simeq B/ \mathfrak{m}^2$, we have that $B/ \mathfrak{m}^2$ is a $k(\mathfrak{m})$-vector space.
Since $\pi_s$ is not an isomorphism and $ \mathfrak{m}/\mathfrak{m}^2$ is a $k(\mathfrak{m})$-vector space,. We have the direct sum decomposition $B/ \mathfrak{m}^2= k( \mathfrak{m})\cdot 1 \oplus \mathfrak{m}/\mathfrak{m}^2$. Indeed, given $\alpha \in B/ \mathfrak{m}^2$, then $\alpha - \pi_{0, 1} ( \alpha) \cdot 1 \in  \mathfrak{m}/\mathfrak{m}^2.$ %Moreover, clearly we have the direct sum decomposition $ \mathfrak{m}/\mathfrak{m}^2 = k( \mathfrak{m}) \cdot (\sigma (b) -b) \oplus V(\mathfrak{m})$ for some $k( \mathfrak{m})$-subspace $V(\mathfrak{m})$. 
We choose $\mathcal{B}=\{ \sigma (b) -b , b_i \}_{i \in I}$ to be a base for $ \mathfrak{m}/\mathfrak{m}^2 $ over $k( \mathfrak{m})$. 
%there is some non-zero element $x_1, \cdots, x_r\in \mathfrak{p}$ that generates 
%then ${\mathfrak{p}}/{\mathfrak{p}^2}$ is a $k( \mathfrak{p})$-vector subspace of the $k( \mathfrak{p})$-vector space $B/ \mathfrak{p}^2$. So that, $\mathfrak{p}/\mathfrak{p}^2$ is a direct summand of $B/ \mathfrak{p}^2$. We write $B/ \mathfrak{p}^2=\mathfrak{p}/\mathfrak{p}^2 \oplus V( \mathfrak{p})$. 
We construct 
$$ \begin{array}{llll} \widetilde{\Psi}: &B / \mathfrak{m}^2 & \rightarrow & F[t]/ (t^2) \\
& b & \mapsto & \pi_{2, 1} ( b) + [t]_2 D( b)
\end{array}$$
where $D$ is the $k (\mathfrak{m})$-linear functional defined on the basis $\mathcal{B}$ as $D ( \sigma(b) -b)=1$ and $D (u_i)=0$ for all $i \in I$. 
We now prove that $ \widetilde{\Psi}$ is a $k(\mathfrak{m})$-algebra morphism. We already know that $\widetilde{\Psi}$ is a $k(\mathfrak{m})$-linear as a sum of two linear morphisms. Let $b, c \in B$. We write $b= b_0+ b_1$ and $c= c_0+ c_1$ where $b_0, c_1 \in k( \mathfrak{m})\cdot 1$ and $b_1, c_1\in \mathfrak{m}/ \mathfrak{m}^2$. We have
$$\widetilde{\Psi} ( bc )= \widetilde{\Psi} ( b_0c_0 + b_1c_0 + b_0c_1 + b_1c_1 )$$  but $b_1c_1\in \mathfrak{m}^2$, so $b_1c_1=0; $
Therefore, 
$$ \widetilde{\Psi}( bc ) = \widetilde{\Psi} (b_0c_0) +  \widetilde{\Psi}(b_1c_0) +  \widetilde{\Psi}(x_0y_1)$$
Since $b_0, c_0 \in k( \mathfrak{m})\cdot 1$,there are $\alpha, \beta\in k( \mathfrak{m})$ such that $b_0= \alpha \cdot 1$, $b_0= \beta \cdot 1$ implies 
then $b_0c_0= \alpha \beta \cdot 1\in k( \mathfrak{m})\cdot 1$, we have $ \widetilde{\Psi} (b_0c_0) = \pi_{2,1} (b_0c_0)=\pi_{2,1} (b_0)\pi_{2,1} (c_0) $. Moreover, since $b_1, c_1 \in \mathfrak{m}/ \mathfrak{m}^2$, and that $\pi_{2, 1}$ is a $k(\mathfrak{m})$-algebra morphism that vanishes in $\mathfrak{m}/ \mathfrak{m}^2$ while $D$ vanishes in $k( \mathfrak{m})\cdot 1$, we obtain 
$$\widetilde{\Psi}(b_1c_0) +  \widetilde{\Psi}(x_0y_1)= [t]_1 [D(b_1 c_0) + D(b_0c_1)]$$
So that, 
$$\widetilde{\Psi}( bc ) = \pi_{2,1} (b_0)\pi_{2,1} (c_0) + [t]_1 [\pi_{2,1} (c_0)D(b_1 ) + \pi_{2,1} (b_0)D(c_1)]$$
On the other hand, we have
$$\begin{array}{lll} \widetilde{\Psi}( b ) \widetilde{\Psi}( c )&=& (\pi_{2,1} (b)+ [t]_1 D(b) )(\pi_{2,1} (c)+ [t]_1 D(c) ) \\
&=&  \pi_{2,1} (b)\pi_{2,1} (c ) + [t]_1 [D(b) \pi_{2,1} (c)+ \pi_{2,1} (b) D(c ) ] \\
&=&  \pi_{2,1} (b_0) \pi_{2,1} (c_0) + [t]_1 [\pi_{2,1} (c_0) D(b_1)+ \pi_{2,1} (b_0)D(c_1)]
\end{array}$$
Thus, $\widetilde{\Psi}( bc )= \widetilde{\Psi}( b ) \widetilde{\Psi}( c )$.
We have $\widetilde{\Psi}^{-1} ( (t)/ (t)^2 ) = \mathfrak{m}/\mathfrak{m}^2$. since given $b \in B /\mathfrak{m}^2$, we have $\widetilde{\Psi} (b) \in(t)/ (t)^2$ if and only if $b \in \mathfrak{m}/\mathfrak{m}^2$. We also have that ${\tau}^B_{1,0} (\widetilde{\Psi} ((B/\mathfrak{m}^2) \backslash (\mathfrak{m}/\mathfrak{m}^2)) ) \subseteq F^*$, since ${\tau}^B_{1,0} \circ \widetilde{\Psi}= \pi_{2,1}$. Finally, $(\widetilde{\Psi}  \circ \sigma ) (b)- \widetilde{\Psi}  (b) = \widetilde{\Psi} ( \sigma ( b) -b ) = [t]_1 D (\sigma (b) -b)\neq 0$. Therefore, $\Psi \circ \sigma \neq \Psi$, it follows that $\mathcal{L}_1 (\sigma ) \otimes \operatorname{id}_{k(\mathfrak{m})} |_{ \mathcal{L}_1(B)_{ \mathfrak{m}, red}} \neq id_{ \mathcal{L}_1(B)_{ \mathfrak{m}, red}} $. 

\end{proof}

\begin{remark}
Combining Lemma \ref{lem:Gmtofibre} and Lemma \ref{lem:redfibretoG1} we have an interesting consequence on the characterization on the first ramification group of an action.
Let $(B, \mathfrak{p})$ be an algebra that satisfies the hypothesis of those lemmas and let $G$ be a group acting on them. On one hand, Lemma \ref{lem:Gmtofibre} says that $\forall \sigma\in G_1(\mathfrak{p})$, $\mathcal{L}_1(\sigma)$ is trivial on $\mathcal{L}_1(B)_{k(\mathfrak{p})}$, in particular $\forall \mathfrak{q}\in \Spec \mathcal{L}_1(B)_{k(\mathfrak{p})}$, $\sigma\in G_0(\mathfrak{q})$; therefore we have the inclusion $\displaystyle G_1(p)\subseteq \bigcap_{\mathfrak{q}\in \Spec \mathcal{L}_1(B)_{k(\mathfrak{p})} } G_0(\mathfrak{q})$.
On the other hand, if $\sigma\in G_0(\mathfrak{q})$ for all $\mathfrak{q}\in \Spec \mathcal{L}_1(B)_{k(\mathfrak{p})}$, then $\mathcal{L}_1(\sigma)$ is trivial on $\mathcal{L}(B)_{\mathfrak{p}, red}$, indeed for $x\in \mathcal{L}_1(B)_{k(\mathfrak{p})}$, we have that $\mathcal{L}_1(\sigma)(x) -x \in \sqrt{0}= \bigcap_{\mathfrak{q}\in \Spec \mathcal{L}_1(B)_{k(\mathfrak{p})} } \mathfrak{q}$; in other words this means that $\mathcal{L}_1(\sigma)|_{\mathcal{L}_1(B)_{k(\mathfrak{p})}/\sqrt{0}}= \mathbf{id}_{\mathcal{L}_1(B)_{k(\mathfrak{p})}/\sqrt{0}}$. It follows by Lemma \ref{lem:redfibretoG1} that $\sigma\in G_1(\mathfrak{p})$.
Therefore we have an equality
$$ G_1(\mathfrak{p}) = \bigcap_{\mathfrak{q}\in \Spec \mathcal{L}_1(B)_{k(\mathfrak{p})} } G_0(\mathfrak{q}) \, . $$

\luigi{If $\mathcal{L}_1(B)_{k(\mathfrak{p})}$ is of finite type over $k(\mathfrak{p})$ (which happens whenever $B$ is finitely generated/$k$, or, more generally, should happen when $B_\mathfrak{p}$ is Noetherian, due to Cohen), then Jacobson = $\sqrt{0}$, so in the equality above we can only consider the maximal spectrum. This is useful for the existence of some functors. The hypotesis of $B$ being of finite type over $k$ is very mild in alg.geom.}
\end{remark}

\sophie{ J'ai essayer de faire marcher mais je comprends pas comment obtenir la decomposition necessaire: Il doit marcher si B, R sont Noetheriennes, ou si R est arbitraire et B est fin. gen. sur R.
Il faut replacer dans la preuve que j’ai envoyié seulement la partie jaune:
en lieu de prendre l’assumption $P/P^2\neq 0$, il faut assumer que le tangent *relative* est pas zero, i.e. $P/(P^2+P^c)$, ou $P^c$ est la contraction de $P$ sur R: remarque que si le tangent relatif est zero, il y a rien à prouver car B est unramifié (en P) sur R et $G_1(P)$ est toujours triviale.} 

\begin{exmp} 
\sophie{ Soit $B=k[x,y]/ (x^2, y^2)$, $P=(x,y)$ et soit $\sigma: B -> B$ donné par $\sigma(x)=x+xy$ et $\sigma(y)=y$. Alors $\sigma$ fixes $B$ mod $P^2$, mais pas mod $P^3$. (En effet $P^3=0$).
Est ce que ta equation montre cela en terms de $J_s$ pour quelques $s\in N$ et en terms de comparison avec $G_0$, $G_1$? Car dans cet example, *il semble que* $\sigma$ est pas dans $G_2$, mais est dans $G_1(q)$ pour chaque $q\in L_2(B)_{k(p)}$ (alors mes conjectures échoue dans ce cas). As tu des resultat differents?

[Autre cas $B=k[x,y,z]/(x^2,y^2,z^2)$, $\sigma(y)=y$, $\sigma(z)=z$, $\sigma(x)= x+ xy+yz+zx$, même problème].}
\end{exmp} 

\begin{lemma}  Let $k$ be a field, $s \in \mathbb{N}$, $B$ be a regular $k$-algebra with maximal ideal $\mathfrak{m}$ and $\sigma: B \rightarrow B$ be an automorphism of the $k$-algebra $B$ such that for all $b \in B$, $\sigma ( b) - b \in  \mathfrak{m}$. 
Let $c \in B$ be an element that minimize $v_{\mathfrak{m}} ( \sigma (c) -c)$ and such that $\sigma (c) - c \in \mathfrak{m}^s \backslash \mathfrak{m}^{s+1}$. Then 
 $\mathcal{L}_s (\sigma) \otimes \operatorname{id}_{k(\mathfrak{m})} |_{ \mathcal{L}_s(B)_{ \mathfrak{m}, red}} = id_{ \mathcal{L}_s(B)_{ \mathfrak{m}, red}} $.  
\end{lemma}

\begin{proof} 
 By Cohen's structure theorem (see for instance \cite[Lemma 10.160.10.]{stack}, we know that any complete regular equicharacteristic Noetherian local ring is a ring of formal power series over the residue class field. Therefore, if we denote $\widehat{B}$ be the $\mathfrak{m}$-adic completion of $B$, then $\widehat{B} \simeq k (\mathfrak{m}) [ [ x_1, \cdots, x_n]]$. Moreover, $\widehat{B}$ is local with maximal ideal $\widehat{\mathfrak{m}}$ and for $s\in \mathbb{N}^*$, $ \widehat{B}/ \widehat{\mathfrak{m}}^{s+1}\simeq  k (\mathfrak{m}) [ [ x_1, \cdots, x_n]]/ (x_1, \cdots, x_n)^{s+1}$. Let $\iota: k (\mathfrak{m}) \hookrightarrow  \overline{   k (\mathfrak{m})}$ the inclusion of fields. 
 
Given $s\in \mathbb{N}$ and $\underline{\lambda} = (\lambda_1, \cdots, \lambda_n)\in k (\mathfrak{m})^n$. Consider 
$$\begin{array}{rrll} \Psi_{\underline{\lambda}} : & k (\mathfrak{m}) [ [ x_1, \cdots, x_n]]/ (x_1, \cdots, x_n)^{s+1} & \rightarrow & { \overline{   k (\mathfrak{m})}}/{(t^{s+1})} \\ 
& u & \mapsto & \iota (u) \text{ for } u \in k (\mathfrak{m}) \\ 
& x_j & \mapsto & [t]_s \cdot \lambda_j 
\end{array}$$
where $\lambda_j \in F$, for all $1 \leq j \leq n$. 
Now, by assumption, there is $c \in B$ be an element that minimize $v_{\mathfrak{m}} ( \sigma (c) -c)$ and such that $\sigma (c) - c \in \mathfrak{m}^s \backslash \mathfrak{m}^{s+1}$. Therefore there is a homogeneous polynomial such that $\widetilde{\pi_{s+1}} : B \rightarrow B / \mathfrak{m}^{s+1} \simeq k (\mathfrak{m}) [ [ x_1, \cdots, x_n]]/ (x_1, \cdots, x_n)^{s+1}$ is the composite of the quotient map $\pi_{s+1}$ with the canonical isomorphism between $B / \mathfrak{m}^{s+1}$ and $k (\mathfrak{m}) [ [ x_1, \cdots, x_n]]/ (x_1, \cdots, x_n)^{s+1}$. Since $f \neq 0$, there is a $n$-tuple $\underline{ \lambda} = ( \lambda_1, \cdots, \lambda_2) \in F^n$ such that $f(\underline{\lambda}) \neq 0$. Therefore, 
$$ \begin{array}{ccl} (\sigma^* \Psi_{\underline{\lambda}}) ( \widetilde{\pi_{s+1}} (c)) -  \Psi_{\underline{\lambda}} (  \widetilde{\pi_{s+1}} (c)) &=& \Psi_{\underline{\lambda}} (  \widetilde{\pi_{s+1}} ( \sigma (c) -c) \\
&=& \Psi_{\underline{\lambda}} ( f( x_1, \cdots , x_n ) )= f( \underline{\lambda}) \neq 0 \end{array}$$ 
This means that $\mathcal{L}_s(\sigma) \otimes \operatorname{id}_{k(\mathfrak{m})}( \Psi) \neq (\Psi)$, hence 
$$ \mathcal{L}_s(\sigma) \otimes \operatorname{id}_{k(\mathfrak{m})} |_{ \mathcal{L}_s(B)_{\mathfrak{m} , \operatorname{red}} }\neq \operatorname{id} |_{ \mathcal{L}_s(B)_{\mathfrak{m} , \operatorname{red}}} .$$
\sophie{ not sure where minimality is used?} 
\end{proof}

\begin{remark} 
Let $B$ be a $k$-algebra, let $G$ be a subgroup of $\operatorname{Aut}_R(B)$. Then $ \sigma \notin G_s(\mathfrak{m})$ then there is $\mathfrak{q}\in \operatorname{Spec} ( \mathcal{L}_s( B)_{k(\mathfrak{m})})$ is such that $\mathcal{L}_s(\sigma) \otimes \operatorname{id}_{k(\mathfrak{m})}  \notin G_0(\mathfrak{q})$. $\mathfrak{q}$ is either the generic point of $ \mathcal{L}_s( B)_{k(\mathfrak{m})}$ or also when $ k(\mathfrak{m})/k$ is finite, we could choose $\mathfrak{q}$ closed point with coordinates $(\underline{\lambda})$ in $ \mathcal{L}_s( B)_{k(\mathfrak{m})}$.  \sophie{ need to be proven} \luigi{We will prove it (in a more complete statement) when we will actually talk about actions and ramifications... I only added this to the file because you asked me to remark connections to Inertia}

\luigi{The actual proof of this Remark goes as the Remark above, unfortunately the regularity of $B$ is an OK-ish hypothesis, but we ought to aim to a milder one. $B$ reduced would be nice because we would be able to work at least in the category of varieties instead of schemes, but we would miss the "historically" important case of Dedekind domains.}
\end{remark}

%
%
%\begin{exmp}
%We consider $B= k[x, y]$ and the maximal idea $\mathfrak{m}= (x-a, y-b)$ where $a, b \in k$. We have that $J_s(B) = k[(x_i, y_j)_{0\leq i\leq s, 0\leq j\leq s}]$. Moreover, $ \mathcal{L}_1(B)\otimes_B k( \mathfrak{m}) \simeq k[(x_i, y_j)_{1\leq i\leq s, 1\leq j\leq s}] $ where the isomorphism sending $p((x_i, y_j)_{0\leq i\leq s, 0\leq j\leq s})\otimes u $ to \\ $p((x_i, y_j)_{0\leq i\leq s, 0\leq j\leq s})|_{(x_0, y_0)=(a,b)}$.  \luigi{Is this independent on $u$? Are you working with $L_1$ or $L_s$?}
%\begin{enumerate} 
%\item 
%Given $p(x,y)\in B$. We define $\theta_1(p)(x_0, x_1, y_0,y_1)$ to be the polynomial in $k[x_0, x_1, y_0,y_1]$ such that $$p(x_0 + [t]_1 x_1, y_0 + [t]_1 x_1) = p(x_0, y_0) + [t]_1 \theta_1 (p)(x_0, x_1, y_0,y_1).$$ %We have $$p(x_0 + [t]_1 x_1, y_0 + [t]_1 x_1)|_{[t]_1=[1]_1}= p(x_0, y_0) + \theta_1(p(x,y))(x_0, x_1, y_0,y_1).$$ 
%We have 
%$$\begin{array}{lll} \theta_1(p)(x_0, x_1, y_0,y_1)&=& \frac{\partial{p}}{{\partial x_0}} (x_0, y_0) x_1+  \frac{\partial{p}}{{\partial y_0}} (x_0, y_0) y_1\\
%&=& D_{p,1}(x_0, x_1, y_0, y_1) \end{array}.$$ 
%We set $D_{p,1}(x_0, x_1, y_0, y_1):= \frac{\partial{p}}{{\partial x_0}} (x_0, y_0) x_1+  \frac{\partial{p}}{{\partial y_0}} (x_0, y_0) y_1$ and $T_{p,1}(x_0, x_1, y_0, y_1):=  p(x_0,y_0)+ \frac{\partial{p}}{{\partial x_0}} (x_0,y_0) x_1+  \frac{\partial{p}}{{\partial y_0}} (x_0,y_0) y_1$.
%Then, we define the following map, 
%$$\begin{array}{llllllll} \kappa_1: & B & \rightarrow  &  k[x_1,y_1]  \\
%& p(x,y)  &\mapsto &T_{p,1}(a, x_1, b, y_1)
%\end{array}$$
%\luigi{IMO, you should use a more specific word than "map", i.e. map of vector spaces or something like that, in a commutative algebra paper, $k-$linear maps are usually understood as homomorphisms of rings that are also linear over $k$, i.e. maps of $k-$algebras.}
%%We note that $  k[x_1,y_1] / (x_1,y_1)^2 \simeq k+kx_1+ ky_1$. 
%%Therefore we have 
%%{\small $$[\theta_1(p(x,y))(a,x_1, b, y_1)]_{(x_1,y_1)^2}=\left[ D_{p,1}(a, x_1, b, y_1) \right]_{(x_1,y_1)^2}.$$ }
%The map $ \kappa_1$ is $k$-linear and its kernel is $\mathfrak{m}^2$. Moreover, this map is a surjection onto $k+kx_1+ ky_1$. Therefore $\kappa_1$ induces a $k$-morphism $\overline{\kappa_1}$ between $B/ \mathfrak{m}^2$ and $J_1(B)_{\mathfrak{m}}$ \luigi{You described the image and this cannot be an isomorphism for dimensional reasons.} and a $k$-isomorphism $\widetilde{\kappa_1}$ between $B/ \mathfrak{m}^2$ and $J_1(B)_{\mathfrak{m}}/(x_1,y_1)^2J_1(B)_{\mathfrak{m}}$. \\
%\item Let $\sigma : B \rightarrow B$ an automorphism of $k$-algebra. The following diagram commutes: 
%$$ \xymatrix{ B \ar[d]^{\kappa_1} \ar[rr]^{\sigma} &&  \ar[d]^{\kappa_1}  B \\
%\mathcal{L}_1(B)_ \mathfrak{m} \ar[rr]_{\mathcal{L}_1(\sigma)\otimes id_{k( \mathfrak{m})}} &&  \mathcal{L}_1(B)_ \mathfrak{m}
%}.$$
%Indeed, if we set $ q_{p_\sigma} ( x,y):= \sigma (p(x,y)) $, we have $q_{x_\sigma} ( x_0+[t]_1 x_1,y_0+[t]_1 y_1)= q_{x_\sigma}(x_0, y_0) + D_{q_{x_\sigma}, 1}(x_0, x_1, y_0, y_1) [t]_1$ and $q_{y_\sigma} ( x_0+[t]_1 x_1,y_0+[t]_1 y_1)= q_{y_\sigma}(x_0, y_0) + D_{q_{y_\sigma}, 1}(x_0, x_1, y_0, y_1) [t]_1$
%
%We have $\kappa_1(p(x,y)) = T_{p,1}(a, x_1, b, y_1) $. We have \\
%$$\begin{array}{lll} \mathcal{L}_1(\sigma)(T_{p,1}(x_0, x_1, y_0, y_1))&=& T_{p,1} (q_{x_\sigma} ,D_{q_{x_\sigma}, 1}, q_{y_\sigma} ,D_{q_{y_\sigma}, 1})\\
%&=& p( q_{x_\sigma},  q_{y_\sigma}) + D_{p,1}(q_{x_\sigma} ,D_{q_{x_\sigma}, 1}, q_{y_\sigma} ,D_{q_{y_\sigma}, 1})
%\end{array}$$
%We have $\sigma ( p(x,y)) = q_{p_\sigma} ( x,y)= p(  q_{x_\sigma}(x,y), q_{y_\sigma}(x,y)) $. \\
%We set $r(x, y) = p(  q_{x_\sigma}(x,y), q_{y_\sigma}(x,y)) $. We have 
%$$\begin{array}{lll} \kappa_1(r(x,y))&=&T_r (x_0, x_1, y_0, y_1)= r(x_0, y_0) + \frac{\partial{r}}{{\partial x_0}} (x_0, y_0) x_1+  \frac{\partial{r}}{{\partial y_0}} (x_0, y_0) y_1\\
%&=& p(q_{x_\sigma},  q_{y_\sigma} )+ D_{q_{x_\sigma}, 1} \frac{\partial{p}}{{\partial x_0}}(q_{x_\sigma},  q_{y_\sigma} )+ D_{q_{y_\sigma}, 1} \frac{\partial{p}}{{\partial y_0}}(q_{x_\sigma},  q_{y_\sigma} ) \\
%&=& T_{p,1} (q_{x_\sigma} ,D_{q_{x_\sigma}, 1}, q_{y_\sigma} ,D_{q_{y_\sigma}, 1})
% .\end{array}$$ 
% Therefore, the diagram commutes.
% \item Let $\sigma : B \rightarrow B$ an automorphism of $k$-algebra such that $\sigma (b)-b \in \mathfrak{m}$ for all $b \in B$. \\
%This map induces a map $\tilde{\sigma} : B/ \mathfrak{m}^2 \rightarrow B/ \mathfrak{m}^2 $.
%We have 
%$$\mathcal{L}_1 ( \mathfrak{m}) =\mathcal{L}_1 (( x,y))= (x_0-a,x_1, y_0-b,y_1)  $$
%$$\begin{array}{lll} &&\mathcal{L}_1 ( \mathfrak{m}^2) \\&=&\mathcal{L}_1 (( x^2 , xy , y^2))\\
%&=& ((x_0-a)^2, 2 (x_0-a)x_1, (y_0-b)^2 , 2(y_0-b) y_1,\\
%&& (x_0-a)(y_0-b), (x_0-a)x_1+ (y_0-b) y_1 )  \\
%&=& ((x_0-a,y_0-b)^2, 2 (x_0-a)x_1 , (x_0-a)x_1+ (y_0-b) y_1 )  
%\end{array}$$
%When $char(k)\neq 2$,  
%
%$$\mathcal{L}_1 ( \mathfrak{m})^2 =( \mathcal{L}_1 ( \mathfrak{m}^2), (x_1, y_1)^2)  $$
%When $char(k) = 2$
%$$\mathcal{L}_1 ( \mathfrak{m})^2 =( \mathcal{L}_1 ( \mathfrak{m}^2),(x_0-a)x_1, (x_1, y_1)^2)  $$
%\luigi{I think you are missing the generator $(y_0-b)y_1$.}
%If $\sigma (  \mathfrak{m}) =  \mathfrak{m}$ we have $\mathcal{L}_1 ( \sigma) ( \mathcal{L}_1 ( \mathfrak{m}) ) = \mathcal{L}_1 ( \mathfrak{m}) $, $\mathcal{L}_1 ( \sigma)( \mathcal{L}_1 ( \mathfrak{m})^2) = \mathcal{L}_1 ( \mathfrak{m})^2$.  
%In $\mathcal{L}_s(B)_ \mathfrak{m}$, we have $ \mathcal{L}_1 ( \mathfrak{m}^2)_{\mathfrak{m}}=0$ and $\mathcal{L}_1 ( \mathfrak{m})^2_{\mathfrak{m}}= (x_1, y_1)^2$. 
%The following diagram commutes applying (1) (b) and the above. 
%$$ \xymatrix{ B/ \mathfrak{m}^2 \ar@/_4pc/[dd]^{\widetilde{\kappa_1}}  \ar[d]^{\overline{\kappa_1}} \ar[rr]^{\widetilde{\sigma}} &&  \ar[d]^{\overline{\kappa_1}}  B/ \mathfrak{m}^2\ar@/^4pc/[dd]^{\widetilde{\kappa_1}}  \\
%\mathcal{L}_1(B)_ \mathfrak{m} \ar[rr]_{{\mathcal{L}_s(\sigma)\otimes id_{k( \mathfrak{m})}}}\ar[d]^{p} && \mathcal{L}_1(B)_ \mathfrak{m} \ar[d]^p\\
%\mathcal{L}_1(B)_ \mathfrak{m} /\mathcal{L}_1 ( \mathfrak{m})^2_{\mathfrak{m}} \mathcal{L}_1(B)_ \mathfrak{m}  \ar[rr]_{\widetilde{\mathcal{L}_1(\sigma)\otimes id_{k( \mathfrak{m})}}} && \mathcal{L}_1(B)_ \mathfrak{m} /\mathcal{L}_1 ( \mathfrak{m})^2_{\mathfrak{m}}\mathcal{L}_1(B)_ \mathfrak{m} 
%}.$$
%Suppose that $\widetilde{\sigma}=id$. Let $b\in \mathcal{L}_s(B)_ \mathfrak{m}$. We have $\widetilde{\sigma} (\widetilde{\kappa_1}^{-1} ( p( b))) = \widetilde{\kappa_1}^{-1} ( p( b))$. Equivalently, $\widetilde{\kappa_1}^{-1}  ( \widetilde{\mathcal{L}_s(\sigma)_\mathfrak{m}} (p(b)) =\widetilde{\kappa_1}^{-1} ( p( b))$. That is $\widetilde{\mathcal{L}_s(\sigma)_\mathfrak{m}} (p(b) =p( b)$. So that, $p ( \mathcal{L}_s(\sigma)_\mathfrak{m}( b) ) = p(b)$. Therefore, $ \mathcal{L}_s(\sigma)_\mathfrak{m}( b) - b \in (x_1, y_1)^2 \mathcal{L}_s(\sigma)_\mathfrak{m}$. If we prove that $ \mathcal{L}_s(\sigma)_\mathfrak{m}( x_i)=x_i $ and $ \mathcal{L}_s(\sigma)_\mathfrak{m}( y_i)=y_i $ for $i=1,2$, we are done. But $\mathcal{L}_s(\sigma)_\mathfrak{m}( x_0)= q_{\sigma}( x_0, y_0)$ and $q_{x_\sigma}( x_0, y_0)-x_0\in (x_1, y_1)^2 \mathcal{L}_s(\sigma)_\mathfrak{m}$ implies $\mathcal{L}_s(\sigma)_\mathfrak{m}( x_0)= x_0$. Similarly, $\mathcal{L}_s(\sigma)_\mathfrak{m}( y_0)= q_{y_\sigma}( x_0, y_0)$. 
%
%Moreover, $\mathcal{L}_s(\sigma)_\mathfrak{m}( x_1)= D_{q_{x_\sigma},1}( x_0,x_1, y_0, y_1)$. So that $D_{q_{x_\sigma},1}( x_0,x_1, y_0, y_1)- x_1$ is linear in $x_1$ and $x_2$. So that $D_{q_{x_\sigma},1}( x_0,x_1, y_0, y_1)- x_1\in (x_1, y_1)^2 \mathcal{L}_s(\sigma)_\mathfrak{m}$ implies $\mathcal{L}_s(\sigma)_\mathfrak{m}( x_1)=x_1$. Similarly, we obtain $\mathcal{L}_s(\sigma)_\mathfrak{m}( y_1)=y_1$. So that we conclude that $\widetilde{\sigma}= id$ if and only if $\mathcal{L}_s(\sigma)_\mathfrak{m}=id$. 
%\\ \\
%\end{enumerate}
%\luigi{I did not understand if here you used the theory for vector spaces or of rings. In any case the conclusion you got to is not correct. COUNTEREXAMPLE: $\sigma(x)=x+y^2, \sigma(y)=y$ induces an isomorphism in $B/M^2$, but not in the bottom row for $s$ large enough.}
%
%\luigi{Even if we stick to the case $s=1$, this seems a very twisted way to describe the {\bfseries tangent map} (and there is plenty of literature about that, so I don't think that this is material for a research paper, maybe for a survey). Could you please write a few lines to describe the insight that you want to give with this example, because I didn't really understand.}
%\end{exmp}
%
%
%\luigi{Will check later the following two examples.}
%\begin{exmp} 
% Let $p(x,y)\in B$. 
%We define $\theta_2(p)(x_0, x_1, x_2, y_0,y_1,y_2)$ as the polynomial in \\$k[x_0, x_1, x_2, y_0,y_1,y_2]$ such that $$\begin{array}{lll} &&p(x_0 + [t]_2 x_1, y_0 + [t]_2 x_1) \\
%&=& p(x_0, y_0) + [t]_2 \theta_1 (p)(x_0, x_1, y_0,y_1)+  [t]_2^2 \theta_2 (p)(x_0, x_1, x_2, y_0,y_1,y_2).\end{array}$$ 
%% We have $p(x_0 + [t]_1 x_1, y_0 + [t]_1 x_1)|_{[t]_1=[1]_1}= p(x_0, y_0) + \theta_1(p(x,y))+\theta_2 (p(x,y))$. 
%We have 
%{\small $$\theta_2 (p)(x_0, x_1, x_2, y_0,y_1,y_2)= D_{p,1}(x_0, y_0, x_2, y_2) + D_{p,2} (x_0, y_0, x_1,y_1).$$ }
%We recall that $$ D_{p,1}(x_0, y_0, x_2, y_2) =  \frac{\partial{p}}{{\partial x_0}} (x_0, y_0) x_2+  \frac{\partial{p}}{{\partial y_0}} (x_0, y_0) y_2$$ and\\ 
%{\footnotesize $$D_{p,2} (x_0, y_0, x_1,y_1)=  \frac{\partial^2{p}}{{\partial y_0^2}} (p(x_0,y_0)) \frac{y_1^2}{2}+  \frac{\partial^2{p}}{{\partial x_0^2}} (p(x_0,y_0)) \frac{x_1^2}{2} + \frac{\partial^2{p}}{{\partial y_0 \partial x_0}} (p(x_0,y_0)) x_1y_1.$$ }
%We have 
%$$p(x_0 + [t]_2 x_1, y_0 + [t]_2 x_1)|_{[t]_2=[1]_2}= T_{p,2} (x_0, y_0, x_1,y_1)+ D_{p,1}(x_0, y_0, x_2, y_2) $$
%We define $\kappa_2$ to be the map
%$$\begin{array}{llllllll} \kappa_2: & B  & \rightarrow &  k[x_1,y_1]   \\
%& p(x,y) &\mapsto &T_{p,2} (a, b, x_1,y_1)+ D_{p,1}(a, b, x_2, y_2) 
%\end{array}$$
%The map $ \kappa_2$ is $k$-linear and its kernel is $\mathfrak{m}^3$ and onto $k+ kx_2+ky_2+ kx_1+ ky_1+ k x_1^2 +ky_1^2 + k x_1y_1$. Therefore, this map induces a map $\overline{ \kappa_2}$ from $B/\mathfrak{m}^3$ to $J_2 ( B)_{\mathfrak{m}}$.
%Let $\sigma : B \rightarrow B$ an automorphism of $k$-algebra such that $\sigma (b)-b \in \mathfrak{m}$ for all $b \in B$. \\
%This map induces a map $\tilde{\sigma} : B/ \mathfrak{m}^2 \rightarrow B/ \mathfrak{m}^2 $.
%$$ \xymatrix{ B/ \mathfrak{m}^2   \ar[d]^{\overline{\kappa_2}} \ar[rr]^{\widetilde{\sigma}} &&  \ar[d]^{\overline{\kappa_2}}  B/ \mathfrak{m}^2 \\
%\mathcal{L}_2(B)_ \mathfrak{m} \ar[rr]_{{\mathcal{L}_2(\sigma)_{\mathfrak{m}}}}&& \mathcal{L}_s(B)_ \mathfrak{m} 
%}.$$
%The above diagram commutes (we can prove this as before). 
%We want to prove that $\widetilde{\sigma}= id$ if and only if $\mathcal{L}_2(\sigma)_{\mathfrak{m}}=id$.  The if direction is easily proven using the injectivity of $\overline{\kappa_2}$. For the only, if direction, let us assume that $\widetilde{\sigma}= id$. We need to prove that $\mathcal{L}_2(\sigma)_{\mathfrak{m}}(x_i) = x_i$ and $\mathcal{L}_2(\sigma)_{\mathfrak{m}}(y_i) = y_i$, for $i=1,2,3$. 
%We have $\overline{\kappa_2} ( x-a ) =x_1$ and $\overline{\kappa_2} ( y-a ) =y_1$.
%\end{exmp}
%\begin{exmp} 
%\begin{enumerate} 
%\item \begin{enumerate} 
%%
%%We have 
%%$$ T_{p,2} (x_0, y_0, x_1,y_1)= p(x_0, y_0) +  D_{p,1} (x_0, y_0, x_1,y_1)+  D_{p,2} (x_0, y_0, x_1,y_1).$$
%%
%%%We have $ k[x_1,y_1] / (x_1,y_1)^3  \simeq J_2(B)_{\mathfrak{m}} / ((x_2, y_2) (x_1,y_1)^3)J_2(B)_{\mathfrak{m}}$.
%%
%%The map $ \kappa_2$ is $k$-linear and its kernel is $\mathfrak{m}^3$. Moreover, this map is onto $k+ kx_1+ ky_1+kx_1^2+ kx_1y_1+ ky_1^2$. Therefore $\kappa_2$ induces a $k$-isomorphism $\widetilde{\kappa_2}$ between $B/ \mathfrak{m}^3$ and $J_2(B)_{\mathfrak{m}} / ((x_2, y_2), (x_1,y_1)^3)J_2(B)_{\mathfrak{m}}$.  \\
%%% \item Let $\sigma : B \rightarrow B$ an automorphism of $k$-algebra. The following diagram commutes: 
%%%$$ \xymatrix{ B \ar[d]^{\kappa_2} \ar[rr]^{\sigma} &&  \ar[d]^{\kappa_2}  B \\
%%%\mathcal{L}_2(B)_ \mathfrak{m} \ar[rr]_{\mathcal{L}_2(\sigma)\otimes id_{k( \mathfrak{m})}} &&  \mathcal{L}_q(B)_ \mathfrak{m}
%%%}.$$ 
%%%The proof goes as above.
%%\item Let $\sigma : B \rightarrow B$ an automorphism of $k$-algebra such that $\sigma (b)-b \in \mathfrak{m}$ for all $b \in B$. \\
%%This map induces a map $\tilde{\sigma} : B/ \mathfrak{m}^3 \rightarrow B/ \mathfrak{m}^3 $.
%%We have 
%%%$$\mathcal{L}_2 ( \mathfrak{m}) =\mathcal{L}_2 (( x,y))= (x_0-a,x_1, x_2, y_0-b,y_1,y_2)= (\mathcal{L}_1 ( \mathfrak{m}) , (x_2, y_2))  $$
%%%$$\begin{array}{lll} \mathcal{L}_2 ( \mathfrak{m}^2) &=&\mathcal{L}_2 (( x^2 , xy , y^2))\\
%%%&=& (\mathcal{L}_1 ( \mathfrak{m}^2),2 (x_0-a) x_2+x_1^2 , 2(y_0-b) y_2+ y_1^2, x_1y_1 )  \\
%%%\end{array}$$
%%%$$\begin{array}{lll} &&\mathcal{L}_2 ( \mathfrak{m}^2)  \mathcal{L}_2 ( \mathfrak{m})\\
%%%&=&(\mathcal{L}_1 ( \mathfrak{m}^2),2 (x_0-a) x_2+x_1^2 , 2(y_0-b) y_2+ y_1^2, x_1y_1 ) (\mathcal{L}_1 ( \mathfrak{m}) , (x_2, y_2)), \\
%%%&=&(\mathcal{L}_1 ( \mathfrak{m}^2)\mathcal{L}_1 ( \mathfrak{m}) ,(2 (x_0-a) x_2+x_1^2 , 2(y_0-b) y_2+ y_1^2, x_1y_1 )\mathcal{L}_1 ( \mathfrak{m}), \\&& \mathcal{L}_1 ( \mathfrak{m}^2)(x_2, y_2),(2 (x_0-a) x_2+x_1^2 , 2(y_0-b) y_2+ y_1^2, x_1y_1 ) (x_2, y_2))\\
%%%\end{array}$$
%%%$$ \begin{array}{lll} \mathcal{L}_2 ( \mathfrak{m})^2&=& (\mathcal{L}_1 ( \mathfrak{m}) , (x_2, y_2)) ^2\\
%%%&=&  (\mathcal{L}_1 ( \mathfrak{m}) ^2 ,  \mathcal{L}_1 ( \mathfrak{m})(x_2, y_2), (x_2, y_2)^2)\\
%%%&=&  (\mathcal{L}_1 ( \mathfrak{m}^2) , (x_1, y_1)^2 ,  \mathcal{L}_1 ( \mathfrak{m})(x_2, y_2), (x_2, y_2)^2)\\
%%%\end{array}$$
%%%
%%%$$\begin{array}{lll} \mathcal{L}_1 ( \mathfrak{m}^3) &=&\mathcal{L}_1 (( x^3 , 3x^2y, 3yx^2 , y^3))\\
%%%&=& ((x_0-a, y_0-a)^3,  3(x_0-a)^2x_1, 3(y_0-b)^2y_1, \\
%%%&&  3(x_0-a)^2 y_1+ 6(x_0-a)x_1(y_0-b) ,  3(y_0-b)^2 x_1+ 6(y_0-b)y_1(x_0-a)) \\
%%%  \end{array}$$
%%%  
%%%  $$\begin{array}{lll} \mathcal{L}_1 ( \mathfrak{m})^3 &=&(x_0-a,x_1, x_2, y_0-b,y_1,y_2)^3\\
%%%&=& ((x_0-a, y_0-a)^3,  3(x_0-a)^2x_1, 3(y_0-b)^2y_1, \\
%%%&&  3(x_0-a)^2 y_1+ 6(x_0-a)x_1(y_0-b) ,  3(y_0-b)^2 x_1+ 6(y_0-b)y_1(x_0-a)) \\
%%%  \end{array}$$
%%
%%$$\begin{array}{lll} \mathcal{L}_2 ( \mathfrak{m}^3) &=&\mathcal{L}_1 (( x^3 , 3x^2y, 3yx^2 , y^3))\\
%%&=& ((x_0-a, y_0-a)^3,  3(x_0-a)^2x_1,  3(y_0-b)^2y_1,\\
%%&&3(x_0-a)^2x_2+3(x_0-a)x_1^2,3(y_0-b)^2y_2+ 3(y_0-b)y_1^2, \\
%%&&  3(x_0-a)^2y_1+ 6 (x_0-a)x_1(y_0-b), 3(y_0-b)^2 x_1+ 6(y_0-b)y_1(x_0-a), \\
%%&& 3(x_0-a)^2 y_2 +6 (x_0-a)x_1y_1+6(x_0-a)x_2(y_0-b)+ 3 (y_0-b)x_1^2,\\
%%&& 3(y_0-a)^2 x_2 +6 (y_0-a)y_1x_1+6(y_0-a)y_2(x_0-b)+ 3 (x_0-b)y_1^2)\\
%%  \end{array}$$
%%
%%
%%$$\begin{array}{lll} \mathcal{L}_1 ( \mathfrak{m})^3 &=&(x_0-a, x_1, x_2, y_0-b,y_1, y_2)^3 \\
%%&=&((x_0-a, y_0-b)^3 , 3 (x_0-a, y_0-b)^2 (x_1, x_2, y_1, y_2) , \\
%%&&3 (x_0-a, y_0-b) (x_1, y_1)^2, 6 (x_0-a, y_0-b) (x_1, y_1)( x_2, y_2),\\
%%&& 3 (x_0-a, y_0-b) ( x_2, y_2)^2,(x_1, x_2, y_1, y_2)^3) \\
%%&=& ( \mathcal{L}_1 ( \mathfrak{m}^3),3 (x_0-a, y_0-b)^2 (x_1, x_2, y_1, y_2) , 6 (x_0-a, y_0-b) (x_1, y_1)( x_2, y_2),\\
%%&& 3 (x_0-a, y_0-b) ( x_2, y_2)^2,(x_1, x_2, y_1, y_2)^3) \\
%%  \end{array}$$
%%
%%If $\sigma (  \mathfrak{m}) =  \mathfrak{m}$ we have $\mathcal{L}_1 ( \sigma) ( \mathcal{L}_1 ( \mathfrak{m}) ) = \mathcal{L}_1 ( \mathfrak{m}) $, $\mathcal{L}_1 ( \sigma)( \mathcal{L}_1 ( \mathfrak{m})^2) = \mathcal{L}_1 ( \mathfrak{m})^2$.  
%%In $\mathcal{L}_s(B)_ \mathfrak{m}$, we have $ \mathcal{L}_1 ( \mathfrak{m}^2)_{\mathfrak{m}}=0$ and $\mathcal{L}_1 ( \mathfrak{m})^2_{\mathfrak{m}}= (x_1, y_1)^2$. 
%%The following diagram commutes applying (1) (b) and the above. 
%%$$ \xymatrix{ B/ \mathfrak{m}^2 \ar[d]^{\widetilde{\kappa_1}} \ar[rr]^{\widetilde{\sigma}} &&  \ar[d]^{\widetilde{\kappa_1}}  B/ \mathfrak{m}^2 \\
%%\mathcal{L}_s(B)_ \mathfrak{m} /\mathcal{L}_1 ( \mathfrak{m})^2_{\mathfrak{m}} \mathcal{L}_s(B)_ \mathfrak{m}  \ar[rr]_{\widetilde{\mathcal{L}_s(\sigma)\otimes id_{k( \mathfrak{m})}}} && \mathcal{L}_s(B)_ \mathfrak{m} /\mathcal{L}_1 ( \mathfrak{m})^2_{\mathfrak{m}}\mathcal{L}_s(B)_ \mathfrak{m} 
%%}.$$
%% Thanks to this diagram we can prove that $\widetilde{\sigma}$ is the identity if and only if $\widetilde{\mathcal{L}_s(\sigma)\otimes id_{k( \mathfrak{m})}}$ is the identity. $\widetilde{\mathcal{L}_s(\sigma)\otimes id_{k( \mathfrak{m})}}$ fully determine $\mathcal{L}_s(\sigma)\otimes id_{k( \mathfrak{m})}$ so that the latter is also equivalent to $\mathcal{L}_s(\sigma)\otimes id_{k( \mathfrak{m})}$ being identity.
%%
%%
%%%We note that  $k[x_1,y_1] / ((x_1,y_1)^3, (x_2,y_2)) \simeq k+k(\mathfrak{m})x_1+ ky_1+k(\mathfrak{m})x_1^2+ ky_1^2+ kx_1y_1 $
%%
%%
%%
%\end{enumerate}
%
%\item Let $\mathfrak{n} =(x^2, y^2)$. We set $C: = B/\mathfrak{n}$ and $\overline{\mathfrak{m}} ={ \mathfrak{m}}/{ \mathfrak{n} }$. We consider the $R$-algebra automorphism $\sigma : C \rightarrow C$ sending $[x]_{\mathfrak{n}}$ to $[x+xy]_{\mathfrak{n}}$  and $[y]_{\mathfrak{n}}$ to $[y]_{\mathfrak{n}}$. Its inverse is the map $\sigma^{-1} : C \rightarrow C$ sending $[x]_{\mathfrak{n}}$ to $[x-xy]_{\mathfrak{n}}$  and $[y]_{\mathfrak{n}}$ to $[y]_{\mathfrak{n}}$.
%\begin{enumerate} 
%\item We have $J_1(\mathfrak{n} )=(x_0^2 , 2x_0x_1  , y_0^2 , 2 y_1y_0)$ and $J_1(B) = k[x_0, x_1, y_0,y_1]/J_1(\mathfrak{n} )$. 
%
%%Let $B= k[x, y]/(x^2, y^2)$, $J_1(B) = k[x_0, x_1, y_0,y_1]/(x_0^2 , 2x_0x_1  , y_0^2 , 2 y_1y_0)$, $\mathfrak{m}= \frac{(x, y)}{(x^2, y^2)}$. 
%
%%Let $p(x,y)\in B$. 
%%We define $\theta(p(x,y)) \in k[x_0, x_1, y_0,y_1]$, $p(x_0 + [t]_1 x_1, y_0 + [t]_1 x_1) = p(x_0, y_0) + [t]_s \theta (p(x,y))$. We have $p(x_0 + [t]_1 x_1, y_0 + [t]_1 x_1)|_{[t]_s=[1]_s} = p(x_0,y_0)+ \frac{\partial{p}}{{\partial x_0}} (x_0,y_0) x_1+  \frac{\partial{p}}{{\partial y_0}} (x_0,y_0) y_1$.
%%Well defined by the definition of $J_s(B)$. 
%We have 
% $J_1(B)_{\overline{\mathfrak{m}}}= k[x_0, x_1, y_0,y_1]/(x_0^2 , 2x_0x_1  , y_0^2 , 2 y_1y_0) \otimes_B k (\overline{\mathfrak{m}}) = k [x_1, y_1]$
%We have $$ C/\overline{\mathfrak{m}^2}\simeq J_s(B)_{\overline{\mathfrak{m}}}/(x_1, y_1)^2 J_s(B)_{\overline{\mathfrak{m}}}$$ 
%%When $char \neq 2$  and $a, b \neq 0$ we have  $\mathcal{L}_s(B)_\mathfrak{m} =  k (\mathfrak{m} )$. \\
%%When $a , b =0$ or $char=2$,  then   $\mathcal{L}_s(B)_\mathfrak{m} =  k (\mathfrak{m} ) [x_1, y_1]$.
%%
%%$$J_1\left( \frac{(x, y)^2}{(x^2, y^2)}\right) = \frac{ (x_0^2 , 2x_0x_1  , y_0^2 , 2 y_0 y_1, x_0y_0, x_0y_1, y_0 x_1)}{(x_1+x_0^2 , 2x_0x_1 , y_0^2 , 2 y_1y_0)}.$$ 
%
%We set $p_\sigma (x, y) := x+xy$, so that $p_\sigma (x_0 + [t]_1 x_1, y_0 + [t]_1 y_1) = x_0 + [t]_1 x_1+ (x_0 + [t]_1 x_1) ( y_0 + [t]_1 y_1) = x_0 + x_0y_0 + (x_1+ x_0 y_1+ y_0 x_1) [t]_1$. So that
%$\widetilde{\mathcal{L}_1( \sigma) \otimes id_{k(\mathfrak{m})}}: k [x_1 , y_1]  \rightarrow  k [x_1 , y_1] $ sends $x_1$ to $ x_1$ and $y_1$ to $y_1$. 
%\item $J_2(\mathfrak{n} )= (x_0^2 , 2x_0x_1 ,2 x_0x_2+x_1^2 , y_0^2 , 2 y_1y_0 ,2 y_0y_2+y_1^2)$. We have 
% $$\begin{array}{lll} J_2(B)_{\overline{\mathfrak{m}}}&=& k[x_0, x_1,x_2, y_0,y_1, y_2]/(x_0^2 , 2x_0x_1 ,2 x_0x_2+x_1^2 , y_0^2 , 2 y_1y_0 ,2 y_0y_2+y_1^2) \otimes_B k (\overline{\mathfrak{m}}) \\
% &=& k [x_1, y_1,x_2, y_2]/( x_2^2, y_2^2)\end{array}$$
% As a consequence, since $\overline{\mathfrak{m}}^{3}= \overline{\mathfrak{m}^3}= (0)$.
% $$ C/\overline{\mathfrak{m}^3}\simeq C  \simeq \mathcal{L}_2(B)_{\overline{\mathfrak{m}}}/((x_1, y_1)/( x_1^2, y_1^2)) \mathcal{L}_2(B)_{\overline{\mathfrak{m}}}$$ 
%We have $p_\sigma (x_0 + [t]_2 x_1+ [t]_2^2 x_2 , y_0 + [t]_2 y_1+ [t]_2^2 y_2) = x_0 + [t]_1 x_1+ [t]_2^2 x_2+ (x_0 + [t]_1 x_1+ [t]_2^2 x_2) ( y_0 + [t]_1 y_1+ [t]_2^2 y_2) = x_0 + x_0y_0 + (x_1+ x_0 y_1+ y_0 x_1) [t]_2 + ( x_2 + x_1y_1+ x_0y_2 + y_0x_2)[t]_2^2$. We have $\widetilde{\mathcal{L}_2( \sigma) \otimes id_{k(\mathfrak{m})}}: k [x_1,x_2 , y_1, y_2]/( x_2^2, y_2^2)  \rightarrow  k [x_1,x_2 , y_1, y_2] /( x_2^2, y_2^2)$ sends $x_1$ to $ x_1$, $x_2$ to $x_2+x_1y_1$, $y_1$ to $y_1$ and $y_2$ to $y_2$.
%\end{enumerate}
%\end{enumerate}
%\end{exmp}
%\luigi{As I said before, I didn't check these example. But it would be great if before any example we could write a few lines of comment (using the commands "luigi"/"sophie") so we communicate to each other what is the take-out/insight for the reader.}

%\begin{definition}
%Given a prime ideal in $k[x_1,\cdots , x_n]$, $\sum_\mathfrak{p}$ to be the field extension of $k$ generated by $(b_{i,j})_{(i,j) \in I \times \{ 1, \cdots , n\}}$ where $(b_{i,j})_{(i,j) \in I \times \{ 1, \cdots , n\}}$ is such that $\{ \mathfrak{m}_i \}_{i \in I}$ is the set of maximal ideal containing $\mathfrak{p}$ in $\overline{k}[x_1, \cdots, x_n]$ and $\mathfrak{m}_i = \langle x_1-b_{i,1} , \cdots, x_n -b_{i, n} \rangle$ for all $i\in I$. 
%\end{definition} 
%
%\sophie{do we have $\sum_\mathfrak{p}$ separable if and only if $k(\mathfrak{p})$ separable? }
\begin{definition}
Let $\mathfrak{p}$ be a prime ideal of a polynomial ring in $n$ variables $k[x_1, \cdots , x_n]$. We say that $\mathfrak{p}$ is separably generated over $k$ if $k(\mathfrak{p})$ is separably generated over $k$.
\end{definition}

\begin{lemma}
Let $\mathfrak{p}$ be a prime ideal of $\operatorname{Spec}(A)$. 
The following assertions are equivalent
\begin{enumerate}
\item $\mathfrak{p}$ is separably generated over k 
\item $\mathfrak{p}k^{sep}[x_1, \cdots , x_n] = \cap_{\mathfrak{m}\in {\mathscr{M}_{sep}}} \mathfrak{m}$ where $\mathscr{M}_{sep} = \{ \langle x_1-a_1 , \cdots , x_n - a_n \rangle | a_i \in k^{sep} , \forall i \in \{ 1, \cdots, n \}  \}$.
\end{enumerate} 
\end{lemma}

\begin{proof}
By Noether normalization lemma, $k[x_1, \cdots, x_n ]/ \mathfrak{p}$ is an algebra of finite type over the field $k$ and is an integral domain, so the transcendence degree of its fraction field is equal to the Krull dimension of $k[x_1, \cdots, x_n ]/ \mathfrak{p}$. More precisely, there exist $T$ subset of $S= \{ x_1, \cdots, x_n\}$ such that $k( \mathfrak{p})$ is finite over $k(T)$. %We call $\zeta_p : k[x_1, \cdots, x_n ] \rightarrow k( \mathfrak{p})$ is the residue field canonical morphism.

$(1) \Rightarrow (2)$ Suppose that $k(\mathfrak{p})$ is separably generated over $k$. Therefore, $k(\mathfrak{p})$ is finite separable over $k(T)$. Thus, by the primitive element theorem, we know that any finite separable extension admits a primitive element therefore there exists $z \in k( \mathfrak{p})$ such that $k(\mathfrak{p})= k(T)(z)$ and the minimal polynomial $p(X)$ of $z$ over $k(T)$ is separable. Moreover, %we have $k(\mathfrak{p})\otimes_{k(T)} k(T)^{sep} = k(T)^{deg( k(\mathfrak{p})/ k(T))}$ and 
%
the image $\mathfrak{P}$ of $\mathfrak{p}$ in $k(T) [ S \backslash T] \simeq k(T) \otimes_{k[T]} k[x_1, \cdots , x_n]$ is a maximal ideal in $k(T) [ S \backslash T]$. Indeed if it was not then the transcendental degree of $k(\mathfrak{P})\simeq k(\mathfrak{p})$ over $k(T)$ would be strictly greater than $1$ and that would constitute a contradiction. %Indeed, we have $\mathfrak{P}$ is the kernel of the map $k(T) [ S \backslash T] \rightarrow k(T) \otimes_{k[T]} k(\mathfrak{p})$. Moreover the following diagram 
%$$\xymatrix{ 0 \ar[r] & \mathfrak{P} \ar[d] \ar[r]  & k(T) [ S \backslash T] \ar@{->>}[d]\ar[r] & k(T) \otimes_{k[T]} k(\mathfrak{p})  \ar[d]^{\simeq}    \\ 0 \ar[r] & \langle p(X) \rangle  \ar[r] & 
% k(T)[X] \ar[r] & k(T)(z) \ar[r] & 0 }$$ 
%
%the image of $\mathfrak{p}$ in $k[x_1, \cdots , x_n]$ is $\langle p(X) \rangle$ maximal ideal of $k(T) [ z]$. 
We have $\langle p(X) \rangle k(T)^{sep} [ X] =\cap_{b \in Z} \langle X- b\rangle $ where $ Z$ is the (finite set of zeros of $p(X)$).  We denote $\iota$ the canonical map from $k(T)^{sep} [ S \backslash T]$ and $  k(T)^{sep} [ X]$ induced by the canonical map from $k(T)^{sep} [ S \backslash T]$ and $  k(T)^{sep} [ X]$ that in turn induces the isomorphism $k(\mathfrak{P})\simeq k(\mathfrak{p})$. We have that $\mathfrak{P}k(T)^{sep} [ S \backslash T]  =\iota^{-1} ( \langle p(X) \rangle  k(T)^{sep} [ X] ) = \cap_{\underline{a} \in \iota^{-1}(Z)} \langle x_i - a_i\rangle_{i \in S\backslash T} $. Finally, we obtain 
$$\mathfrak{p} k^{sep} [S] =  \bigcap_{(a_i)_{i \in T}  \in {k^{sep}}^T } \bigcap_{(a_i)_{S\backslash T} \in \iota^{-1}(Z)} \langle x_i - a_i\rangle_{i \in S}$$
$(2) \Rightarrow (1)$ Suppose that $\mathfrak{p}k^{sep}[x_1, \cdots , x_n] = \cap_{\mathfrak{m}\in {\mathscr{M}_{sep}}} \mathfrak{m}$ where $\mathscr{M}_{sep} = \{ \langle x_1-a_1 , \cdots , x_n - a_n \rangle | a_i \in k^{sep} , \forall i \in \{ 1, \cdots, n \}  \}$. We denote $\eta : k[x_1, \cdots, x_n] \rightarrow k(T) [ S \backslash T]$ and $\mathfrak{P}= \eta ( \mathfrak{p})$. We can deduce $\mathfrak{P}k^{sep}(T)[S \backslash T] \simeq \cap_{\mathfrak{m}\in {\mathscr{M}_{sep}}} \eta(\mathfrak{m})$. As in the other implication $\mathfrak{P}$ is maximal and $k(\mathfrak{p}) \simeq k (\mathfrak{P})$ is generated by $\underline{a}\in {k^{sep}}^{S\backslash T} $ such that $f(\underline{a} )=0$ for all $ f \in \eta( \mathfrak{m})$, for all $\mathfrak{m} \in {\mathscr{M}_{sep}}$. Thus $k(\mathfrak{p})$ is finite and separable over $k(T)$. Proving that $k(\mathfrak{p})$ is finitely generated over $k(T)$.
\end{proof}

\begin{lemma} 
Let $k$ be a field, $B$ be a $k$-finitely generated algebra, and $\mathfrak{p}$ be a prime ideal of $B$. Let $\sigma: B \rightarrow B$ be an automorphism of the $k$-algebra $B$ such that for all $b \in B$, $\sigma ( b) - b \in  \mathfrak{p}$. We have $B= k[\underline{x}]/\mathfrak{a}$ and $\mathfrak{p} = \mathfrak{P}/\mathfrak{a}$ where $\mathfrak{P}$ is is a prime ideal of $k[\underline{x}]$. We suppose that $k(\mathfrak{P}) $ is separably generated over $k$.
We define $ \overline{T} : B/ \mathfrak{p}^2 \rightarrow \mathcal{L}_1(B)_{ k(\mathfrak{p})}/ (x_{1,1}^2 , \cdots , x_{1,n}^2)_{k(\mathfrak{p})}  $ to be the map induced by the map from $B/ \mathfrak{p}^2$ to $k( \mathfrak{p}) [(x_{i,j})_{(i,j)\in \{ 0 , \cdots , s\} \times \{ 1, \cdots , n\}}]/ \mathcal{L}_1(\mathfrak{a})_{k(\mathfrak{p})}$ sending $[p((x_i)_{1 \leq i \leq n})]_{\mathfrak{a}}$ to $[ [ p((x_{i,0} )_{1 \leq i \leq n})]_{\mathfrak{p}} + [\nabla{p ((x_{i,0} )_{1 \leq i \leq n})} ]_{\mathfrak{p}} \cdot ( (x_{i,1} )_{1 \leq i \leq n})^T]_{ \mathcal{L}_1(\mathfrak{a})_\mathfrak{p}} $.
The map $ \overline{T}$ is one-to-one in $ \mathcal{L}_1(B)_{k(\mathfrak{p})}/ (x_{1,1}^2 , \cdots , x_{1,n}^2)_{k(\mathfrak{p})}$. Moreover, $ \overline{T}$ makes the following diagram
$$ \xymatrix{ B/ \mathfrak{p}^2  \ar[d]^{\overline{T} } \ar[rr]^{\widetilde{\sigma}} &&  \ar[d]^{\overline{T} }  B/ \mathfrak{p}^2  \\
 \mathcal{L}_1(B)_{ k(\mathfrak{p})}\ar[rr]_{{\mathcal{L}_1(\sigma)_{k( \mathfrak{p})}}} / (x_{1,1}^2 , \cdots , x_{1,n}^2)_{k(\mathfrak{p})}&& \mathcal{L}_1(B)_{ k(\mathfrak{p})}/ (x_{1,1}^2 , \cdots , x_{1,n}^2)_{k(\mathfrak{p})} 
}$$
commute. Moreover, $\mathcal{L}_1(\sigma)_{k( \mathfrak{p})} ( \operatorname{Im} ( \overline{T}))  \subseteq  \operatorname{Im} ( \overline{T})$. 
 %Moreover $\mathcal{L}_1(\mathfrak{p})_{ k(\mathfrak{p})}^2 = ( (x_{1,j}^2)_{0\leq j \leq 1})$. 
\end{lemma} 

\begin{proof} 
We start by proving the result for finitely generated algebra. Suppose $B$ is a finitely generated algebra over $R$. 
That is there is $n \in \mathbb{N}$, $(x_i)_{1 \leq i \leq n}$ indeterminates and $\mathfrak{a}$ be an ideal of $B$ such that $B = k[x_1, x_2, \cdots, x_n]/ \mathfrak{a}$.
We have $ \mathcal{L}_1(B)_{ k(\mathfrak{p})}\simeq k(\mathfrak{p})[ (x_{i,j})_{1 \leq i \leq n, 0\leq j \leq 1}]/  \mathcal{L}_1(\mathfrak{\mathfrak{a}})_\mathfrak{p} $ .

We set ${\bf x}= (x_i)_{1 \leq i \leq n}$. 
We define the map 
$$ T : B  \rightarrow k(\mathfrak{p})[ (x_{i,j})_{1 \leq i \leq n, 0\leq j \leq 1}]/  \mathcal{L}_1(\mathfrak{a})_\mathfrak{p}$$
sending $[p((x_i)_{1 \leq i \leq n})]_{\mathfrak{a}}$ to $[ [ p((x_{i,0} )_{1 \leq i \leq n})]_{\mathfrak{p}} + [\nabla{p ((x_{i,0} )_{1 \leq i \leq n})} ]_{\mathfrak{p}} \cdot ( (x_{i,1} )_{1 \leq i \leq n})^T]_{ \mathcal{L}_1(\mathfrak{a})_\mathfrak{p}} $ \\
where $ \nabla{p ((x_{i,0} )_{1 \leq i \leq n})}$ is the gradient of $p$ seen as a polynomial in the indeterminates $(x_{i,0} )_{1 \leq i \leq n}$ vector evaluated at $(x_{i,0} )_{1 \leq i \leq n}$. This map is a map as $k$-linear vector space. 
We prove that the kernel of $T$ is $ker(T) =\mathfrak{p}^2$. 
Let $f({\bf x}) \in \mathfrak{p}^2$. Then $f({\bf x}) = \sum_{k=1}^s r_{k}({\bf x} ) t_k({\bf x} )  s_k ({\bf x} )$ where $r_k({\bf x} )\in  \mathfrak{p}$ and $ s_k ({\bf x} ),t_k({\bf x} )  \in k[{\bf x}]$. We have 
$$\partial f ({\bf x} )/ \partial {x_i} ({\bf x} )  = \sum_{k=1}^s ( \partial r_k / \partial {x_i}({\bf x} ) t_k({\bf x} )  s_k ({\bf x} ) + r_k({\bf x} ) \partial t_k / \partial {x_i}({\bf x} )   s_k ({\bf x} )+ r_{k}({\bf x} ) t_k({\bf x} ) ( \partial s_k / \partial {x_i}({\bf x} ))\in \mathfrak{p}$$ 
Therefore, We have $[ f((x_{i,0} )_{1 \leq i \leq n})]_{\mathfrak{p}}=[0]_{\mathfrak{p}}$ and $[\nabla{f ((x_{i,0} )_{1 \leq i \leq n})} ]_{\mathfrak{p}}= [0]_{\mathfrak{p}}$. That is $f({\bf x}) \in ker(\overline{T})$


Let $f({\bf x}) \in ker(T)$. We prove that $f(\underline{x})\in \mathfrak{p}^2$.

We first prove the result when $k$ is an algebraically closed field, $B = k [\underline{x}]$ and $\mathfrak{p}$ is maximal. There exists $a_i \in k$ for $i \in \{ 1, \cdots , n \}$ such that $\mathfrak{p}= \langle x_i-a_i\rangle_{i \in \{ 1, \cdots , n \}}$. %where $J \subset \{ 1, \cdots , n \}$. %We consider the evaluation map $e_\mathfrak{p} : B \rightarrow k$ sending $p((x_i)_{1 \leq i \leq n})$ to $p((a_i)_{1 \leq i \leq n})$. 
We have by the assumption that $f((a_{i} )_{1 \leq i \leq n})=0$ and $\nabla{f ((a_{i} )_{1 \leq i \leq n}})=0$. Therefore $f({\bf x}) \in \mathfrak{p}^2$. Indeed, simply write $f({\bf x})= c_{0} + \sum_{\bar{i}\in S_1 } c_{\bar{i}} ({\bf x}-{\bf a})^{\bar{i}}+  \sum_{\bar{i}\in S} c_{\bar{i}} ({\bf x}-{\bf a})^{\bar{i}}$ where $S_1 =\{ \bar{i} \in \mathbb{N}^n | |\bar{i} |=1 \}$ and $S =\{ \bar{i} \in \mathbb{N}^n | | \bar{i}| >1  \}$. %For $\bar{i} \in S_1$ such that $i_j  = 1$ for some $j \in \{ 1, \cdots, n\}$ and $i_k =0$, $\forall k \in \{ 1, \cdots, n\}$.  
We have $c_{\bar{i}}=  \partial (f({\bf x}))/\partial x_j$ giving us the result, since $f({\bf a}) =0$ and $\partial (f({\bf a}))/\partial x_j=0$ by assumption.

When $k$ is not algebraically closed  $B = k [\underline{x}]$ and $\mathfrak{p}$ is separably generated prime. %We set $\overline{k}$ to be an algebraic closure of $k$. 
By the previous lemma, we have $\mathfrak{p}k^{sep}[x_1, \cdots , x_n] = \cap_{\mathfrak{m}\in {\mathscr{M}_{sep}}} \mathfrak{m}$ where $\mathscr{M}_{sep} = \{ \langle x_1-a_1 , \cdots , x_n - a_n \rangle | a_i \in k^{sep} , \forall i \in \{ 1, \cdots, n \}  \}$.
%Let $\{ \mathfrak{m}_i\}_{i \in I}$ be the set of distinct maximal ideals containing $\mathfrak{p} k^{sep}[x_1, \cdots, x_n]$ in $ k^{sep}[x_1, \cdots, x_n]$. By Lemma 10.43.6. Stack project, we have that $\mathfrak{p}k^{sep}[x_1, \cdots, x_n] = \cap_{i \in I} \mathfrak{m}_i$ and 
Moreover, $ \cap_{\mathfrak{m}\in {\mathscr{M}_{sep}}} \mathfrak{m}^2 \subseteq \mathfrak{p}^2 k^{sep}[x_1, \cdots, x_n] $ . We have $[ f((x_{i,0} )_{1 \leq i \leq n})]_{\mathfrak{m}}=[0]_{\mathfrak{m}}$ and $[\nabla{f ((x_{i,0} )_{1 \leq i \leq n})} ]_{\mathfrak{m}}= [0]_{\mathfrak{m}}$ for all ${\mathfrak{m}\in {\mathscr{M}_{sep}}}$. Therefore by the above $f({\bf x})\in \mathfrak{m}^2$ for all ${\mathfrak{m}\in {\mathscr{M}_{sep}}}$. Thus $f({\bf x})\in \mathfrak{p}^2k^{sep}[x_1, \cdots, x_n]$. We have $f({\bf x}) = \sum_{k=1}^s r_k({\bf x} ) t_k({\bf x} ) m_k({\bf x} )$ where $ r_k({\bf x} ) ,t_k({\bf x} ) \in \mathfrak{p}$  and $m_k({\bf x} ) \in k^{sep}[x_1, \cdots, x_n]$. Let $L$ be the extension generated by all the coefficient of $m_k({\bf x} )$ for all $k \in \{ 1, \cdots , s\}$ then $L$ is a finite extension and since $L[{\bf x}]$ is a integral extension of $k [{\bf x}]$. Thus $f({\bf x})\in \mathfrak{p}^2$. 


We denote $\overline{T}_{B/ \mathfrak{p}^2} : B/ \mathfrak{p}^2 \rightarrow \mathcal{L}_1(B)_{ k(\mathfrak{p})}/ (x_{1,1}^2 , \cdots , x_{1,n}^2)_{k(\mathfrak{p})}$.
Now let us consider the general case. We have that from the correspondence theorem for a prime ideal that $\mathfrak{p}= \mathfrak{P}/\mathfrak{a}$ where $\mathfrak{P}$ is a prime ideal of $ k[{\bf x}]$. We have $k(\mathfrak{p}) \simeq k(\mathfrak{P})$. We consider the following diagram 
$$\xymatrix{ & 0 & 0  &  \\ 
& \left( \frac{ \mathfrak{P}}{\mathfrak{a}} \right)^2 \ar[r] \ar[u] & k[{\bf x}]/ \mathfrak{a} \ar[rr]^{\overline{T}_{k[\underline{x}]/\mathfrak{a}/ \left( \mathfrak{P}/ \mathfrak{a} \right)^2} }  \ar[u]& &  \operatorname{im} (\overline{T}_{k[\underline{x}]/\mathfrak{a}/ \left( \mathfrak{P}/ \mathfrak{a} \right)^2} ) \ar[r] & 0 \\ 
0\ar[r] &  \mathfrak{P}^2 \ar[r]\ar[u] & k[{\bf x}] \ar[rr]^{\overline{T}_{k[\underline{x}]/ \mathfrak{P}^2}} \ar[u] &&\operatorname{im} (\overline{T}_{k[\underline{x}]/ \mathfrak{P}^2}) \ar[u]^{\iota} \ar[r] & 0 \\
0\ar[r] & \mathfrak{P}^2 \cap \mathfrak{a} \ar[r] \ar[u] & \mathfrak{a} \ar[u] \\%\ar[rr]^{\overline{T}_{\mathfrak{a}/ \mathfrak{P}^2}} \ar[u] & & \operatorname{im} ( \overline{T}_{ (\mathfrak{P} \backslash \mathfrak{a})^2})\ar[u]^{\iota_1}  \ar[r] & 0 \\
& 0 \ar[u] & 0\ar[u]  && %0\ar[u] 
}$$

Chasing the diagram, we obtain that $\iota$ is an isomorphism. From there we can also prove that the following sequence 
$$\xymatrix{0\ar[r] & \left( \frac{ \mathfrak{P}}{\mathfrak{a}} \right)^2 \ar[r] & k[{\bf x}]/ \mathfrak{a} \ar[rrr]^{\overline{T}_{k[\underline{x}]/\mathfrak{a}/ \left( \mathfrak{P}/ \mathfrak{a} \right)^2} } & & & \operatorname{im} (\overline{T}_{k[\underline{x}]/\mathfrak{a}/ \left( \mathfrak{P}/ \mathfrak{a} \right)^2} ) \ar[r] & 0}$$
is exact.

We set $ {p_\sigma} ( x,y):= \sigma (p(x,y)) $. In particular $x_\sigma (x,y) = \sigma (x)$ and $y_\sigma (x,y) = \sigma (y)$. 
We have $${x_\sigma} ( x_0+[t]_1 x_1,y_0+[t]_1 y_1)= {x_\sigma}(x_0, y_0) + D_{{x_\sigma}, 1}(x_0, x_1, y_0, y_1) [t]_1$$ and 
$${y_\sigma} ( x_0+[t]_1 x_1,y_0+[t]_1 y_1)= q_{y_\sigma}(x_0, y_0) + D_{{y_\sigma}, 1}(x_0, x_1, y_0, y_1) [t]_1$$

We have $\kappa_1(p(x,y)) = T_{p,1}(a, x_1, b, y_1) $. We have \\
$$\begin{array}{lll} \mathcal{L}_1(\sigma)(T_{p,1}(x_0, x_1, y_0, y_1))&=& T_{p,1} ({x_\sigma} ,D_{{x_\sigma}, 1}, {y_\sigma} ,D_{{y_\sigma}, 1})\\
&=& p( {x_\sigma},  {y_\sigma}) + D_{p,1}({x_\sigma} ,D_{{x_\sigma}, 1}, {y_\sigma} ,D_{{y_\sigma}, 1})
\end{array}$$

%That is $f({\bf x} ) = \sum_{k=1}^s r_{k}({\bf x} ) s_k ({\bf x} )$ where $r_k({\bf x} )\in  \mathfrak{p}$ and $ s_k ({\bf x} ) \in k[{\bf x}]$. We have $\partial f ({\bf x} )/ \partial {x_i} ({\bf x} )  = \sum_{k=1}^s ( \partial r_k / \partial {x_i}({\bf x} ) s_k ({\bf x} ) + r_{k}({\bf x} )( \partial s_k / \partial {x_i}({\bf x} ))$. 
%Since $\sum_{k=1}^sr_{k}({\bf x} )( \partial s_k / \partial {x_i}({\bf x} )) \in  \mathfrak{p} $, we obtain $\sum_{k=1}^s  \partial r_k / \partial {x_i}({\bf x} ) s_k ({\bf x} )\in \mathfrak{p}$.  Then $f({\bf x} )\in \mathfrak{p}^2$. 


%In any case, there I am assuming that k is perfect, if you prefer.
%In case of perfect field your question boils down to asking if p is regular in B. SO f\in p is also in p^2 if and only if d_j(f) \in p for all j. THIS is the jacobian criterion of regularity over an algebraically closed field and p maximal. If k is not algebraically closed and p is still maximal, just tensorize by overline{k} and you lose no information bevause of perfectness. If p is not maximal, then, you still tensorize with \overline{k} and then you choose a point \overline{p} that "lifts" p. \overline{p} is regular if and only if there is a maximal that contains that and it is regular; and in that case the maximal ideals that contain p with that property are an open subset of V(p), so you throw a closed subset and assume that all the maximal that contain p have that property. Then you write p as the intersection of all maximals that contain p (you can do that in the finitely gen case;  notice that we have the fin gen in L_1 \otimes B/q^2 just by assumning that q is fin gen in B, so it is bery mild condition that doesn not require that B is itself noetherian); morevover p^2 is the intersection of the squares of the maximal ideals. Thus if what i said holds for regular maximals it holds also for all the regular primes.

%$f = q p+r$
%
%$f=p(a, b) + (x-a) f_y(a,b) + (y-b) f_x(a,b)$. 

\end{proof} 



\begin{exmp} 
Let $B=k[x]/ (x^2-y)^2$. We consider $\sigma : B \rightarrow B$ sending $ [x]$ to $ [x+ (x^2 -y) x]$. It is an involution $\sigma^2 ([x]) = \sigma ( [x+ (x^2 -y) x]) = [x+ (x^2 -y) x +  (x^2 -y) x]=[x]$. 
\begin{enumerate} 
\item Suppose that $k =\mathbb{F}_2(y)$ and set $\mathfrak{p}:= \frac{ (x^2-y)}{(x^2-y)^2}$. We have that $\sigma ( [x]) -  [x])\notin \mathfrak{p}^2$. We have $\mathcal{L}_1(\sigma)_{k ( \mathfrak{p})}  ([x_0]) = [x_0]$ and $\mathcal{L}_1(\sigma)_{k ( \mathfrak{p})}  ([x_1]) = [x_1]$. 
\item Suppose that $k =\mathbb{F}_2(y)[z]/(y^2-z)$ where $z= y^2$. Let $\mathfrak{m}= \frac{ (x-z)}{(x^2-y)^2}$ be a maximal ideal containing $\mathfrak{p}:= \frac{ (x^2-y)}{(x^2-y)^2}$. $\sigma ( [x]) -  [x] \in \mathfrak{m}^2$. We have $\mathcal{L}_1(\sigma)_{k ( \mathfrak{p})}  ([x_0]) = [x_0]$ and $\mathcal{L}_1(\sigma)_{k ( \mathfrak{p})}  ([x_1]) = [x_1]$.
\end{enumerate} 
Let $B=k[x,z]$. $(z-a) \in Spec (B)$. 
\end{exmp} 

\begin{lemma} 
 Let $B = k \oplus (\oplus_{i=1}^r x_i k) \oplus ( \oplus_{1\leq i\leq j \leq r} x_i \cdot x_j  k/ \mathbf{L})$ where $\mathbf{L}$ is a linear subspace of $\oplus_{1\leq i\leq j \leq r} x_i \cdot x_j k$. Let $\sigma : B \rightarrow B$ be an automorphism of $k$-algebras such that $ \sigma( x_i) - x_i = \sum_{1\leq j \leq l \leq r } h_{jl}^i \cdot x_j x_l$ for all $i\in \{ 1, \cdots, r\}$ and assume that there is $i_0 \in \{ 1, \cdots, r\}$ such that $ \sum_{1\leq j \leq l \leq r } h_{jl}^{i_0} \cdot x_j x_l \neq 0$. (In other words, $\sigma \in G_1 ( (\overline{x} )) \backslash G_2 (( \overline{x}) )$. 
 Then there exists $\mathfrak{q} \in \operatorname{Spec} ( \mathcal{L}_1(B) \otimes_B B/ \mathfrak{m})$, there exists $\alpha \in \mathcal{L}_1(B)$ such that $ \mathcal{L}_1(B) (\alpha) - \alpha \notin \mathfrak{q}^2$ (In other words, $ \mathcal{L}_1(\sigma) \notin G_1 (\mathfrak{q})$).  
 
 \sophie{should it be $\mathfrak{q} \in \operatorname{Spec} ( \mathcal{L}_1(B) \otimes_B B/ \mathfrak{m}^2)$?}
\luigi{Since $\mathfrak{m}$ is contained in $\sqrt{0} \subseteq B/\mathfrak{m}^2$, topologically $\operatorname{Spec} ( \mathcal{L}_1(B) \otimes_B B/ \mathfrak{m}^2)=\operatorname{Spec} ( \mathcal{L}_1(B) \otimes_B B/ \mathfrak{m})$, i.e. the primes are the same; we will, in any case, take the primes in the fibre over $\mathfrak{m}$.}

 \sophie{Because of the remark, otherwise, I do not understand the Remark? Is $B$ an algebra how so? what is $\mathfrak{m}$ in terms of $B$? is $\mathfrak{m}$ and $(\overline{x})$ the same thing?}
\luigi{Yes, $\mathfrak{m}$ is generated by the $x_i$; the algebra structure in $B$ comes from the fact that the product of $x_i$ and $x_j$ is the $x_ix_j$ that is among the generators of the "degree 2 " part}.

  \sophie{Are we acting trivially on $\otimes_B B/ \mathfrak{m}^2$? }
\luigi{We are acting on $B/\mathfrak{m}$ via the restriction of $\sigma$.  If you prefer the construction is, you start with $B$, then construct the $B-$algebra $\mathcal{L}_1(B)$, where $\mathcal{L}_1(\sigma)$ is defined, then you quotient with respect to the extension of the ideal $\mathfrak{m}^2$, and since $\sigma(\mathfrak{m}^2) \subseteq \mathfrak{m}$, then $\mathcal{L}_1(\sigma)$ descends on $\mathcal{L}_1(B)\otimes_B B/ \mathfrak{m}^2$.}
 \end{lemma}


==> chapters/schemadejets.tex <==




\begin{definition} \cite[\S 2]{EM}
Let $m\in \mathbb{N}$. We define the {\sf $m^{th}$ jet algebra functor at $B$} to be the covariant functor defined by
$$\begin{array}{llll} \underline{J_m(B)} : & \mathbf{Alg}_R &  \rightarrow & \mathbf{Sets}\\
& C & \mapsto & \operatorname{Hom}_{ \mathbf{Alg}_R}( B ,C [t]/ (t^{m+1}) )\\
& \varphi  & \mapsto & \tilde{\varphi}_*
\end{array},$$ 
When $\underline{J_m(B)}$ is representable is the category of $R$-algebras, we call {\sf $m^{th}$ jet algebra at $B$} denoted $\mathcal{L}_m (B)$ over $R$ the $R$-algebra representing the functor $\underline{J_m(B)}$. 
\end{definition}

The following Lemma/definition, give the construction of a jet $R$-algebra from an algebra of finite type. 
\begin{definition}(Lemma) \cite[\S 2]{EM} \label{defft}
Let $m\in \mathbb{N}$. Let $B$ be a $R$-algebra of finite type. We write $ B = R[x_1, \cdots , x_n]/ I$ for some ideal $I$.
\begin{enumerate}  
\item We have $$\mathcal{L}_m (B)= R[(x_{s,j})_{(s,j) \in \{1, \cdots, n\} \times  \{0, \cdots, m\}  } ]/ \mathcal{L}_m(I)$$ where $\mathcal{L}_m(I)$ denotes the ideal
$$ \left< g^m_{h,j}\in R[(x_{i,j})_{(i,j) \in \{1, \cdots, n\} \times  \{0, \cdots, m\} }]|  h\left( \left( \sum_{j=0}^m x_{i,j} [t]_{m}^j \right)_i \right) = \sum_{j=1}^m g^m_{h, j} [t]_{m}^j, h\in I, j\in  \{0, \cdots, m\} \right>$$ with $R[(x_{i,j})_{(i,j) \in \{1, \cdots, n\} \times  \{0, \cdots, m\}  }]$ is the polynomial ring on the interminates \\ 
$(x_{i,j})_{(i,j) \in \{1, \cdots, n\} \times  \{0, \cdots, m\}}.$ 

%The functor $\underline{J_m(B)}$ is representable by the $R$-algebra $\mathcal{L}_m(B)$. More precisely, 
Moreover, we have a natural correspondence $\eta_m^B$ from $ \underline{J_m(B)}$ to $ \underline{\mathcal{L}_m(B)}$  (resp. $\epsilon_m^B$ from $ \underline{\mathcal{L}_m(B)}$ to $ \underline{J_m(B)}$) defined by for every $C$ $R$-algebra, 
$$\begin{array}{cccc} {\eta_m^B}_C: &   \operatorname{Hom}_{ \mathbf{Alg}_R}( \mathcal{L}_m(B) , C ) & \rightarrow & \operatorname{Hom}_{ \mathbf{Alg}_R}( B , C [t]/ (t^{m+1})) \\
& \psi & \mapsto &  {\eta_m^B}_C(\psi)
\end{array}
$$
where $ {\eta_m^B}_C(\psi) : B  \rightarrow C [t]/ (t^{m+1})$ sending $[x_i]_{I}$ to $\sum_{j=0}^m \psi ( [x_{i,j}]_{\mathcal{L}_m(I)}) [t]_m^j$, for all $i \in \{ 1, \cdots, n\}$
and 
$$\begin{array}{cccc} {\epsilon_m^B}_C:  &  \operatorname{Hom}_{ \mathbf{Alg}_R}( B , C [t]/ (t^{m+1})) & \rightarrow  &  \operatorname{Hom}_{ \mathbf{Alg}_R}( \mathcal{L}_m(B) , C ) \\
& \phi & \mapsto &   {\epsilon_m^B}_C( \phi) 
\end{array}
 $$
 where $ {\epsilon_m^B}_C(\phi) : \mathcal{L}_m(B) \rightarrow C $ sending $[x_{i,j}]_{\mathcal{L}_m(I)}$ to $c_{i,j}$ defined by $\phi ( [x_i]_I) = \sum_{j=0}^m c_{i,j} [t]_m^j$. $\eta_m^B$ and $\epsilon_m^B$ are inverses of each other.
 
%%%
%\item Let $s\in \mathbb{N}$ with $s \leq m$. We define the canonical $R$-algebra morphism 
% $$\begin{array}{cccc} \sigma_{m,s}^B: & B & \rightarrow &\mathcal{L}_s(B)[t]/ (t^{m+1})\\ & [x_i]_{I} & \mapsto & \sum_{j=1}^{s} [x_{i,j}]_{J_s(I)} [t]_m^j\end{array}$$
% \sophie{ Question: I am not sure if we can define this map when $m<  s$}
% for any $i \in \{ 1, \cdots, n \}$. We note that $\epsilon_{m}^B (  \sigma_{m, m}^B)= \operatorname{Id}_{\mathcal{L}_m(I)}$. For $m=0$, we denote $ \sigma_{m,s}^B$ by $ \sigma_{s}^B: B  \rightarrow \mathcal{L}_s(B)$. \sophie{ I have some problem defining this please help}
%%%

\item Let $s\in \mathbb{N}$ with $s\geq m$. The truncation maps ${\tau}^C_{m, s} \colon  C[t]/(t^{s+1})\rightarrow C[t]/(t^{m+1})$ where $C$ is a $R$-algebra induces a natural transformation of functors
$$ {\tau_{m,s}^{(-)}}_* \colon  \operatorname{Hom}_{ \mathbf{Alg}_R}( B , - \otimes_R R [t]/ (t^{s+1}) )\ \rightarrow \operatorname{Hom}_{ \mathbf{Alg}_R}( B , -\otimes_R R [t]/ (t^{m+1}) )  $$
which is identified, via the natural correspondences $\eta_m^B$ and $\epsilon_m^B$ and Yoneda Lemma to with the morphism of $R-$algebras  $\mu^B_{m,s}  := (\epsilon_m^B \circ \tau_{m, s}^{(-)} \circ \eta_s^B)_{\mathcal{L}_s(B)} ( id_{\mathcal{L}_s(S)})$. That is, 
$$\begin{array}{cccc}
\mu^B_{m,s} \colon & \mathcal{L}_m (B) & \rightarrow & \mathcal{L}_s(B) \\
  & [x_{i,j}]_{\mathcal{L}_m (I)} &\mapsto  & [x_{i,j}]_{\mathcal{L}_s (I)}  
\end{array}
$$
In other words, ${\mu^{B}_{m,s}}^\ast\circ \epsilon_{s}^B=\epsilon_{m}^B\circ {\tau_{m,s}^B}_{\ast}$ and $\eta_{m,C}^B \circ {\mu^{B}_{m,s}}^{\ast}= {\tau_{m,s}^B}_{\ast}\circ \eta_{s,C}^B$.

%%%%
%\item %We defines a canonical $R$-algebra morphism $\mu^B_{m}: \mathcal{L}_m (B)\rightarrow B$ sending $[x_{1,j}]_{J_m (I)}$ to $[x_1]_I$ and $[x_{i,j}]_{J_m (I)}$ to $0$ when $i\neq 1$. That is $\mu^B_{m}= \epsilon_B(e_m^B)$. %We also define a canonical $R$-algebra morphism $\rho_m^B : B \rightarrow \mathcal{L}_m(B)$ sending $ [x_1]_I$ to $[x_{1, j}]_{J_m(I)}$. 
%Let $s\in \mathbb{N}$ with $s \leq m$. We define a canonical $R$-algebra morphism $\mu^B_{m,s}: J_m (B)\rightarrow J_s(B)$ sending $[x_{i,j}]_{J_m (B)}$ to $[x_{i,j}]_{J_s (B)}$ for all $i \in \{ 1, \cdots, n \}$ and $j \in \{0 , \cdots , \operatorname{min}(s,m) \}$ and $[x_{i,j}]_{J_m (B)}$ to  0 otherwise. We have $\mu^B_{m,s} = {\epsilon_m}_C^B ( \sigma_{m,s}^B)$. In particular, when $s=0$, we denote $\mu^B_{m,0}$ simply as $\mu^B_{m}$. We have $\mu^B_{m} \circ  \sigma_{m}^B = \operatorname{Id}_B$.

\item %Consider the standard inclusion $\iota^B\colon B\rightarrow B[t]/(t^{m+1})$ and let 
Let $s\in \mathbb{N}$. We have $\sigma_s^B \colon = \epsilon_{s,B}^B(\iota^B_s) \colon \mathcal{L}_s(B)\rightarrow B$. Then $\sigma_s^B\circ \mu^B_{s,0}=\mathbf{id}_B$. 
\item We also set $\rho^B_{m,s}:={\eta_m^B}_{\mathcal{L}_s(B)} ( \mu_{m,s}^B) $. We have $$\begin{array}{cccc} \rho_{m,s}^B: & B & \rightarrow &\mathcal{L}_s(B)[t]/ (t^{m+1})\\ & [x_i]_{I} & \mapsto & \sum_{j=1}^{m} [x_{i,j}]_{\mathcal{L}_s(I)} [t]_m^j.\end{array}$$
\end{enumerate}

%When $X$ and $J_m(X)$ are not necessarily affine, gluing this construction from an affine covering defines $Spec(R)$-scheme morphism $s_X: X \rightarrow J_m(X)$. 

%When $s<m$. We have the canonical morphism denote $\rho_{m,s}^B$ from $J_s (B)$ to $J_m (B)$ sending the class of $([x_{i,j}]_{J_m(I)})_{(i,j) \in \{1, \cdots, n\} \times  \{0, \cdots, s\}}$ in $J_s(B)$ to the class of $([x_{i,j}]_{J_m(I)})_{(i,j) \in \{1, \cdots, n\} \times  \{0, \cdots, s\}}$ in $J_m(B)$. In particular when $m=0$, we obtain a canonical morphism from $B$ to $ J_s (B)$. Moreover, $\mu^B_m \circ \rho_{m,0}^B= Id_B$. We also have $
\end{definition} 
\begin{proof} 
Part of this proof are an adaptation of \cite[Proposition 2.2]{EM}

%, we know that $J_m(X)$ exists for every scheme $X$ of finite type over $k$ and is again a scheme of finite type over $R$. In particular, when $X$ is an affine scheme of finite type over $R$, we do a proof similar to \cite[Proposition 2.2]{EM} gives a construction for an affine $J_m (X)$ for a general commutative unitary ring as follows. Suppose that $X = Spec(B)$ where 
\begin{enumerate}
\item Suppose that $B = k[x_1, \cdots , x_n]/ I$. %where $I= ( f_1, \cdots, f_t)$, with $f_s \in k[x_1, \cdots , x_n]$, for all $s \in \{ 1, \cdots , t \}$. 
For every $R$-algebra $C$, since giving a morphism $\phi: R[x_1, \cdots, x_n]/I\rightarrow C[t]/(t^{m+1})$ is equivalent to giving $u_i=\phi ( x_i)=\sum_{j=0}^m c_{i,j} [t]_{m}^j$ such that \\ $h( u_1, \cdots, u_n)=0$ %for all $s \in \{1, \cdots, t\}$, 
for all $h \in I$, where $c_{i,j} \in C$, for all $i\in \{ 1, \cdots, n \}$ and $j \in \{ 0, \cdots, m\}$. %and $\bar{t}$ is the class of $t$ in the quotient $C[t]/(t^{m+1})$. 
%We consider $k[(x_{i,j})_{(i,j) \in \{1, \cdots, n\} \times  \{0, \cdots, m\} }]$ the polynomial ring on the interminates \\ $(x_{i,j})_{(i,j) \in \{1, \cdots, n\} \times  \{0, \cdots, m\}}.$ Let $s\in\{ 1, \cdots, t\}$. 

Let $h\in I$. There is $g^m_{h,j}\in k[(x_{i,j})_{(i,j) \in \{1, \cdots, n\} \times  \{0, \cdots, m\} }]$ such that if we set $p_{i}([t]_{m}):=\sum_{j=0}^m x_{i,j} [t]_{m}^j$ with $i \in \{ 1, \cdots, n\}$, we have 
$$h ( p_{1}([t]_{m}), \cdots , p_{n}([t]_{m}))= \sum_{j=1}^m g^m_{h, j}[t]_{m}^j.$$
Then $\underline{J_{m}(B)}$ is represented by $\mathcal{L}_m (B)$ defined as 
$$\mathcal{L}_m (B)= R[(x_{i,j})_{(i,j) \in \{1, \cdots, n\} \times  \{0, \cdots, m\}  } ]/ \left< (g^m_{h,j})_{(h,j) \in I \times  \{0, \cdots, m\}}\right>.$$
Indeed, one proves that $\eta_m^B$ is well-defined by noting that keeping the notation of the statement
$${\eta_m^B}_C (\psi) = \tilde{\psi} \left( \sum_{j=0}^m [x_{i,j}]_{\mathcal{L}_m(I)} [t]_m^j\right).$$ 
Moreover, given $\phi\in  \operatorname{Hom}_{ \mathbf{Alg}_R}( B , C [t]/ (t^{m+1}))$, we have by definition of $\phi$, that for every $h \in I$, $\phi ([h]_I)=\sum_{j=0}^m g^m_{h,j}( (c_{i,j})_{i,j}) [t]_{m}^j=0$. That is $g_{h,j}( (c_{i,j})_{i,j})=0$ for all $j \in \{ 0 , \cdots, m\}$. Equivalently, $l ( (c_{i,j})_{i,j})=0$, for all $l \in \mathcal{L}_m (I)$. Proving that ${\epsilon_m^B}_C$ is well-defined for every $R$-algebra $C$. One then prove that $\epsilon$ and $\eta$ are natural transformations such that $$\epsilon_m^B \circ \eta_m^B = \operatorname{Id}_{\operatorname{Hom}_{ \mathbf{Alg}_R}( \mathcal{L}_m(B) , C )} \text{ and } \eta_m^B\circ \epsilon_m^B =\operatorname{Id}_{\operatorname{Hom}_{ \mathbf{Alg}_R}( B , - \otimes_R R [t]/ (t^{m+1}))}.$$ 
%\item $\sigma_{m,s}^B$ is well-defined since for any $h \in I$, we have 
%$$\begin{array}{ccll} \sigma_{m,s}^B ( [h]_I) &=&  [ h ( \sum_{j=0}^{s} x_{i,j} [t]_m^j)]_{J_s(I)J_s(B)[t]/ (t^{m+1})} \\
%& =& [ \sum_{j=0}^{s} g_{h,j}^{s}[t]_m^j]_{J_s(I)J_s(B)[t]/ (t^{m+1})}=[0]_{J_s(I)J_s(B)[t]/ (t^{m+1})}.\end{array}$$ 
%\item The well-definiteness of  $\mu^B_{m,s}$ respectively is guaranteed by the equalities $\mu^B_{m}= \epsilon_B(e_m^B)$, 

\item We have, 
$$\begin{array}{clll} {\eta_s^B }_{\mathcal{L}_s(B)} ( id_{\mathcal{L}_s(B)}) : &B& \rightarrow & \mathcal{L}_s(B) [t]/(t^{s+1}) \\
& [x_i]_I &\rightarrow  & \sum_{j=1}^s [x_{i,j}]_{\mathcal{L}_s(B)} [t]^j_s.
\end{array}$$
Therefore, 
$$\begin{array}{clll} {\tau_{m,s \ \ast}^{\mathcal{L}_s(B)}} ({\eta_s^B }_{\mathcal{L}_s(B)} ( id_{J_s(B)})) : &B& \rightarrow & \mathcal{L}_s(B) [t]/(t^{m+1}) \\
& [x_i]_I &\rightarrow  & \sum_{j=1}^m [x_{i,j}]_{\mathcal{L}_s(B)} [t]^j_m.
\end{array}$$
Finally, 
$$\begin{array}{clll} {\epsilon_m^B}_{\mathcal{L}_s(B)} ({\tau_{m,s}^{\mathcal{L}_s(B)}}_\ast ({\eta_s^B }_{\mathcal{L}_s(B)} ( id_{\mathcal{L}_s(B)})) ): &\mathcal{L}_m(B) & \rightarrow & \mathcal{L}_s(B) \\
& [x_{i,j}]_{\mathcal{L}_m(I)} &\rightarrow  & [x_{i,j}]_{\mathcal{L}_s(B)} 
\end{array}$$
Proving the result.
%\luigi{I am writing a proof of well-definiteness of $\mu$, but if it is unnecessary we can delete it.}
%We begin by showing that $\mu^B_{m,s}$ is a well defined map of $R-$algebras,  i.e. that $J_m(I)$ is contained in the kernel of the map of $R-$algebras $\overline{\mu}\colon R[(x_{i,j})_{1\leq i\leq n, 0\leq j\leq n}]\rightarrow J_s(B)$ sending $x_{i,j}$ to $[x_{i,j}]_{J_s(I)}$. Let $h\in I$, then $h((x_{i,0}+\cdots+t^m x_{i,m})_{i\in \{1,\dots\}}) \equiv h((x_{i,0}+\cdots+t^s x_{i,s})_{i\in \{1,\dots\}}) \pmod t^{m+1}$ $g_{h,j}^m=g_{h,j}^s\in J_s(I)$ for all $j\in \{0,\dots,m\}$, so $J_m(I)$ is generated by polynomials that are mapped to 0 by $\overline{\mu}$, hence $\overline{\mu}$ descends to $\mu^B_{m,s}$.
%
%Let $\phi\in \operatorname{Hom}_{ \mathbf{Alg}_R}(B, C[t]/t^{s+1})$ and, for $i\in \{1,\dots, n\}$, $j\in \{0,\dots, s\}$, let $c_{i,j}\in C$ be such that $\phi(x_i)=c_{i,0}+\cdots+c_{i,s}t^s$; then we have that ${\tau_{m,s}^{C}}_\ast(\phi)(x_i)= c_{i,0}+\cdots+c_{i,m}t^m$, therefore $\epsilon_s^B({\tau_{m,s}^{C}}_\ast(\phi))([x_{i,j}]_{J_m(I)})=c_{i,j}$, $\forall (i,j)\in \{1,\dots, n\}\times\{0,\dots, m\}$. On the other hand, for every $i\in\{1,\dots, n\}$ and every $j\in \{0,\dots, m\}$ we have
%\begin{align*}
%{\mu^B_{m,s}}^\ast(\epsilon_s^B(\phi)) ([x_{i,j}]_{J_m(I)}) & = \epsilon_s^B(\phi) (\mu_{m,s}^B([x_{i,j}]_{J_m(I)})) \\
%& = \epsilon_s^B(\phi) ([x_{i,j}]_{J_s(I)}) \\
%& = c_{i,j}  \, .
%\end{align*}
%Hence ${\mu^{B}_{m,s}}^\ast\circ \epsilon_{s}^B=\epsilon_{m}^B\circ {\tau_{m,s}^B}_{\ast}$.
%
%Finally
%\begin{align*}
%\eta_m^B\circ {\mu^{B}_{m,s}}^\ast= {\tau_{m,s}^B}_{\ast} \circ \eta_s^B      & \Leftrightarrow \eta_m^B\circ {\mu^{B}_{m,s}}^\ast\circ \epsilon_{s}^B= {\tau_{m,s}^B}_{\ast} \\
%& \Leftrightarrow  {\mu^{B}_{m,s}}^\ast\circ \epsilon_{s}^B=\epsilon_{m}^B\circ {\tau_{m,s}^B}_{\ast}  \, .
%\end{align*}

\item Clearly $\tau^B_{s,0}\circ\iota^B_s=\mathbf{id}_B$, hence
\begin{align*}
\sigma_s^B\circ \mu^B_{0,s}  &= ({\mu^{B}_{0,s}}^\ast\circ \epsilon_{s}^B)(\iota^B_s) \\
 & =  (\epsilon_{0}^B\circ {\tau_{0,s}^B}_{\ast})(\iota^B_s) \\
& =  \epsilon_{0}^B(\mathbf{id}_B)= \mathbf{id}_B \, .
\end{align*}

\item We have,
\begin{align*}
({\eta_m^B}_{\mathcal{L}_s(B)} ( \mu_{m,s}^B)) ([x_i]_I) & = \left(\left({ {\eta_m^B}_{\mathcal{L}_s(B)} \circ {\mu_{m,s}^B}^\ast }\right) (\mathbf{id}_B)\right) ([x_i]_I) \\
& = {\tau_{m,s}^B}\left( \left( \eta_{s, \mathcal{L}_s(B)}^B (\mathbf{id}_B) \right) ([x_i]_I) \right) \\
&= \tau_{m,s}^B\left( \sum_{j=1}^s [x_{i,j}]_{\mathcal{L}_s(I)} [t]^j_s \right) \\
&= \sum_{j=1}^m [x_{i,j}]_{\mathcal{L}_s(I)} [t]^j_m \, .
\end{align*}
 

\end{enumerate}
%
%For $s< m$ and $C$ any $R$-algebra, we have the canonical morphism $\iota_{s, m} : C[t]/(t^{s+1})\rightarrow C[t]/(t^{m+1})$ sending $\sum_{j=0}^s c_{i,j} [t]_{s}^j$ to $\sum_{j=0}^s c_{i,j} [t]_{m}^j$ induce the map $$- \circ \iota_{s, m}: X( C[t]/ (t^{m+1})) \rightarrow X( C[t]/ (t^{s+1}))$$ sending $f$ to $f  \circ \iota_{s, m}$. Since the functor $\underline{J_m(X)}$ is represented by the scheme $J_m (X)$, we have $X( C[t]/ (t^{m+1}))\simeq J_m(X)(C)$ and $X( C[t]/ (t^{s+1}))\simeq J_s(X)(C))$. Considering a covering of $J_m (X)$ by affine, using Yoneda Lemma and gluing, we obtain a canonical projection map $\pi_{m,t}^{X} \colon J_m(X)\rightarrow J_s(X)$. In particular, we obtain a canonical projection $\pi_{m,0}^X\colon J_m (X)\rightarrow X$. 


\end{proof} 

We now define how a $R$-algebra morphism induces a morphism of the corresponding jet $R$-algebra. 

\begin{definition}(Lemma)
Let $\phi\colon C\rightarrow B$ be a morphism of $R-$algebras. We define natural transformations of functors for all $ m\in \mathbb{N}$
$$\begin{array}{cccc}
\underline{J_m(\phi)}(A) : &  \operatorname{Hom}_{ \mathbf{Alg}_R}(B, A[t]/(t^{m+1}) )   &\rightarrow&   \operatorname{Hom}_{ \mathbf{Alg}_R}(C, A[t]/(t^{m+1}) ) \\
& \psi  &\mapsto &  \psi \circ \phi \, ,
\end{array}$$
where $A$ is an $R-$algebra.

If $\varphi: D \rightarrow C$ is another morphism of $R-$algebras, then $\underline{J_m(\varphi)}\circ \underline{J_m(\phi)}= \underline{J_m(\phi\circ \varphi)}$;
let $m,s \in \mathbb{N}$ with $s \leq m$, we have that ${\tau_{m,s}^{(-)}}_\ast\circ \underline{J_s(\phi)}=\underline{J_m(\phi)} \circ {\tau_{m,s}^{(-)}}_\ast$.

This construction induces morphisms of $R-$ algebras
$$ \mathcal{L}_m(\phi)\colon \mathcal{L}_m(C)\rightarrow \mathcal{L}_m(B) $$
defined as $\mathcal{L}_m(\phi):= (\epsilon_{m, \mathcal{L}_m(B)}^C\circ \underline{J_m(\phi)}(\mathcal{L}_m(B))\circ\eta^B_{m, \mathcal{L}_m(B)}) (\mathbf{id}_{\mathcal{L}_m(B)})$.
We can express explicitly this morphism:
Let $B:=R[x_1, \cdots, x_{n_1} ]/I_1$ and $C:= R[y_1, \cdots, y_{n_2}]/I_2$, for every $i \in \{ 1, \cdots, n_2 \}$, we set $[p_i]_{I_1}:= \phi ( [y_i]_{I_2})$. We write 
$p_i( (\sum_{j=1}^m x_{i, j} [t]_m^j)_i) = \sum_{j=0}^s q^m_{i,j} [t]_m^j $,  \\
$\mathcal{L}_m(C)= k[(y_{i,j})_{1\leq i\leq n_2, 1\leq j\leq s}]/\mathcal{L}_m(I_2)$ and $\mathcal{L}_m(B)=k[(x_{u,v})_{1\leq u\leq n_1, 1\leq v\leq s}]/ \mathcal{L}_s(I_1)$. We define the {\sf $m^{th}$ jet algebra morphism associated to $\phi$} denoted $\mathcal{L}_m(\phi)$ to be the $R$-algebra morphism 
$$\begin{array}{cccc}
\mathcal{L}_m(\phi) : & \mathcal{L}_m(C)  &\rightarrow& \mathcal{L}_m(B) \\
& [y_{i,j}]_{\mathcal{L}_m(I_2)}  &\mapsto &[q^m_{i,j}]_{\mathcal{L}_m(I_1)}.
\end{array}$$
%We have $\mathcal{L}_m(\phi)={\epsilon_m^B}_{J_m(C)} ( \rho_{m,0}^{C} \circ \phi)$. 
We have $\mu^B_{m,s} \circ \mathcal{L}_m(\phi)=\mathcal{L}_s(\phi) \circ \mu^C_{m,s}$ and $\mathcal{L}_m (Id_{B}) = Id_{\mathcal{L}_m (B)}$. If $\varphi: D \rightarrow C$, then $\mathcal{L}_m(\phi \circ \varphi) = \mathcal{L}_m (\phi) \circ \mathcal{L}_m ( \varphi)$.
\end{definition} 

\begin{proof} 
Let $\psi\in \operatorname{Hom}_{ \mathbf{Alg}_R}(B, A[t]/(t^{s+1}) )$, we have that
$$
\underline{J_m(\varphi)}(A)(\underline{J_m(\phi)}(A)(\psi))= \underline{J_m(\varphi)}(A)(\psi\circ\phi)=\psi\circ\phi\circ\varphi=\underline{J_m(\phi\circ\varphi)}(A)(\psi) \, .
$$
Moreover,
\begin{align*}
{\tau_{m,s}^{(A)}}_\ast ( \underline{J_s(\phi)}(A) (\psi)) & = {\tau_{m,s}^{(A)}}_\ast (\psi\circ \phi) \\
& = \tau_{m,s}^A\circ \psi \circ \phi  \\
& = \underline{J_m(\phi)}(A) ( \tau_{m,s}^A\circ \psi) \\
& = (\underline{J_m(\phi)}(A) ( {\tau_{m,s}^{(A)}}_\ast (\psi)) \, .
\end{align*}

We compute $\eta^C_{m,\mathcal{L}_m(B)}(\mathcal{L}_m(\phi)) ( y_i )$. 
\begin{align*} \eta^C_{m,\mathcal{L}_m(B)}(\mathcal{L}_m(\phi)) ([y_i]_{I_2}) &=  \eta^B_{m,\mathcal{L}_m(B)}(Id_{\mathcal{L}_m(B)} ) \circ \phi (y_i) \\
& = \eta^B_{m,\mathcal{L}_m(B)}(Id_{\mathcal{L}_m(B)} )([p_i]_{I_1}) \\
& = p_i(\eta^B_{m,\mathcal{L}_m(B)}(Id_{\mathcal{L}_m(B)} )(x_1),\dots, \eta^B_{m,\mathcal{L}_m(B)}(Id_{\mathcal{L}_m(B)} )(x_{n_1}) ) \\
& = p_i(x_{1,0}+\cdots + [t]^m x_{1,m},\dots, x_{n_1,0}+\cdots + [t]^m x_{n_1,m} ) \\
&= [q_{i,0}]_{\mathcal{L}_m(I_1)}+\cdots + [t]^m [q_{i,m}]_{J_m(I_1)} \, .
\end{align*}
It follows from the definition of $\epsilon^C_{m, \mathcal{L}_m(B)}$ that
$$ \mathcal{L}_m(\phi) ([y_{i,j}]_{J_m(I_2)})= [q_{i,j}]_{J_m(I_1)} \, ,$$
which proves that $\mathcal{L}_m(\phi)$ has the abovementioned form.

The rest is just a consequence of the functorial equalities above.


%We compute ${\epsilon_m^C}_{J_m(B)} ( \rho_{m,0}^{C} \circ \phi) (  [y_{i,j}]_{J_m(I_2)})$. Do do this we observe that for every $i \in \{ 1, \cdots , n_2\}$, 
%$$\begin{array}{llll} ( \rho_{m,0}^{C} \circ \phi) ( [y_i]_I) &=&  \sigma_m^{C} ( \phi ([y_i]_I))= \sigma_m^{C} ( p_i )=[p_i ( (\sum_{j=1}^{s} x_{i,j} [t]_m^j)_i)]_{J_s(I)J_s(B)[t]/ (t^{m+1})} \\
%&=& [\sum_{j=0}^s q^m_{i,j} [t]_m^j]_{J_s(I)J_s(B)[t]/ (t^{m+1})}=\sum_{j=0}^s [q^m_{i,j}]_{J_m(I_1)} [t]_m^j .
%\end{array}
%$$
%Therefore, by definition, ${\epsilon_m^C}_{J_m(B)} ( \rho_{m,0}^{C} \circ \phi) (  [y_{i,j}]_{J_m(I_2)}) =[q^m_{i,j}]_{J_m(I_1)}$ as wanted. The last equality follows from the definition of $\mu^C_{m,s}$. 



%Given $X$ and $Y$ be two schemes of finite type over $Spec(R)$. Let $f\colon X\rightarrow Y$ be a morphism of schemes. The natural transformation $- \circ f$ between $\operatorname{Hom}_{ \mathbf{Sch}_k}(-,X)$ and $\operatorname{Hom}_{ \mathbf{Sch}_k}(-,Y)$ induces, a family of maps $$(\underline{{f_m}}_C \colon X(C[t]/(t^{m+1}))\rightarrow Y(C[t]/(t^{m+1})))_{C \in  \mathbf{Alg}_R }$$ which defines a natural transformation $\underline{{f_m}}$ between the functors $\underline{J_m(X)}$ and $\underline{J_m(Y)}$. By Yoneda lemma, $\underline{{f_m}}$ induces a morphism of schemes denoted $J_m(f) \colon J_m(X)\rightarrow J_m(Y)$. These morphisms are compatible with the abovementioned projections, in the sense that whenever $s\leq m$, the equality
%$$ J_s (f) \circ\pi^{X}_{m,s} = \pi^{Y}_{m,s}\circ J_m (f)$$
%holds. Therefore $J_m$ defines an endofunctor of the category of schemes over $R$.
%
%
%%\begin{exmp} 
%We first describe jet morphisms induced by schemes morphisms between $\mathbb{A}^s$ and $\mathbb{A}^n$. To do this it is enough to consider a $R$-algebra morphism between two polynomial rings. Given $B=R[x_1, \cdots, x_n]/I_1$ and $C= R[y_1, \cdots, y_m]/I_2$ be two polynomial rings. 
%Consider a morphism $\phi : C \rightarrow B$ sending $[y_i]_{I_2}$ to $ [p_i]_{I_1}$ in $ R[x_1,\dots, x_n]/I_1$, for every $i \in \{ 1, \cdots, m \}$. We have $h(p_1, \cdots , p_m)\in I_1$, for every $h\in I_2$.  %% Here := should be improved
%For each $1\leq i\leq m$, consider the polynomial
%$$p_i(x_{1,0}+[t]_sx_{1,1}+\cdots +[t]_s^sx_{1,s}, \dots, x_{n,0}+[t]_sx_{1,1}+\cdots +[t]_s^sx_{n,s} )\in  k[(x_{u,v})_{1\leq u\leq n, 0\leq v \leq s}][t]/(t^{s+1}) \, , $$ 
%which can be written as 
%$$ \sum_{j=0}^s q_{i,j}((x_{u,v})_{u,v}) [t]_s^j \, , $$
%where each $q_{i,j}\in k[(x_{u,v})_{1\leq u\leq n, 0\leq v \leq n}]$.
%%Let us show that the map of algebras
%We define $J_s(\phi)$ the morphism 
%$$\begin{array}{cccc}
%J_s(\phi) : & k[(y_{i,j})_{1\leq i\leq m, 1\leq j\leq s}]/J_s(I_2)  &\rightarrow& k[(x_{u,v})_{1\leq u\leq n, 1\leq v\leq s}]/ J_s(I_1) \\
%& [y_{i,j}]_{J_s(I_2)}  &\mapsto &[q_{i,j}]_{J_s(I_2)}.
%\end{array}$$
%We prove that this map is a well-defined morphism of $R$-algebra 
%inducing the canonical map of jet schemes $J_s(f) \colon J_s(X)\rightarrow J_s(Y)$ associated to $$f : Spec (R[x_1,\dots, x_n]/I_1) \rightarrow Spec ( R[y_1, \cdots, y_m]/I_2)$$ where $f= Spec(\phi)$.
%We prove that the map is well defined, that is $l( (q_{i,j})_{i,j} ) \in J_s(I_1) $, for all $l\in J_s(I_2)$. Let $i \in \{ 1, \cdots, m \}$, we set $\overline{q_{i,j}}:=q_{i,j}((x_{u,v})_{u,v})$ and $\overline{p_i}:= p_i(x_{1,0}+[t]_sx_{1,1}+\cdots +[t]_s^sx_{1,s}, \dots, x_{n,0}+[t]_sx_{1,1}+\cdots +[t]_s^sx_{n,s} )= \sum_{j=0}^s q_{i,j}((x_{u,v})_{u,v}) [t]_s^j $. Let $h \in I_2$, we have $h(p_1, \cdots , p_m)\in I_1$
%$$h ( \overline{p_1}, \cdots , \overline{p_m})= h\left( \sum_{j=0}^s \overline{q_{1,j}} [t]_s^j, \cdots ,  \sum_{j=0}^s \overline{q_{m,j}} [t]_s^j \right) = \sum_{j=1}^m g_{h, j}( (\overline{q_{i,j}})_{i,j}) [t]_{m}^j . $$ So that $g_{h, j}( (q_{i,j})_{i,j}) \in J_s( I_1)$. 
%Moreover, the morphism $\phi$ induces, at the level of $C$-valued points, a map of sets 
%$$- \circ \phi : \operatorname{Hom}_R(R[x_1,\dots,x_n]/I_1, C[t]/(t^{s+1}))\rightarrow \operatorname{Hom}_R(R[y_1,\dots,y_m]/I_2, C[t]/(t^{s+1}))$$
%that sends $\psi$ to $\psi\circ \phi $. Let $\psi([x_u]_{I_1})=a_{u,0}+[t]_s a_{u,1}+\cdots+ [t]_s^s a_{u,s}$ for $1\leq u\leq n$ and for $a_{u,v}\in A$; then
%\begin{align*}
%\psi\circ \phi ([y_i]_{I_2}) &=\psi([p_i]_{I_1})  =p_i(a_{1,0}+\cdots+ [t]_s^s a_{1,s},\dots, a_{n,0}+\cdots+ [t]_s^s a_{n,s}) \\
%&=\sum_{j=0}^s q_{i,j}((a_{u,v})_{u,v}) [t]_s^j \, .
%\end{align*}
%This proves the above. 
\end{proof}
We can now define the Jet algebra functor 
\begin{definition} Let $m,s \in\mathbb{N}$ such that $s\leq m$.
We define the {\sf $m^{th}$ Jet algebra functor} denoted $ \underline{J_m}_{\mathbf{Alg}}$ (or simply $ \underline{J_m}$ when no confusion can be made)  to be the functor 
$$ \begin{array}{llll} \underline{J_m}_{\mathbf{Alg}} : &  \mathbf{Alg}_R & \rightarrow  &\mathbf{Alg}_R\\
&B & \mapsto & \mathcal{L}_m (B) \\
&\phi & \mapsto & \mathcal{L}_m (\phi) 
\end{array}$$
\end{definition}





We now give a construction of a jet $R$-algebra associated with an algebra that is not necessarily of finite type. To do this we need the following Lemma permitting to obtain the direct limit of a natural transformation. 

\begin{lemma}%[Abstract nonsense longer than the proof we need it for]
\label{lem:absnonsense}
Let $\mathcal{F}, \mathcal{F}_i \colon \mathcal{C} \rightarrow \mathcal{D}$, for $i\in I$, with $I$ poset, be functors between two categories.
%from a category $\mathcal{C}$ to a category $\mathcal{D}$ admitting limits.
Assume that, $\forall j \leq i \in I$, there are natural transformations $\eta^i_j\colon \mathcal{F}_i \rightarrow \mathcal{F}_j$ and $\eta_i\colon \mathcal{F}\rightarrow \mathcal{F}_i$ such that $\forall k\leq j\leq i\in I$, $\eta_{k}^i= \eta^j_k\circ \eta^i_j$ and $\eta_j= \eta^i_j \circ \eta_i$. Assume furtherly that $\forall c\in \mathcal{C}$, then $\eta_i(\mathbf{id}_c) \colon \mathcal{F}(c) \rightarrow \mathcal{F}_i(c)$ is the limit of the system $\eta^i_j(\mathbf{id}_c)\colon \mathcal{F}_i(c)\rightarrow \mathcal{F}_j(c)$. Then $\eta_i \colon \mathcal{F} \rightarrow \mathcal{F}_i$ is the limit of the system $\eta^i_j\colon \mathcal{F}_i\rightarrow \mathcal{F}_j$ in the category $\operatorname{Mor}(\mathcal{C}, \mathcal{D})$.
\end{lemma}
\begin{proof}
Let $\mathcal{G}\colon \mathcal{C}\rightarrow \mathcal{D}$ be a functor and let $\epsilon_i\colon \mathcal{G}\rightarrow \mathcal{F}_i$ be natural transformations such that, $\forall j\leq i\in I$, $\epsilon_j = \eta^i_j\circ\epsilon_i$. We need to show that $\exists! \epsilon\colon \mathcal{G}\rightarrow \mathcal{F}$ such that $\forall i\in I$, $\epsilon_i= \eta_i\circ \epsilon$.
Let us define $\epsilon$ as follows:
Given an object $c\in \mathcal{C}$, let $\epsilon(c)\colon \mathcal{G}(c)\rightarrow \mathcal{F}(c)$ be the unique morphism such that $\forall i\in I$, $\epsilon_i(c)=\eta_i(c)\circ\epsilon(c)$.
Now, given a morphims $f\colon c_1\rightarrow c_2$ in $\mathcal{C}$, consider the following diagram:
$$
\begin{tikzpicture}{scale=1.4}
\node (1) at (-2.5,1) {$\mathcal{G}(c_1)$};
\node (2) at (0,1) {$\mathcal{F}(c_1)$};
\node (3) at (2.5,1) {$\mathcal{F}_i(c_1)$};
\node (4) at (-2.5,-1) {$\mathcal{G}(c_2)$};
\node (5) at (0,-1) {$\mathcal{F}(c_2)$};
\node (6) at (2.5,-1) {$\mathcal{F}_i(c_2)$};
\draw [->] (1) -- (2) node[pos=.5, above]{$\epsilon(c_1)$};
\draw [->] (1) -- (4) node[pos=.5, left]{$\mathcal{G}(f)$};
\draw [->] (2) -- (3) node[pos=.5, above]{$\eta_i(c_1)$};
\draw [->] (2) -- (5) node[pos=.5, right]{$\mathcal{F}(f)$};
\draw [->] (4) -- (5) node[pos=.5, below]{$\epsilon(c_2)$};
\draw [->] (5) -- (6) node[pos=.5, below]{$\eta_i(c_2)$};
\draw [->] (3) -- (6) node[pos=.5, right]{$\mathcal{F}_i(f)$};
\end{tikzpicture} \, .
$$
Since $\epsilon_i=\eta_i\circ\epsilon$ and $\eta_i$ are natural transformations, we have that the big rectangle and the right square are commutative. Therefore whe have, $\forall i\in I$
$$ \eta_i(c_2)\circ\epsilon(c_2)\circ \mathcal{G}(f) = \mathcal{F}_i(f)\circ \eta_i(c_1)\circ\epsilon(c_1) =  \eta_i(c_2)\circ \mathcal{F}(f)\circ\epsilon(c_2) \, , $$
which implies, due to the universal proprty of the limit, that
$$ \epsilon(c_2)\circ \mathcal{G}(f) = \mathcal{F}(f)\circ\epsilon(c_2) \, ,  $$
hence that $\epsilon$ is a natural transformtation.
Now let $\varepsilon\colon \mathcal{G}\rightarrow \mathcal{F}$ a natural transformation such that $\forall i\in I$, $\epsilon_i= \eta_i\circ \varepsilon$. Then for any $c\in C$, we have that $\eta_i(c)\circ\varepsilon(c)=\eta_i(c)\circ\epsilon(c)$, therefore $\varepsilon(c)=\epsilon(c)$ because $\mathcal{F}(c)=\varprojlim \mathcal{F}_i(c)$, thus $\varepsilon=\epsilon$.
\end{proof}


\begin{lemma}
The Jet algebra functor is representable for any $R$-algebra.  
\end{lemma}
\begin{proof}
 Let $B$ be a $R$-algebra. By \cite[Lemma 10.127.2.]{stack}, there exists a directed system $B_\lambda$, $\lambda \in \Lambda$, of R-algebras of finite presentation such that $B=\varinjlim B_{\lambda}$.  We set $\pi_\lambda : B_\lambda \rightarrow B$ to be the canonical maps associated with the direct limit. We have that $\mathcal{L}_m(B_\lambda )$ forms also a directed system since $\underline{J_m}$ is a functor. We now prove that $\underline{J_m(B)}$ is represented by $D_m := \varinjlim \mathcal{L}_m(B_\lambda )$ %. The canonical maps associated with the direct limit are 
with canonical maps $\Pi^m_\lambda:\mathcal{L}_m (B_\lambda)  \rightarrow D_m $.  In order to prove this we need to prove that there is a natural correspondence between $ \underline{D_m}$ and $\underline{J_m(B)}$. 
%\luigi{I'll start from here.}
By Lemma \ref{lem:absnonsense}, $\underline{J_m(B)}=\varprojlim \underline{J_m(B_\lambda)}$ with natural transformations $\underline{J_m(\pi_\lambda)}$ and, similarly, $\underline{D_m}=\varprojlim \underline{L_m(B_\lambda)}$ with natural transformations ${\Pi^m_{\pi_\lambda}}^\ast$. By the universal property of the limits, there is a unique natural transformation $\epsilon^B_m\colon \underline{J_m(B)}\rightarrow \underline{D_m}$ such that 
$$ \forall \lambda \in \Lambda \quad  {\Pi^m_\lambda}^\ast\circ \epsilon^B_m =  \epsilon^{B_\lambda}_m \circ \underline{J_m(\pi_\lambda)} $$
and a unique natural transformation $\eta^B_m\colon \underline{D_m}\rightarrow \underline{J_m(B)}$ such that 
$$ \forall \lambda \in \Lambda \quad  \underline{J_m(\pi_\lambda)}\circ \eta^B_m =  \epsilon^{B_\lambda}_m \circ {\Pi^m_\lambda}^\ast \, .$$
Moreover $\eta^B_m \circ \epsilon^B_m = \mathbf{id}_{\underline{J_m(B)}}$ and $\epsilon^B_m\circ\eta^B_m= \mathbf{id}_{\underline{D_m}}$.
%
%\luigi{Stopped here}
%
%That is there exists a natural transformation  $\epsilon_m^{B}=( {\epsilon_m^{B}}_C : \underline{J_m(B)} (C) \rightarrow \underline{D_m}(C))_{C \in \mathbf{Alg}_R }$ and there exists a natural transformation  $\eta_m^{B}=( {\eta_m^{B}}_C : \underline{D_m} (C) \rightarrow \underline{J_m (B)}(C))_{C \in \mathbf{Alg}_R }$ such that $\epsilon_m^{B}$ and $\eta_m^{B}$ are inverse of each other. Let $C$ be a $R$-algebra and $\phi: B \rightarrow C[t]/(t^{m+1})$. For each $\lambda$, we have $\phi_\lambda : B_\lambda \rightarrow C[t]/(t^{m+1})$ defined by $\phi_\lambda:= \phi \circ \pi_\lambda$.
%We start by defining $\epsilon_m^{B}$. 
% For each $\lambda$, since $B_\lambda$ is a $R$-algebra of finite presentation, we have defined in Definition (Lemma) \ref{defft} a natural transformation $\epsilon_m^{B_\lambda}$. %$ \epsilon_m^{B_\lambda} : \underline{J_m(B_\lambda)} (C) \rightarrow \underline{\mathcal{L}_m (B_\lambda)}(B)$.  
% We define ${\epsilon_m^{B}}_C ( \phi)$ to be the only map such that for all $\lambda$, ${\epsilon_m^{B_\lambda}}_C ( \phi_\lambda )= {\epsilon_m^{B}}_C ( \phi) \circ J_m (\pi_\lambda)$. 
% Again, for each $\lambda$, since $B_\lambda$ is a $R$-algebra of finite presentation, we have defined in Definition (Lemma) \ref{defft} a natural transformation ${\eta_m}_C^{B_\lambda}$. We define ${\eta_m}_C^{B} ( \phi)$ to be the only map such that for all $\lambda$, ${\eta_m}_C^{B_\lambda} ( \phi_\lambda )= {\eta_m}_C^{B} ( \phi) \circ \Pi^m_\lambda$. 
% We need to prove that ${\epsilon_m}_C^{B}$ and ${\eta_m}_C^B$ are natural transformations inverse of each other. \sophie{stopped here} 
% %Let $\phi: B \rightarrow C[t]/(t^{m+1})$.  Since $B_\lambda$ is a $R$-algebra of finite presentation, there is $


\end{proof} 


We denote $N_s(\mathfrak{p}):= B_\mathfrak{p} / \mathfrak{p}^s B_\mathfrak{p} $ and $\zeta_{\mathfrak{p}, s} : B \rightarrow N_s(\mathfrak{p})$ be the canonical map.  
We now describe the fiber of the jet at a prime ideal


\begin{definition}(Lemma) \label{Nsp}
Let $B$ be a $R$-algebra and $\mathfrak{p}$ be a prime ideal of $B$. 
\begin{enumerate}
\item We define the fiber of $\underline{J_1(B)}$ at $N_s(\mathfrak{p}) $ to be the subfunctor of $\underline{J_1(B)}$ denoted $\underline{J_1(B)}_{N_s(\mathfrak{p})}$ defined as the fiber product $\underline{J_1(B)} \times_{\underline{B}}  \underline{N_s(\mathfrak{p})}$. That is, we have natural isomorphisms, for any $N_s(\mathfrak{p})$-algebra $C$ whose structural map is given by $\eta : N_s(\mathfrak{p}) \rightarrow C$ 
$$\begin{array}{lll} \underline{J_1(B)}_{N_s(\mathfrak{p})}(C)&\simeq&   \{\psi \in \operatorname{Hom}_k(B, C[t]/(t^{2}))  \colon  \tau_{0,s}^B \circ \psi= \eta \circ \zeta_{\mathfrak{p},s}  \}    \simeq Der_{k} ( N_{s+1}(\mathfrak{p}) , C) \,  \\
%&\simeq & \{\psi \in \operatorname{Hom}_k(B, C[t]/(t^{2}))  \colon \mathfrak{p}= \psi^{-1}(\overline{t} C[t]/(t^{2})) \text{ and } p_1^B ( \psi (B \backslash \mathfrak{p}) ) \subseteq C^\times \} \, 
 \end{array}$$
and for all $\phi :  C \rightarrow D$ is a morphism of $N_s(\mathfrak{p})$-algebra 
$$ \text{ $\underline{J_s(B)}_{N_s(\mathfrak{p})}(\phi)$}=\widetilde{\phi}_* \times \phi_*.$$ Moreover, this functor is representable by the $k$-algebra $\mathcal{L}_1(B)\otimes_B$ $N_s(\mathfrak{p})$.
%Given $s, t \in \mathbb{N}$ where $s \geq t$, we denote ${\mu^B_{,t}}_{k(\mathfrak{p}^s)}:\mathcal{L}_1(B)\otimes_B k(\mathfrak{p}^s) \rightarrow \mathcal{L}_1(B)\otimes_B k(\mathfrak{p}^s)$ the canonical morphism induced by $\mu^B_{s,t}$.
\item  We define the reduced fiber of $\underline{J_1(B)}$ at $\mathfrak{p}$ to be the subfunctor of $\underline{J_1(B)}$ denoted $\underline{J_1(B)}_{N_s(\mathfrak{p}), \operatorname{red}}$ defined as $\underline{({\mathcal{L}_1(B)\otimes_B N_s(\mathfrak{p})})_{red}}$. We have that $\pi_{red}^*$ is a natural correspondence from $\underline{J_1(B)}_{\mathfrak{p}, \operatorname{red}}|_{\mathbf{RedAlg}_R}$ to $\underline{J_1(B)}_{N_s(\mathfrak{p})}|_{\mathbf{RedAlg}_R} $ where $\pi_{red} : \mathcal{L}_1(B)\otimes_B N_s(\mathfrak{p}) \rightarrow (\mathcal{L}_1(B)\otimes_B N_s(\mathfrak{p}))_{\operatorname{red}} $ 
\end{enumerate} 
\end{definition}


\begin{proof}
\begin{enumerate}
\item We set $$\mathscr{M}_s :=\{\psi \in \operatorname{Hom}_k(B, C[t]/(t^{2}))  \colon  \tau_{0,s}^B \circ \psi= \eta \circ \zeta_{\mathfrak{p},s}  \} .$$ It is not hard to  prove that the family of maps $(\Phi_C)_{C \in \mathbf{Alg}_{ N_s(\mathfrak{p})}}$ where 
$$\begin{array}{lrrl}\Phi_C  : & \underline{J_1(B)}(C) \times_{\underline{B}(C)}  \underline{N_s(\mathfrak{p})}(C)&\mapsto & \mathscr{M}_s \, \\ 
& (\phi, f) & \mapsto & {\eta^B_m}_C  (\phi)
 \end{array}$$
 is a natural correspondence, since $f = \eta$. 
Now we define $$\begin{array}{lrrl}\Psi_C  : & \mathscr{M}_s &\mapsto &Der_{k} ( N_{s+1} (\mathfrak{p}) , C)  \, \\ 
& \psi & \mapsto &\Psi_C (\psi)
 \end{array}$$
 where $\Psi_C (\psi)\in Der_{k} ( N_{s+1} (\mathfrak{p}) , C)$ induced by $\psi$ as follows. 
 %Since $\psi :B\rightarrow C[t]/(t^{2}) $ is such that $\tau_{0,s}^B \circ \psi= \eta \circ \zeta_{\mathfrak{p}}$.  %We have  $\psi ( B \backslash \mathfrak{p}) \subseteq C[t]/(t^{2})^\times$. Indeed,  $\mathfrak{p}= \psi^{-1}(\overline{t} C[t]/(t^{s+1}))$ and $p_s^B ( \psi (B \backslash \mathfrak{p}) ) \subseteq C^\times$. To see this we observe that by assumption, we have $\tau_{0,s}^B ( \psi  ( \mathfrak{p}))  = \eta ( \zeta_\mathfrak{p} ( \mathfrak{p}))=0$.  So that, $ker (\tau_{0,s}^B\circ  \psi ) = \mathfrak{p}$, since $\eta$ is one-to-one map as a non-trivial map from a field. That is equivalent to  $\mathfrak{p}= \psi^{-1}(\overline{t} C[t]/(t^{s+1}))$. Thus $\psi ( \mathfrak{p}) = \psi ( \psi^{-1}(\overline{t} C[t]/(t^{s+1}))) \subseteq \overline{t} C[t]/(t^{s+1})$. So that $\psi (B \backslash \mathfrak{p})  \subseteq  C[t]/(t^{s+1}) \backslash \overline{t} C[t]/(t^{s+1})$. 
 
 %$(a+[t] b)(c+ [t] d) = ac + [t] (bc+ ad) =1$. thus $ac=1$ and $bc+ad =0$. 
There are $\psi_0 \in \operatorname{Hom}_k(B , C)$ and $\psi_1 \in \operatorname{Der}_k(B , C)$ such that $\psi (b)= \psi_0(b) + [t] \psi_1 (b)$, for all $b \in B$. Let $\psi_0$ and $\psi_1$ such maps. 
  
 Let $b \in B \backslash \mathfrak{p}$. We want to prove that $\psi(b) \in C[t]/(t^{2})^\times$. 
 Since  $\tau_{0,s}^B \circ \psi= \eta \circ \zeta_{\mathfrak{p},s}$, we have $\psi_0 = \eta \circ \zeta_{\mathfrak{p},s}$. 
 So if $b \in B \backslash \mathfrak{p}$. Then $\psi_0(b) \in C^\times$. Let $c$ be the multiplicative inverse of $\psi_0(b)$. We prove that $c-[t] \psi_1 (b) c^2$ is the inverse of $\psi(b) $. Indeed, $\psi(b)( c-[t] bc^2)  =( \psi_0(b) + [t] \psi_1 (b)) (c-[t] \psi_1 (b) c^2) = 1 +[t] (\psi_1 (b)c - \psi_0(b)\psi_1 (b) c^2 ) = 1$. 
 
This proves that $\psi$ induces a canonical localization map $\overline{\psi}: B_\mathfrak{p} \rightarrow C[t]/(t^2)$.  
There are $\overline{\psi_0} \in \operatorname{Hom}_k(B_\mathfrak{p} , C)$ and $\overline{\psi_1} \in \operatorname{Der}_k(B_\mathfrak{p}  , C)$ such that $\overline{\psi} (b)= \overline{\psi_0}(b) + [t]\overline{ \psi_1 }(b)$, for all $b \in B$. Let $\overline{\psi_0}$ and $\overline{\psi_1}$ such maps

Now, prove that $\mathfrak{p}^{s+1} B_\mathfrak{p} \subseteq ker(\overline{\psi})$.  Since $\mathfrak{p} B_\mathfrak{p}  \subseteq ker(\overline{\psi_0})$, it is enough to prove that $\mathfrak{p}^{s+1} B_\mathfrak{p}   \subseteq ker(\overline{\psi_1})$. The former is a direct consequence from the fact that $\overline{\psi_1}\in \operatorname{Der}_k(B_\mathfrak{p}  , C)$. %Let $b\in \mathfrak{p}^{s+1}B_\mathfrak{p} $. There are $I$ finite set, $a_i  \in\mathfrak{p}B_\mathfrak{p} $ and $c_i  \in\mathfrak{p}B_\mathfrak{p} $  such that $b= \sum_{i \in I } a_i c_i$. Since $\overline{\psi_1}\in \operatorname{Der}_k(B_\mathfrak{p}  , C)$, we have $\overline{\psi_1}(b) = \overline{\psi_1} ( \sum_{i \in I } a_i c_i) = \sum_{i \in I } ( \overline{\psi_1}(a_i)\overline{\psi_0}(c_i) + \overline{\psi_0}(a_i)\overline{\psi_1}(c_i))=0$.  

Therefore, by the first isomorphism theorem, $\overline{\psi}$ induces a $k$-algebra $\widetilde{\psi}$ from $N_{s+1}(\mathfrak{p})$ to $C[t]/(t^2)$. Thus again, there are $\widetilde{\psi_0} \in \operatorname{Hom}_k(B_\mathfrak{p} , C)$ and $\widetilde{\psi_1} \in \operatorname{Der}_k(B_\mathfrak{p}  , C)$ such that $\widetilde{\psi} (b)= \widetilde{\psi_0}(b) + [t]\widetilde{ \psi_1 }(b)$, for all $b \in B$. Let $\widetilde{\psi_0}$ and $\widetilde{\psi_1}$ such maps. We set $\Psi_C (\psi):=\widetilde{\psi_1}$. 

We defined the map 
$$\begin{array}{lrrl}\Phi_C  : & Der_{k} ( N_s(\mathfrak{p})  , C) &\mapsto &\mathscr{M}_s  \, \\ 
& \psi & \mapsto &  \eta \circ \zeta_\mathfrak{p} + [t] \psi\circ \zeta_{\mathfrak{p},s}
 \end{array}$$
 It is not hard to see that $\Phi_C$ is the inverse of $\Psi_C$. 
 
 %Moreover since $ \eta$ is a $k$-algebra morphism from the field  $k(\mathfrak{p})$ to $C$ we know that every non zero element of $k(\mathfrak{p})$ is sent to an invertible element of $C$. Therefore, any elements not in $\mathfrak{p}$ is sent to an invertible element of $C$ via $\eta \circ \zeta_\mathfrak{p}$. $Thus, p_s^B ( \psi (B \backslash \mathfrak{p}) ) \subseteq C^\times$.

 
%$$\begin{array}{lll} && Hom_{k ( \mathfrak{p})} ( \mathcal{L}_1 (B) \otimes_B k ( \mathfrak{p}) , C ) \\
%&\simeq&  \{\psi \in \operatorname{Hom}_k(B, C[t]/(t^{2}))  \colon  p_1^B \circ \psi= f \circ \zeta_{\mathfrak{p}}  \} \\
%%p_s^B ( \psi (B \backslash \mathfrak{p}) ) \subseteq C^\times
%&\simeq &\{  \psi\in \operatorname{Hom}_k(B_\mathfrak{p}, C[t]/(t^{2})): \psi ( b) = \psi_0 (b) + [t] \psi_1(b), \  \psi_0 = f \circ \pi_\mathfrak{p} \}\\
%&\simeq& \{ \widetilde{\psi} \in \operatorname{Hom}_k(B_\mathfrak{p}/ \mathfrak{p}^2 , C[t]/(t^{2})):   \widetilde{\psi} ( b) = \widetilde{\psi}_0 (b) + [t]  \widetilde{\psi}_1(b), \   \widetilde{\psi}_0 = f \circ \pi_{2, \mathfrak{p}}  \}\\
%&\simeq& Der_{k} ( B_\mathfrak{p}/ \mathfrak{p}^2  , C)  
%\end{array}
% $$
%\item Given a $k$-algebra $C$ and $\phi :  C \rightarrow D$ a morphism of $k$-algebra, we consider the functor $\underline{J_s(B)}_\mathfrak{p}$. We set $$\mathscr{M} := \{\psi \in \operatorname{Hom}_k(B, C[t]/(t^{s+1}))  \colon \mathfrak{p}= \psi^{-1}(\overline{t} C[t]/(t^{s+1})) \text{ and } p_s^B ( \psi (B \backslash \mathfrak{p}) ) \subseteq C^\times \} .$$ We want to prove it is a representable functor represented by $\mathcal{L}_s(B)\otimes_B$ $k(\mathfrak{p})$. That is, we need to prove that the map 
%$$\begin{array}{lrrl}\Phi_C  : & \underline{J_s(B)}(C) \times_{\underline{B}(C)}  \underline{k(\mathfrak{p})}(C)&\mapsto & \mathscr{M} \, \\ 
%& (\psi, \eta) & \mapsto & \psi
% \end{array}$$
%Let $(\psi, \eta)  \in \underline{J_s(B)} \times_{\underline{B}}  \underline{k(\mathfrak{p})}(C)$. That is, $\tau_{0,s}^B \circ \psi   =  \eta \circ \zeta_\mathfrak{p} .$ We have $\tau_{0,s}^B ( \psi  ( \mathfrak{p}))  = \eta ( \zeta_\mathfrak{p} ( \mathfrak{p}))=0$.  So that, $ker (\tau_{0,s}^B\circ  \psi ) = \mathfrak{p}$, since $\eta$ is one-to-one map as a non-trivial map from a field. That is equivalent to  $\mathfrak{p}= \psi^{-1}(\overline{t} C[t]/(t^{s+1}))$ moreover since $ \eta$ is a $k$-algebra morphism from the field  $k(\mathfrak{p})$ to $C$ we know that every non zero element of $k(\mathfrak{p})$ is sent to an invertible element of $C$. Therefore, any elements not in $\mathfrak{p}$ is sent to an invertible element of $C$ via $\eta \circ \zeta_\mathfrak{p}$. 
%
%Now, let $\psi  \in \operatorname{Hom}_k(B, C[t]/(t^{s+1}))$ such that $\mathfrak{p}= \psi^{-1}(\overline{t} C[t]/(t^{s+1}))$ and $p_s^B ( \psi (B \backslash \mathfrak{p}) ) \subseteq C^\times$. The universal property of the localization and the universal property of the quotient guarantee us the existence of only morphism $\eta \in \operatorname{Hom}_k(k(\mathfrak{p}), C)$ such that $\tau_{0,s}^B \circ \psi   =  \eta \circ \zeta_\mathfrak{p} .$ This gives us the injectivity and the surjectivity of $\Phi$.
%
%The fact that $\mathcal{L}_s(B)\otimes_B$ $k(\mathfrak{p})$ represents $\underline{J_s(B)}_\mathfrak{p}$ can be deduced from the universal property of the tensor product, the fact that $\mathcal{L}_s(B)$ represents $\underline{J_s(B)}$ via $\eta_m^B$ and $\epsilon_m^B$ and that $\tau_{0,s}^C \circ \psi= {\epsilon_m}_C^B (\psi) \circ \mu_{0,s}^B$ (see Definition \ref{defft} (1) and (2)). 
\item We prove that the natural transformation 
$$\pi_{\operatorname{red}}^*: Hom_{R} ( (\mathcal{L}_1(B)\otimes_B N_s(\mathfrak{p}))_{\operatorname{red}} , -)\rightarrow Hom_{R} ( \mathcal{L}_1(B)\otimes_B N_s(\mathfrak{p}) , -) $$
is a natural correspondence. That is, for any $C$ reduced $R$-algebra, 
 $${\pi_{\operatorname{red}}}^*_C: \operatorname{Hom}_{R} ( (\mathcal{L}_1(B)\otimes_B N_s(\mathfrak{p}))_{\operatorname{red}} , C) \rightarrow \operatorname{Hom}_{R} ( \mathcal{L}_1(B)\otimes_B N_s(\mathfrak{p}) , C)$$
 is a bijection. The injectivity follows from the fact that $\pi_{Nil}$ is surjective. For the surjectivity, let $\phi \in \operatorname{Hom}_{R} ( \mathcal{L}_1(B)\otimes_B N_s(\mathfrak{p}) , C)$.  There is a $\tilde{\phi} \in \operatorname{Hom}_{R} ( (\mathcal{L}_1(B)\otimes_B N_s(\mathfrak{p}))_{\operatorname{red}} , C)$ such that $\tilde{\phi} \circ \pi_{\operatorname{red}}= \phi$ if $ \operatorname{Nil} ( \mathcal{L}_1(B)\otimes_B N_s(\mathfrak{p}))  \subseteq\operatorname{ker} (\operatorname{\phi})$. Let $b \in  \operatorname{Nil} ( \mathcal{L}_1(B)\otimes_B N_s(\mathfrak{p}))  $. We have then there is $n \in \mathbb{N}^*$ such that $b ^n =0$. Thus, $\phi(b)^n = \phi (b^n ) = \phi (0)=0 $. Since $C$ is reduced, we have $\phi(b)=0$. Therefore, we obtain the result. 
\end{enumerate} 

%$p_s^B \circ \psi   =  \eta \circ \zeta_\mathfrak{p} .$ Since $ker (p_s^B) = \overline{t} C[t]/(t^{s+1})$ and $\mathfrak{p} = ker (\zeta_\mathfrak{p} )$. 

%We have $p_s^B ( \psi  ( \mathfrak{p}))  = \eta ( \zeta_\mathfrak{p} ( \mathfrak{p}))=0$.

%We have $ \underline{J_s(B)} \times_{\underline{B}}  \underline{k(\mathfrak{p})} = $. 
%$$ \underline{J_s(B)}_\mathfrak{p} \simeq  \underline{\text{ $\mathcal{L}_s(B)$}\otimes_B k(\mathfrak{p}) }.$$
%Let $\phi \in \underline{\text{ $\mathcal{L}_s(B)$}\otimes_B k(\mathfrak{p}) } (C) = \operatorname{Hom}_k (\text{$\mathcal{L}_s(B)$}\otimes_B k(\mathfrak{p}), C)$. We consider the canonical map $\iota: B \rightarrow  \text{ $\mathcal{L}_s(B)$}\otimes_B k(\mathfrak{p})  $ sending $b$ to $\mu_{s,0}^B (b) \otimes 1$. We define $\psi = \iota_s^B \circ \phi \circ \iota$. 
%
%
%\sophie{ I am not sure of the proof}  
%By definition, $\mathcal{L}_s(B)\otimes_B$ $k(\mathfrak{p})$ corepresents the functor $\underline{J_s(B)} \times_{\underline{B}} \underline{k(\mathfrak{p})}$
%%$$  \operatorname{Hom}_k(k(p), -) \times_{\operatorname{Hom}_k(B, -)} \operatorname{Hom}_k(B, (-)[t]/(t^{s+1}) \, , $$
%which is the subfunctor of $\underline{J_s(B)}$ that we denote $\underline{J_s(B)}_\mathfrak{p}$. It is defined by for any $C$ $k$-algebra, 
%$$\begin{array}{lll} \underline{J_s(B)}_\mathfrak{p}(C)&=& \{\psi\in \operatorname{Hom}_k(B, C[t]/(t^{s+1})) \colon  \psi \circ \mu_{s, 0}^B = \psi \circ \zeta_\mathfrak{p} \} \\
%&=& \{\psi\in \operatorname{Hom}_k(B, C[t]/(t^{s+1})) \colon \psi(\mathfrak{p})\subseteq \overline{t} C[t]/(t^{s+1}) \} \, . \end{array}$$
%Indeed, let $\psi\in \operatorname{Hom}_k(B, C[t]/(t^{s+1}))$ such that $\psi \circ \mu_{s, 0}^B = \psi \circ \zeta_\mathfrak{p}$. 
%%We have $\operatorname{ker}( \psi \circ \mu_{s, 0}^B) = \operatorname{ker}(\psi \circ \zeta_\mathfrak{p})$. 
%In particular, 
\end{proof}

\luigi{It might be useful the following definition, it should be meant to be a "thickening" of the fibre of $J_s$, except that it is simpler to define it without localising by P. Also, I need to think of a better name for the functor.}

\begin{definition}[Lemma]
Let $\mathfrak{p}\subseteq B$ be a prime and $m\in \N$.
The functor $\underline{J_s(B)}\times_{\underline{B}} \underline{B/\mathfrak{p}^m}$, which is corepresented by $\mathcal{L}_s(B)\otimes_B B/\mathfrak{p}^m$, embeds in $\underline{J_s(B)}$ as a subfunctor $\underline{J_s(B)}_{B/\mathfrak{p}^m}$ defined by the following:
$$ \underline{J_s(B)}_{B/\mathfrak{p}^m}(C)= \{\psi\in \underline{J_s(B)}(C) \colon p^B_s\circ\psi(\mathfrak{p}^m)=0 \}   \, .$$
\end{definition}

\begin{proof}
By definition, for any $R-$algebra $C$, we have
$$ \underline{J_s(B)}\times_{\underline{B}} \underline{B/\mathfrak{p}^m}(C) =\{(\psi, \phi)\in \Hom_R(B, C[t]/(t^s))\times \Hom_R(B/\mathfrak{p}^s, C)\colon \tau^C_{s,0,\ast}(\psi)= \pi_m^{\ast}(\phi) \}  \, ,$$
where $\pi_m\colon B\rightarrow B/\mathfrak{p}^m$ is the usual reduction modulo $\mathfrak{p}^m$.

We want to show that the forgetful map
\begin{align*}
\underline{J_s(B)}\times_{\underline{B}} \underline{B/\mathfrak{p}^m}(C) & \rightarrow \underline{J_s(B)}(C) \\
(\psi, \phi) & \mapsto \psi 
\end{align*}
is injective and its image contain $\psi\in \Hom_R(B, C[t]/(t^s))$ if and only if $\psi(\mathfrak{p}^m)\subseteq (t)$.

If $(\psi, \phi), (\psi, \varphi)\in \underline{J_s(B)}\times_{\underline{B}} \underline{B/\mathfrak{p}^m}(C)$, then $\pi_m^{\ast}(\phi)=\pi_m^{\ast}(\varphi)$, hence $\phi=\varphi$ due to the injectivity of $\pi_m^\ast$. Thus the forgetful map is injective.

Now let us describe the image of that map; one one hand, for $(\psi, \phi)\in \underline{J_s(B)}\times_{\underline{B}} \underline{B/\mathfrak{p}^m}(C)$, we have that $$\tau^C_{s,0,\ast}(\psi)(\mathfrak{p}^m)=\pi_m^\ast(\phi)(\mathfrak{p}^m)=\phi(\pi_m(\mathfrak{p}^m))=\phi(0)=0 \, . $$
On the other hand, if $\psi\in \underline{J_s(B)}(C)$ has the property that $\psi(\mathfrak{p}^m)\subseteq (t)$, then $\mathfrak{p}^m\subseteq \ker \tau_{m,0,\ast}^C(\psi)$, thus there is a map $\phi\colon B/\mathfrak{p}^m\rightarrow C$ such that $\phi\circ\pi_m=\tau_{m,0,\ast}^C(\psi)$, showing that such a $\psi$ belongs to the image of the forgetful map.
\end{proof}



\begin{lemma} 
Let $B = k[\underline{x}]$ and $I$ ideal of $B$. We set $I_s:= \mu_{0,s}^B( I)$. We have 
$$ \mathcal{L}_1( B) \simeq^\varphi { B[ (\underline{x}_i)_{1\leq i\leq s}]}$$ 
$$ \mathcal{L}_1( B)/I_s \simeq^{\overline{\varphi}} { B/I[ (\underline{x}_i)_{1\leq i\leq s}]}$$
and 
$$ \mathcal{L}_1( B/I) \simeq^{\widetilde{\varphi}} { B/I[ (\underline{x}_i)_{0\leq i\leq s}]}/{\overline{\varphi}(  \mathcal{L}_1( I)/ I_s)}$$ 
where \begin{itemize} 
\item $\varphi $ sends $\underline{x}_0$ to $\underline{x}$ and $\underline{x}_i$ to $\underline{x}_i$ for all $i \in \{ 1, \cdots, s\}$
\item $\overline{\varphi} $ sends $[\underline{x}_0]_{I_s}$ to $[\underline{x}]_{I_s}$ and $[\underline{x}_i]_{I_s}$ to $[\underline{x}_i]_{I_s}$ for all $i \in \{ 1, \cdots, s\}$.
\item $\widetilde{\varphi} $ sends $[\underline{x}]_{ \mathcal{L}_s(I)}$ to $[\underline{x}_0]_{ \mathcal{L}_s(I)}$ and $[\underline{x}_i]_{ \mathcal{L}_s(I)}$ to $[\underline{x}_i]_{ \mathcal{L}_s(I)}$ for all $i \in \{ 1, \cdots, s\}$. 
\end{itemize} 
Moreover, for all $C$ $B/I$-algebra, we have 
$$  \mathcal{L}_1( B/I) \otimes_{B/I} C\simeq { C[ (\underline{x}_i)_{1\leq i\leq s}]}/{\pi_C (\overline{\varphi} (  \mathcal{L}_1( I)/ I_s))}$$
where $\pi_C $ is the canonical map from $B/I[ (\underline{x}_i)_{1\leq i\leq s}]$ to $C[ (\underline{x}_i)_{1\leq i\leq s}]$. 
\end{lemma}


%\begin{lemma} 
%Let $B = k[\underline{x}]$ and $\mathfrak{p} \in \operatorname{Spec} (B)$. We have 
%$$\mathcal{L}_1( \mathfrak{p})^2_{k( \mathfrak{p})} = \langle (\pi_{k(\mathfrak{p})} (dp(\underline{x}_0) (\underline{x}_{1,1}, 
%\cdots , \underline{x}_{1, n})))^2| p(\underline{x}) \in  \mathfrak{p} \rangle$$
%and 
%$$\mathcal{L}_1 (B)_{k( \mathfrak{p} )} \simeq B_\mathfrak{p}/ \mathfrak{p}^2 B_\mathfrak{p}.$$
%\end{lemma}

%\end{exmp}
\section{Induced jet action}
\begin{definition}(Lemma)
Let $m\in \mathbb{N}$, $G$ be an abstract group, $B$ be a $R$-algebra, $\mathfrak{p} $ be a prime ideal of $B$ and $ \alpha :G \times B \rightarrow B $. We define the {\sf $m^{th}$ jet action induced by $\alpha$} denoted by $\mathcal{L}_m(\alpha) : \Gamma \times \mathcal{L}_m( B) \rightarrow \mathcal{L}_m (B)$ to be the map sending $(g, a)$ to $\mathcal{L}_m ( \alpha_g)(a)$ where $\alpha_g: B \rightarrow B$ is the map sending $b$ to $\mu (g, b)$. Let $m \geq -1$ and $s \leq m$, we denote $G_{m,s} ( \mathfrak{q})$  the $s^{th}$ ramification group at the prime ideal $\mathfrak{q}$ of $\mathcal{L}_m  (B)$. 
%This action induces a {\sf $m^{th}$-jet Galois morphism} $\mathcal{L}_m( Gal(\alpha)): \Gamma \times \mathcal{L}_m( B) \rightarrow \mathcal{L}_m(B) \times \mathcal{L}_m(B)$ sending $(g, a)$ to $( \mathcal{L}_m ( \alpha_g)(a), a)$. 
\end{definition} 
\begin{proof} 
$\mathcal{L}_m(\alpha)$ is a group action since $\underline{J_m}$ is a functor, that preserves the identity and composition of morphisms.
\end{proof} 
%\begin{exmp}
%We consider $B_n= \mathbb{Z}[x]/ (x^n-1)$, $p_n(x):= x^n$, $I_n= (p_n(x))$ be the ideal of $\mathbb{Z}[x]$ generated by $p_n(x)$, $\Gamma_n = \mathbb{Z}/n \mathbb{Z}$ and an action $\alpha_n : \Gamma_n \times   \mathbb{Z}[x]/ I_n \rightarrow  \mathbb{Z}[x]/ I_n$ sending $([k]_n , [x]_{c_n})$ to $[x^k]_{c_n}$ where $[k]_n$ is the class of $k$ in $\mathbb{Z}/n \mathbb{Z}$ and $[x]_{c_n}$ is the class of $x$ in $ \mathbb{Z}[x]/ I_n$. We have $p_n'(x)= n x^{n-1}$ and $p''_n(x) = n(n-1) x^{n-2}$. 
%
%Let $s \in \mathbb{Z}$. We have 
%%We compute $\mathcal{L}_s(B_n)$. 
%%We have 
%%$$\begin{array}{llll} ( \sum_{j=0}^s x_j [t]_s^j )^n-1 &=& \sum_{k_0 + \cdots + k_s = n} \frac{n!}{ k_0! k_1!\cdots k_s !} \prod_{0 \leq j \leq s } ( x_j [t]_s^j)^{k_j} -1 \\
%%&=& \sum_{k_0 + \cdots + k_s = n}  \frac{n!}{ k_0! k_1!\cdots k_s !} \prod_{0 \leq j \leq s } x_j^{k_j}  [t]_s^{\sum_{j=0}^s j k_j} -1 \\
%%& = &\sum_{l=0}^{s} \left( \sum_{\sum_{j=0}^s j k_j=l , \ k_0 + \cdots + k_s = n}\frac{n!}{ k_0! k_1!\cdots k_s !} \prod_{0 \leq j \leq s } x_j^{k_j} \right) [t]_s^{l} -1 \end{array} $$
%%Let $g_{n,l,s} = \sum_{\sum_{j=0}^s j k_j=l, k_0 + \cdots + k_s = n}\frac{n!}{ k_0! k_1!\cdots k_s !} \prod_{0 \leq j \leq s } x_j^{k_j}$.
%%Therefore,
%$$J_s( I_n)= \left\langle  g_{0}^{p_n(x)} -1, \left( g_{l}^{p_n(x)} \right)_{1\leq l\leq s}  \right\rangle$$
%$$\mathcal{L}_s(B_n) = k[ (x_i)_{0 \leq i \leq n}]/ J_s( I_n).$$
%Let $r\in \{ 0, \cdots, n-1\}$. We compute $J_s({\alpha_n}_{[r]}): \mathcal{L}_s (B) \rightarrow \mathcal{L}_s(B)$.
%$$\begin{array}{llll} ( \sum_{j=0}^s x_j [t]_s^j )^r &=&% \sum_{k_1 + \cdots + k_s = r} \frac{r!}{ k_1! k_2!\cdots k_s !} \prod_{0 \leq j \leq s } ( x_j [t]_s^j)^{k_j} = \sum_{k_1 + \cdots + k_s =r}  \frac{r!}{ k_1! k_2!\cdots k_s !} \prod_{0 \leq j \leq s } x_j^{k_j}  [t]_s^{\sum_{j=0}^s j k_j}\\ & = &
%\sum_{l=0}^{s}  g_{l}^{p_r(x)} [t]_s^{l}  \end{array} $$
%Therefore
%$$ \begin{array}{llll} \mathcal{L}_s({\alpha_n}_{[r]}): & \mathcal{L}_s (B) & \rightarrow & \mathcal{L}_s(B)\\
%& [x_l]_{\mathcal{L}_s(I_n)} & \mapsto & [g_{l}^{p_r(x)} ]_{\mathcal{L}_s(I_n)}
%\end{array} $$
%
%In particular, when $s=1$. 
%We have 
%$$( x_0+ x_1 [t]_1)^n-1= p_n(x_0 )-1 + p_n'(x_0 ) x_1 [t]_1  $$
%%= \left(\sum_{j=0}^{\lfloor n/2 \rfloor}  \binom{n}{2j} x_0^{n-2j} x_1^{2j} \right) + \left( \sum_{j=0}^{\lfloor n/2 \rfloor}  \binom{n}{2j+1} x_0^{n-(2j+1)} x_1^{2j+1} \right) [t] $$
%and 
%$$\mathcal{L}_1(B_n)= k[x_0, x_1] / \left\langle p_n(x_0) -1 ,p_n'(x_0 )x_1\right\rangle.$$
%and 
%$$ \begin{array}{llll} \mathcal{L}_1(\alpha_{[r]}): & \mathcal{L}_1 (B_n) & \rightarrow & \mathcal{L}_1(B_n)\\
%& [x_0]_{J_s(I_n)} & \mapsto & \left[ p_r(x_0 ) \right]_{\mathcal{L}_s(I_n)}\\
%& [x_1]_{J_s(I_n)} & \mapsto & \left[p_r'(x_0 ) x_1 \right]_{\mathcal{L}_s(I_n)}\\
%\end{array} $$
%
%When $s=2$. 
%We have 
%$$( x_0+ x_1 [t]+ x_2[t]^2)^n-1= p_n(x_0 )-1 + p_n'(x_0 ) x_1 [t] + \left( p_n'(x_0 )x_2 + \frac{1}{2} p_n''(x_0 ) x_1^2 \right) [t]^2  $$
%
%%= \left(\sum_{j=0}^{\lfloor n/2 \rfloor}  \binom{n}{2j} x_0^{n-2j} x_1^{2j} \right) + \left( \sum_{j=0}^{\lfloor n/2 \rfloor}  \binom{n}{2j+1} x_0^{n-(2j+1)} x_1^{2j+1} \right) [t] $$
%and 
%$$\mathcal{L}_1(B_n)= k[x_0, x_1, x_2] / \left\langle p_n(x_0 ) -1,p_n'(x_0 ) x_1, p_n'(x_0 ) x_2 +  \frac{1}{2} p_n''(x_0 ) x_1^2 \right\rangle.$$
%and 
%$$ \begin{array}{llll} \mathcal{L}_1(\alpha_{[r]}): & \mathcal{L}_1 (B_n) & \rightarrow & \mathcal{L}_1(B_n)\\
%& [x_0]_{J_s(I_n)} & \mapsto & \left[p_r(x_0 )  \right]_{\mathcal{L}_s(I_n)}\\
%& [x_1]_{J_s(I_n)} & \mapsto & \left[p_r'(x_0 ) x_1 \right]_{\mathcal{L}_s(I_n)}\\
%& [x_2]_{J_s(I_n)} & \mapsto & \left[p_r'(x_0 )x_2 + \frac{1}{2} p_r''(x_0 ) x_1^2 \right]_{\mathcal{L}_s(I_n)}\\
%\end{array} $$
%
%We have $B_n \simeq \prod_{d|n}  \mathbb{Z}[x]/ (\phi_d (x) )$ and $\Gamma_n$ also acts on $\mathcal{O}_{\mathbb{Q}(\zeta_n)} =  \mathbb{Z}[x]/ I_{\zeta_n} $ where $I_{\zeta_n}= \langle \phi_n(x)\rangle$ sending $( [r]_n ,[x]_{\zeta_n})$ to $[x^r]_{\zeta_n}$ where $[x]_{\zeta_n}$ is the class of $x$ in $\mathcal{O}_{\mathbb{Q}(\zeta_n)} $ . When $p$ is odd and $h, k \in \mathbb{N}$, we have $\phi_{2^h} (x) = x^{2^{h-1}}+1$, $\phi_{p^k}(x) = \sum_{j=0}^{p-1} x^{jp^{k-1}}$ and $\phi_{2^h p^k} (x) = \sum_{j=0}^{p-1} (-1)^j x^{j 2^{h-1} p^{k-1}} $.
%%\begin{itemize} 
%%\item $\phi_{2^h} (x) = x^{2^{h-1}}+1$, $$\mathcal{L}_s( I_{\zeta_{2^h}} )= \left\langle g_{2^{h-1},0,s}+ 1 , \left( g_{2^{h-1},l,s} \right)_{1\leq l\leq s}  \right\rangle$$ 
%%$$\mathcal{L}_1( I_{\zeta_{2^{h-1}}} )=  \left\langle x_0^{2^{h-1}} +1 ,x_0^{2^{h-1}-1} x_1\right\rangle,$$ 
%%$$\mathcal{L}_2( I_{\zeta_{2^{h-1}}} )=  \left\langle x_0^{2^{h-1}} +1 ,2^{h-1} x_0^{2^{h-1}-1} x_1, 2^{h-1} x_0^{2^{h-1}-1}x_2 + 2^{h-2}(2^{h-1}-1) x_0^{2^{h-1}-2} x_1^2\right\rangle$$
%%
%%\item $\phi_{p^k}(x) = \sum_{j=0}^{p-1} x^{jp^{k-1}}$
%%$$\mathcal{L}_s( I_{\zeta_{p^k}} )= \left\langle  \left(  \sum_{j=0}^{p-1} g_{jp^{k-1},l,s} \right)_{0\leq l\leq s}  \right\rangle$$
%%$$\mathcal{L}_1( I_{\zeta_{p^k}} )=  \left\langle  \sum_{j=0}^{p-1}x_0^{jp^{k-1}}  , \sum_{j=0}^{p-1} jp^{k-1} x_0^{jp^{k-1}-1} x_1\right\rangle =\left\langle  \frac{x_0^{(p-1) p^{k-1}}- 1}{x_0^{p^{k-1}}-1}  , \frac{jp^{k-1} \left( x_0^{(p-1) p^{k-1}}- 1 \right) x_1}{x_0(x_0-1)}\right\rangle ,$$ 
%%$$\begin{array}{lll} \mathcal{L}_2( I_{\zeta_{p^k}} )&=&  \left\langle  \sum_{j=0}^{p-1} x_0^{jp^{k-1}}  ,  \sum_{j=0}^{p-1}x_0^{jp^{k-1}-1} x_1, \sum_{j=0}^{p-1} \left( p^{k-1}   x_0^{jp^{k-1}-1}x_2 + \frac{p^{k-1}(p^{k-1}-1)}{2} x_0^{jp^{k-1}-2} x_1^2 \right) \right\rangle \\
%%&=&  \left\langle  \frac{x_0^{(p-1) p^{k-1}}- 1}{x_0-1} ,  \frac{x_1\left( x_0^{(p-1) p^{k-1}}- 1\right)}{x_0(x_0-1)} , p^{k-1}   \frac{x_0^{(p-1) p^{k-1}}- 1}{x_0(x_0-1)}x_2 + \frac{p^{k-1}(p^{k-1}-1)}{2} \frac{x_0^{(p-1) p^{k-1}}- 1}{x_0^2(x_0-1)} x_1^2 \right\rangle \\
%%&=&  \left\langle  \frac{x_0^{(p-1) p^{k-1}}- 1}{x_0-1} ,  \frac{x_1\left( x_0^{(p-1) p^{k-1}}- 1\right)}{x_0(x_0-1)} ,    \frac{p^{k-1} \left( x_0^{(p-1) p^{k-1}}- 1\right) \left( x_2x_0 + \frac{p^{k-1}-1}{2} x_1^2 \right)}{x_0^2(x_0-1)} \right\rangle 
%% \end{array}$$
%%and  
%%\item $\phi_{2^h p^k} (x) = \sum_{j=0}^{p-1} (-1)^j x^{j 2^{h-1} p^{k-1}} $ 
%%$$\mathcal{L}_s( I_{\zeta_{2^h p^k}} )= \left\langle  \left(  \sum_{j=0}^{p-1} (-1)^j g_{j 2^{h-1} p^{k-1},l,s} \right)_{0\leq l\leq s}  \right\rangle$$
%%$$\mathcal{L}_1( I_{\zeta_{2^{h} p^{k}}} )=  \left\langle  \sum_{j=0}^{p-1}(-1)^j  x_0^{j2^{h-1} p^{k-1}} ,\sum_{j=0}^{p-1}(-1)^j x_0^{j2^{h-1} p^{k-1}-1} x_1\right\rangle,$$
%% $$\begin{array}{lll} \mathcal{L}_2( I_{\zeta_{2^h p^k}} )&=&  \left\langle \sum_{j=0}^{p-1} (-1)^j x_0^{j2^{h-1} p^{k-1}} , \sum_{j=0}^{p-1} x_0^{j2^{h-1} p^{k-1}-1}(-1)^j  x_1, \right. \\
%%&& \left. \sum_{j=0}^{p-1} (-1)^j \left( 2^{h-1} p^{k-1} x_0^{j2^{h-1} p^{k-1}-1}x_2 + \frac{2^{h-1} p^{k-1}(2^{h-1} p^{k-1}-1)}{2} x_0^{j2^{h-1} p^{k-1}-2} x_1^2 \right) \right\rangle \\
%%&=&  \left\langle  -\frac{x_0^{(p-1) p^{k-1}2^{h-1}}+1}{x_0-1} ,  \frac{-x_1\left( x_0^{(p-1) p^{k-1}2^{h-1}}+ 1\right)}{x_0(x_0-1)} ,    \frac{- p^{k-1} 2^{h-1}\left( x_0^{(p-1) p^{k-1}2^{h-1}}+ 1\right) \left( x_2x_0 + \frac{p^{k-1}2^{h-1}-1}{2} x_1^2 \right)}{x_0^2(x_0-1)} \right\rangle . 
%%\end{array} $$
%%\end{itemize} 
%\end{exmp} 
\begin{lemma}
Let $B$ be a $R$-algebra, $\Gamma$ be a group and $\alpha : \Gamma \times B \rightarrow B$ be a group action. If $\alpha$ is a free action then $\mathcal{L}_m(\alpha)$ is a free group action. 
\end{lemma}
\begin{proof} 
 %\sophie{Suppose that $\alpha$ is a free action. 
%Let $(g, b) \in \Gamma \times B$ with $b\neq 0$ such that $\mathcal{L}_m(\alpha) ( g, b) = b$. We want to prove that $ g =e_\Gamma$.  To do this we consider the following commutative diagram 
%$$\xymatrix{ \Gamma \times B \ar[d]_{Id\times \rho_{m,0}^B}   \ar[rrrr]^{ \alpha} &&& & B \ar[d]^{\rho_{m,0}^B \times \rho_{m,0}^B}    \\   \Gamma \times \mathcal{L}_m( B)  \ar@/_1pc/[u]_{Id\times \sigma_{m}^B}  \ar[rrrr]^{ \mathcal{L}_m( Gal(\alpha)) }&& &&\mathcal{L}_m(B) \times \mathcal{L}_m(B)  \ar@/^1pc/[u]^{  \sigma_{m}^B \times \sigma_{m}^B}}$$ 

%We apply $\sigma_m^B$ to the equality and obtain, $\sigma_m^B (\mathcal{L}_m(\alpha) ( g, b) )= b$.
% That is the Galois map $Gal(\alpha): \Gamma \times B  \rightarrow B  \times B$ sending $( g, b)$ to $(\alpha(g, b), b)$ is injective. We want to prove that $ \mathcal{L}_m( \alpha )$ is free. That is $\mathcal{L}_m ( Gal(\alpha))$ is injective. To do this we consider the following commutative diagram 
%$$\xymatrix{ \Gamma \times B \ar[d]_{Id\times \mu_{m,0}^B}   \ar[rrrr]^{ Gal(\alpha)} &&& & B  \times B \ar[d]^{\mu_{m,0}^B \times \mu_{m,0}^B}    \\   \Gamma \times \mathcal{L}_m( B)  \ar@/_1pc/[u]_{Id\times \sigma_{m}^B}  \ar[rrrr]^{ \mathcal{L}_m( Gal(\alpha)) }&& &&\mathcal{L}_m(B) \times \mathcal{L}_m(B)  \ar@/^1pc/[u]^{  \sigma_{m}^B \times \sigma_{m}^B}}$$ 
%Let $(g_1, b_1), (g_2, b_2) \in \Gamma \times B$ such that $(\mathcal{L}_m ( Gal(\alpha)) (g_1, b_1), b_1) =(\mathcal{L}_m ( Gal(\alpha)) (g_2, b_2), b_2) $. 
%
%Applying $  \sigma_{m}^B \times \sigma_{m}^B$ to the last equality, we get 
%$$ ( \sigma_{m}^B(\mathcal{L}_m ( Gal(\alpha)) (g_1, b_1)),\sigma_{m}^B( b_1))  =  ( \sigma_{m}^B(\mathcal{L}_m ( Gal(\alpha)) (g_2, b_2)),\sigma_{m}^B( b_2)) $$
%By the commutativity of the diagram we have for $i=1,2$, 
%$$  Gal(\alpha)(g_i,  \sigma_{m}^B(b_i))= ( \sigma_{m}^B(\mathcal{L}_m ( Gal(\alpha)) (g_i, b_i)),\sigma_{m}^B( b_i)).$$
%Therefore, 
%$$ Gal(\alpha)( g_1,  \sigma_{m}^B(b_1))= Gal(\alpha)( g_2,  \sigma_{m}^B(b_2)).$$
%Since $\alpha$ is free, we have $g_2 =g_1$ as wanted.  Similarly, using $\mu_{m, 0}^B$, we can prove the converse. I don't understand what I am doing wrong here}
\end{proof} 
\section{Jet ramification group} 



